Studying Alignment in a Collaborative Learning Activity via Automatic Methods: The Link Between What We Say and Do

A dialogue is successful when there is alignment between the speakers at different linguistic levels. In this work, we consider the dialogue occurring between interlocutors engaged in a collaborative learning task, where they are not only evaluated on how well they performed, but also on how much they learnt. The main contribution of this work is to propose new automatic measures to study alignment; focusing on verbal (lexical) alignment, and behavioral alignment (when an instruction given by one was followed with concrete actions by another). A second contribution of our work is to study how spontaneous speech phenomena are used in the process of alignment. Lastly, we make public the dataset to study alignment in educational dialogues. Our results show that all teams verbally and behaviourally align to some degree regardless of their performance and learning, and our measures capture that teams that did not succeed in the task were simply slower to collaborate. Thus we find that teams that performed better, were faster to align. Furthermore, our methodology captures a productive period that includes the time where the interlocutors came up with their best solutions. We also find that well-performing teams verbalise the marker "oh" more when they are behaviourally aligned, compared to other times in the dialogue; showing that this marker is an important cue in alignment. To the best of our knowledge, we are the first to study the role of "oh" as an information management marker in a behavioral context (i.e. in connection to actions taken in a physical environment), compared to only a verbal one. Our measures contribute to the research in the field of educational dialogue and the intersection between dialogue and collaborative learning research.

==> sections/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}
In this article, we are interested in how children collaborate as they solve a problem together, in which what they say and do is strongly tied to how they perform, and subsequently what they will ultimately learn from the situated activity. To investigate this relationship, we consider the corpus of data (dialogue transcripts from audio files and action logs) generated by teams of two children engaged in a collaborative learning activity, called JUSThink, which aims at providing an intuitive understanding of graphs and spanning trees. Collaborative learning activities are a particularly interesting type of collaborative task, due to their ``multi-layered goals'', typically including immediate, performance goals (e.g., finding the solution to a math problem) and deeper, learning goals (e.g., understanding the notion of equation).

Collaboration often involves a dialogue amongst interlocutors. It has been shown that a dialogue is successful when there is alignment between the interlocutors, at different linguistic levels. However, research on alignment in dialogue shows a lack of (automatic) measures capable of capturing the links between alignment and task success, particularly for collaborative learning settings.

This work builds upon automatic state-of-the-art alignment measures to study a collaborative learning activity eliciting completely spontaneous spoken dialogues. We introduce new measures that allow us to study another level of alignment in situated dialogues; i.e.\ via automatically inferring instructions, and then linking those instructions to (matched or mismatched) actions. Specifically we consider in the situated environment the interlocutor's \romannumeral 1)~\emph{use} of expressions related to the task, and the \romannumeral 2)~\emph{follow-up} actions of such expressions. There is a crucial relationship between the two in this task, as interlocutors could simply be stuck \textit{saying}. For this purpose, we investigate in RQ1 what interlocutors ``say" at various phases in the dialogue (in H1.1), and how such expressions are surrounded by hesitation phenomena, i.e.\ the use of fillers like `um' and `uh' (H1.2). Then, RQ2 focuses on the relationship between expression and follow-up actions, at various phases in the dialogue (H2.1), and how the follow-ups are surrounded by information management phenomena, i.e.\ the use of `oh'. We also contribute a dataset of anonymised, transcribed children dialogues, event logs of their task progression, and code, which are all made publicly available to either reproduce our results or to use for further research. Our work highlights the need to bridge the gap between the fields of collaborative learning and dialogue analysis, and expand existing automatic measures for verbal behaviours, as they can have an impact on our understanding of the way children learn.

Considering the nature of the task, i.e.\ the situated environment, we limited our analysis to referents that were specific to the task. From a methodological perspective, this was done for several reasons: aside from being the minimal terminology interlocutors are required to use to ensure task success, it gives us insights into the way interlocutors (children) use (potentially unfamiliar) terminology related to the environment. Additionally, the referents are easy to automatically annotate from the transcripts without hand crafted annotations, and allow us to pinpoint specific areas of the activity where immediate effects on the situated environment are apparent -- by observing the process of instructions evolving into actions. Looking at the results of our automatic methods, the benefits of this methodological choice are more apparent 
%(for e.g.\ in Table~\ref{tab: algo_results_oh_17})
, as we can see that the annotations can be thought of as periods of the task where there are immediate, situated actions. These periods, by inspecting the annotations, are about specific objects in the situated environment and can be thought of as ``local contexts" in the timeline of the dialogue, i.e.\ the explicit reference to a node name; which results in actions that can be matched, mismatched or nonmatched. We complement the explicit use of these expressions with implicit markers of hesitation and information management. We thus decompose the overall \textit{use} of these expressions and \textit{follow-up} with actions into two aspects, i.e.\ `\textit{what} was said and done' and `\textit{how} it was said and done'.

A first finding of this work is the discovery that the measures we propose are capable of capturing elements of lexical alignment in such a context. In terms of results, for RQ1, we see that all teams establish routines, regardless of task success. An assumption that might be commonly made, is that the more aligned interlocutors are, the more are chances of their task success (usually, measured by performance alone). Indeed, our results from RQ1 indicate that this is not necessarily the case for lexical alignment: we rather observed that better performing teams were earlier than badly performing teams to align by our measures. In terms of the formation of a routine, we see that hesitation phenomena tend to occur around establishment times, and greatly after priming times, indicating that the IF could be using fillers in the role of clarification. For RQ2, we observe that all teams, regardless of task success, had matches and mismatches of instructions-to-actions. Similar to RQ1, we observed a general trend that better performing teams tend to follow up their instructions with actions earlier in the task rather than later. We see that information management phenomena tend to occur around the vicinity (specifically earlier) of (mis)matched actions, but the distributions overlap more for better-performing teams. 

While our measures discussed in RQ1 and RQ2 do not show significant results for learning, we still think considering learning with performance is an important first step in evaluating task success in these activities, as performance does not necessarily bring about learning~\citepalias{nasir_when_2020}. As an example we looked at Team 20, that performed well but did not learn. For this team, in H2.2, we saw that our measures suggest that the interlocutors were working in isolation, as evidenced by nonmatched actions. Our measures still reflect some fine-grained aspects of learning in the dialogue (such as an exploratory and collaborative period the interlocutors go through during the alignment process), even if we cannot conclude that overall they are linked to the final measure of learning. Our measures capture more aspects of performance than learning, as our measures focus on what was said specifically about the environment, and the immediate apparent changes to the environment -- essentially the crux of the task. At a higher level, lack of understanding/learning etc.\ could be reflected by other phenomena (such as other multimodal features \citep{nasir_is_2020,nasir_what_2021}), other expressions (``I don't understand") etc. Since there are many ways to learn, and hence different behaviours that could result in learning, it is unsurprising that such patterns are difficult to capture. 
 
Working with dialogues is complicated, due to \romannumeral 1)~the lack of automatic evaluation criteria (e.g.\ human annotators might instinctively be able to say that a particular team collaborated well after observing a dialogue, but it is hard to empirically pinpoint the exact reasons such a judgement was taken), and \romannumeral 2)~the nature of spontaneous speech (variable turn taking, disfluencies, etc.). Our results, albeit limited to a small dataset, highlight that in a situated activity, focusing simply on task-specific expressions and certain surrounding spontaneous speech phenomena can still give good insights into the nuances of collaboration between the interlocutors, and its ultimate links to task success (with the awareness that there are several other aspects that remain to be observed in the dialogue such as studying the gaze patterns, prosodic features and so on). However, work in collaborative learning tends to focus more on these non-verbal features; especially in automatic analysis. Future work will concentrate on other levels of alignment, for example prosodic cues. It would be interesting to look at the inferred instructions, rather than simply the (mis)match of these to actions, to see if this could give further insights into periods of collaboration and eventually learning amongst the interlocutors. We hope that the above findings can inspire further research on the topic and contribute to the design of technologies for the support of learning. 

==> sections/materials.tex <==
\section{Materials} \label{sec:materials}

\subsection{Collaborative problem solving activity, scenario and setup} \label{subsec:activity}

JUSThink is a collaborative problem solving activity for school children~(\citealt{nasir_you_2020}; \citetalias{nasir_when_2020}). It aims to improve their CT skills by exercising their abstract reasoning on graphs. Recent research on educational curricula stresses the need for learning CT skills in schools, as going beyond simple digital literacy to developing these CT skills becomes crucial~\citep{menon_going_2019}. With this in mind, the objective of the activity is to expose school children to minimum-spanning-tree problems\footnote{The minimum-spanning-tree problem is defined on a graph $G = (V, E)$ with a cost function on its edges $E$, where $V$ is the set of nodes, ${E \subseteq V \times V}$ is the set of edges that connects pairs of nodes. The goal is to find a subset of edges $T \subseteq E$ such that the total cost of the edges in $T$ is minimised. This corresponds to finding a minimum-cost sub-network of the given network.}.

\paragraph*{Scenario.}
A humanoid robot, acting as the CEO of a gold mining company, presents the activity to the children as a game, asking them to help it collect gold, by connecting gold mines one another with railway tracks. They are told to spend as little money as possible to build the tracks, which change in cost according to how they connect the gold mines. The goal of the activity is to find a solution that minimises the overall cost, i.e.\ an optimal solution for the given network\footnote{In the network used in the JUSThink activity, there exist 10 nodes: \{ `Luzern', `Interlaken', `Montreux', `Davos', `Zermatt', `Neuchatel', `Gallen', `Bern', `Zurich', `Basel' \} and 20 edges. A description of the network, with the node labels (e.g.\ ``Mount Luzern"), x, y position of a node, possible edges between the nodes, and edge costs, is publicly available online with the dataset (JUSThink Dialogue and Actions Corpus), from the Zenodo Repository DOI:~\href{\datasetLinkDOI}{\datasetDOI}.\label{foot:network}}.

Children participate in teams of two to collaboratively construct a solution, by drawing and erasing tracks. Once all gold mines are reachable, i.e.\ in some way connected to each other, they can submit their solution to the robot for evaluation. They must submit their solution together, and can submit as many times as they want. The robot then reveals whether their solution is an optimal solution or, if not, how far it is from an optimal solution (in terms of its cost). In the latter case, children are also encouraged by the robot to try again. They can submit a solution as many times as they want until the allotted time for the activity is over\footnote{Note that we treat this triadic activity as a dyadic dialogue. The children are initially prompted by the robot to work with each other, and later simply given the cost of their sub-optimal solution. However, almost all of the exchanges are between the two interlocutors. After careful observation of the dialogues in the dataset, we observe the tendency to ignore the robot unless submitting a solution.}.

\paragraph*{Setup.}
Two children sit across each other, separated by a barrier. A touch screen is placed horizontally in front of each child. Children can see each other, but cannot see the other's screen, as shown in Fig.~\ref{fig:setup}. They are encouraged by the robot to verbally interact with each other, and work together to construct a solution to the activity.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/setup-photo.jpg}
  \caption{The JUSThink activity setup.}
  \label{fig:setup}
\end{figure}

The screens display two different views of the current solution to the children. One view is an \emph{abstract view}, where the gold mines are represented as nodes, and the railway tracks that connect them as edges (see Fig.~\ref{fig:optimal_abstract}). The other view, or the \emph{visual view}, represents the gold mines and railway tracks with images (see Fig.~\ref{fig:optimal_visual}). A child in the abstract view can see the cost of built edges, but cannot act upon the network. Conversely, in the visual view, a child can add or delete an edge, which is a railway track, but cannot see its cost. The views of the children are swapped every two \emph{edit actions}, which is any addition or deletion of an edge. Hence, after every two edit actions, the child that was in the abstract view moves to the visual view and vice versa. A turn is thus the time interval between two view swaps, i.e.\ in which one child is in the visual view and the other child is in the abstract view. A turn lasts for two edit actions. This design aims at encouraging children (interlocutors) to collaborate.

\begin{figure}[tbp]
\centering
\subfloat[An example abstract view.]{%
\resizebox*{.49\linewidth}{!}{\includegraphics{figs/optimal-abstract.png}}\label{fig:optimal_abstract}} 
\hspace{0.01in}
\subfloat[Corresponding visual view.]{%
\resizebox*{.49\linewidth}{!}{\includegraphics{figs/optimal-visual.png}}\label{fig:optimal_visual}}
\caption{interlocutors' views during the JUSThink activity} \label{fig:optimal_views}
\end{figure}

This activity is particularly suited to study alignment, since it is designed in such a way to create interdependence, i.e.\ a mutual reliance to further the task, between the interlocutors. This interdependence requires interlocutors to align with each other on multiple levels, e.g.\ how to refer to the environment and how to represent the activity, in order to succeed. Concretely, the activity enables:

\begin{itemize}
\item \textbf{Swapping and visual view control.} Since a turn changes every two edit actions, if an interlocutor has a particular action they want to take, they have to either wait for their turn in the visual view to implement the desired change, or instruct the other interlocutor. Here, we follow an idealised perspective on the activity: at a given time, the interlocutor in the abstract view is an Instruction Giver (IG) who describes their instructions for the task by using specific referring expressions, and the other (in visual view) is the Instruction Follower (IF) who executes the action (this is akin to the Map Task~\citep{anderson_hcrc_1991})\footnote{In fact, the IF could also be following their own intuitions and ignoring the IG. Yet, ultimately we think this is a justified assumption, as only the IF is in control of the actions.}. The activity design creates a frequent swapping of views. This aims to discourage interlocutors from working in isolation or in fixed roles of IG and IF, which could potentially happen in collaborative tasks.
\item \textbf{Routine expressions and alignment in the task.} Since the robot uses brief and general instructions to present the activity and its goal, the interlocutors must figure out for themselves the way to approach the activity. The task-specific referents, which are the names of the gold mines (cities in Switzerland, a multi-lingual country)\footref{foot:network}, are potentially unfamiliar to interlocutors. Interlocutors must refer to the task, and then align with the other to form routine expressions. By aligning, they establish a shared lexicon, and thus align their representations of the activity with each other. 
\item \textbf{Submission of solutions.} Since the interlocutors have to submit their solution together by pressing the ``submit'' button that is present in both views, they have to, at least, align in terms of their intent to submit. Alternatively, one interlocutor must convince the other to reach a common intent.
\end{itemize}

\subsection{The Dataset} \label{subsec:dataset}

\paragraph*{Dataset description.} We collected the JUSThink dataset\footnote{The anonymised version of the dataset (JUSThink Dialogue and Actions Corpus), that includes dialogue transcripts, event logs, and test responses, is publicly available online, from the Zenodo Repository DOI:~\href{\datasetLinkDOI}{\datasetDOI}.}, which consists of 76 children in teams of two (41 females: ${M = 10.3}$, ${SD = 0.75}$ years old; and 35 males: ${M = 10.4}$, ${SD = 0.61}$). We have one problem solving session, i.e.\ task, per team. 8 out of the 38 teams ($\approx 21\%$) found an optimal solution to the activity. The teams were formed randomly, without considering the gender, nationality, or the mother tongue. They include mixed and same gender pairs, and this information is available but not used in our analyses. The study was conducted in multiple international schools in Switzerland, where the medium of education is in English, and hence students are proficient in English. The dataset contains:

\begin{enumerate}
\item \emph{The recorded audio files}: Audio was recorded as two mono audio channels synchronised to each other, with one lavalier microphone per channel. The interlocutors were asked to speak in English. The microphones were clipped onto the interlocutors' shirts. 
\item \emph{Event log files}: Event log entries consist of timestamped touch and button press events, application status changes, and the interlocutor's edits to the tracks.
\item \emph{Pre-test and post-test}: Interlocutors' responses to the items in the pre-test and post-test\footnote{See the App.~\ref{sec:pretest_and_posttest} for more details on the pre-test and the post-test\label{foot:suppl}.}.
\end{enumerate}

To measure \emph{performance} in the task, we use the cost of the solution submitted at each attempt, extracted from the event log files. To compute a measure of \emph{learning outcomes}, we use interlocutors' scores in the pre-test and the post-test (see Sec.~\ref{subsec:task_success} for the measure we adopt). To study how are task-specific referents are used (RQ1), we focus on the recorded audio files and transcribe a representative subset. For (RQ2), to see how do the interlocutors follow up the use of task-specific referents with actions, we combine the edit actions from the log files the with the transcripts.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=.75\linewidth]{figs/performance_vs_learning.pdf}
    \caption{Scatter plot of the transcribed teams (red dots) and non-transcribed teams (blue dots) in the learning outcome (\measure{learn}) vs.\ task performance (\measure{error}) space.
    The mean of a set (transcribed or other) is shown as a dashed line.
    Lines indicate the fit of a univariate kernel density estimate for the corresponding set.
    Numbers denote the ID of teams.
    } \label{fig:transcribed_scatter}
\end{figure}

\paragraph*{Transcribing a representative subset.} In order to study referring and alignment of the interlocutors, we selected a \emph{subset} of 10 teams of the dataset\footnote{We relied on manual transcription, due to the poor performance of state-of-the-art automatic speech recognition systems on this dataset which consists of children's speech with music playing in the background. The transcripts are publicly available online (in the \texttt{transcripts/} folder, available from the Zenodo Repository, DOI:~\href{\datasetLinkDOI}{\datasetDOI)}}. The teams were chosen to be a representative sample of the overall dataset (see Fig.~\ref{fig:transcribed_scatter}), keeping in mind the task success distribution; which we measure through performance in the task and learning outcomes observed from the pre-test and the post-test\footnote{See App.~\ref{sec:choosing_subset} for details on the selection.}. Table~\ref{tab:transcribed_descriptive_statistics} provides further details about the transcribed subset. As shown, the mean duration of the task is $\approx{23}$ minutes, and the transcriptions account for $\approx{4}$ hours of data. 

The transcripts report which interlocutor is speaking (either $A$ or $B$) and the start and end timestamps for each utterance, beside the utterance content. Utterance segmentation is based on~\citet{koiso1998analysis}'s definition of an \textit{Inter Pausal Unit (IPU)}, defined as ``a stretch of a single interlocutor's speech bounded by pauses longer than 100 ms". We also annotated punctuation markers, such as commas, full stops, exclamation points and question marks.  Fillers, such as `uh' and `um', (using~\citet{meteer_dysfluency_1995} for reference) were transcribed, as well as the discourse marker `oh'\footnote{`Oh' can also be treated as a filler in \citet{meteer_dysfluency_1995}, but we consider the usage of `oh' more aligned with~\citep{schiffrin1987discourse}.}. The above 3 spontaneous speech phenomena occur frequently in the dataset \{`um': 236, `uh': 173, `oh': 333\}. Other phenomena, such as `ew' or `oops!' were also transcribed, however, their frequency is too low for analysis. Transcription included incomplete elements, such as ``Mount Neuchat-'' in ``Mount Neuchat- um Mount Interlaken". 

\begin{table}[tbp]
    \centering
    \caption{Descriptive statistics for the transcribed teams (${N=10}$). SD stands for standard deviation.}
    \begin{tabular}{r|rrrr}
        {}                             & mean  &   SD   & min              &       max  \\
        \midrule
        number of submitted solutions        &  9.4  &  4.7  & 4\phantom{.0}    & 19\phantom{.0} \\
        number of turns in task           & 50.4  & 21.4  & 28\phantom{.0}   & 98\phantom{.0} \\ \hline
        total duration (mins)           & 23.7  &  7.1  & 11.2             & 36.0           \\
        time per submission (mins)       &  2.6  &  2.3  & 0.7              &  12.8           \\
        duration of a turn (secs)           &  25.0 & 30.3  & 1.1             & 240.2           \\ \hline
        length of utterance (in tokens) & 6.6 & 5.4 & 1\phantom{.0} & 32\phantom{.0} \\
    \end{tabular}
    \label{tab:transcribed_descriptive_statistics}
\end{table}

Pronunciation differed among and within interlocutors (for example, for the word `Montreux', pronouncing the ending as /{}ks/{} or /{}\o/{}), due to the unfamiliarity of the interlocutors with the referents, and individual accents. As our methodology is dependent on matching surface forms (refer to Sec.~\ref{sec:methodology}), we did not transcribe pronunciation variants of a word\footnote{We standardise variations of pronunciation in the transcriptions, and we do not account for e.g.\ variations in accent.}. A graduate student completed two passes on each transcript, which were then checked by another native English speaker graduate student with experience in transcription/annotation tasks.

\newpage

==> sections/methodology.tex <==
\section{Methodology} \label{sec:methodology}

\subsection{Structure of the Paper and the Hypotheses} \label{subsec:structure}

The present work focuses on the \emph{task-specific referents} that interlocutors minimally require to succeed in the task. Therefore, we restrict the possible referring expressions to ones that contain task-specific referents, in particular, to the objects that the interlocutors are explicitly given on the map (see Fig.~\ref{fig:optimal_views}). Interlocutors only need this terminology with certain function words to progress in the task (e.g.\ ``Montreux to Basel"). We believe that this design choice is particularly suited to study alignment in this type of activity, as the frequent swapping of views encourages the interlocutors to communicate with the other their intents using these referents. This allows us to focus on verbal contributions that are explicitly linked to the `situatedness' of the task and it's relation to a final measure of task success. While there are certainly other referring expressions to consider (e.g.\ ``That mountain there") not containing task-specific referents, it would require some degree of manual annotation. We thus focus on task/domain specific referents that can be automatically extracted.

With this in mind, RQ1 considers the \emph{use} of task-specific referents, while RQ2 considers the \emph{follow-up} actions taken after these task-specific referents were uttered. Thus RQ1 focuses solely on the surface-level utterances, i.e.\ ``What did the interlocutors say", while RQ2 builds on this with actions, i.e.\ ``What did the interlocutors do \textit{afterwards}". Since the nature of the activity is situated, we look into whether the interlocutors are stuck \textit{saying} task specific referents, or whether the use of these referents spurs the interlocutors into action; i.e.\ into \textit{doing}. We investigate RQ1 and RQ2's relation to task success, which is evaluated by two measures: \romannumeral 1)~performance, and \romannumeral 2)~learning outcomes. Please refer to Fig.~\ref{fig:structure} for an overview of the RQs. 

\paragraph*{RQ1: How do the interlocutors use task-specific referents? Does this link to task success?}
In RQ1, we specifically consider the link between the use of task-specific referents and task success through the routines' \romannumeral 1)~temporality, and \romannumeral 2)~surrounding hesitation phenomena. We expand on these in Sec.~\ref{subsec:studying_RQ1}.  Specifically, we hypothesise:
\begin{itemize}
    \item \textbf{H1.1: Task-specific referents become routine early for more successful teams.} We expect better performing teams to establish routine expressions earlier in the dialogue. Ideally by quicker establishment of routine expressions, teams will understand each other faster and thus perform better in the task, and learn more.
    
    % when task-specific referents become routine, 
    \item \textbf{H1.2: Hesitation phenomena are more likely to occur in the vicinity of priming and establishment of task-specific referents for more successful teams.}
    We expect that new contributions to the dialogue, via priming (the speaker first introduces the referent) and establishment (the listener utilises this referent for the first time) of routine expressions are associated with hesitation phenomena. A prolonged occurrence of hesitation phenomena not associated with the priming or establishment of routine expressions could highlight greater lack of understanding of the task, and hence be related to lower task success.
\end{itemize}

\paragraph*{RQ2: How do the interlocutors follow up the use of task-specific referents with actions? Does this link to task success?}
RQ2 investigates how the use of task-specific referents manifests in the interlocutors' actions within the task, and whether this affects their task success. For this purpose, we consider the \emph{instruction}s of an interlocutor, as the verbalised instructions one interlocutor gives to the other, which we extract through their use of task-specific referents. A physical manifestation of this instruction could result in a \emph{corresponding} an edit action\footnote{Note that there need not be an instruction that precedes an action, i.e.\ an interlocutor in the visual view can take less-informed actions by him/herself, see Sec.~\ref{subsec:activity}.}, or a \emph{different} edit action. We investigate the follow-up actions of the task-specific referents which its effect on task success, through the follow-up actions' \romannumeral 1)~temporality, and the \romannumeral 2)~surrounding information management phenomena. We expand on these in Sec.~\ref{subsec:studying_RQ2}. We hypothesise:

\begin{itemize}
    \item \textbf{H2.1: Instructions are more likely to be followed by a corresponding action early in the dialogue for more successful teams.}
    We expect that the earlier interlocutors align with each other in terms of instructions and follow-up actions, the better they progress in the task, and the greater the chance of success in the task. This idea of verbalised instructions being followed up by corresponding actions is in line with previous research on alignment (i.e., interlocutors being in alignment in a successful dialogue, see Sec.~\ref{sec:introduction}). However, work on collaborative learning suggests that individual cognitive development (in our case, positive learning outcomes) happens via \emph{socio-cognitive conflict}~\citep{mugny_socio-cognitive_1978,doise_social_1984}, and its regulation~\citep{butera_sociocognitive_2019}. In our task, this means a verbalised instruction could be followed by a corresponding or a different action; as a different action could result in collaboratively resolving conflicts and together building a solution -- resulting in task success. It is thus the required effort to construct the shared understanding together that results in collaborative learning~\citep{dillenbourg_evolution_2009}. For alignment purposes we focus on corresponding actions, but also follow-ups with a different action to gain a clearer picture into the alignment processes of the interlocutors.
    
    \item \textbf{H2.2: When instructions are followed by a corresponding or a different action, the action is more likely to be in the vicinity of information management phenomena for more successful teams.}
    The activity involves the creation of a joint focus of attention and the management of information states that are likely to be accompanied by information management phenomena, such as the use of `oh' as an information marker~\citep{schiffrin1987discourse}. Ultimately, an increase in shared information should lead to an increase in task success.
\end{itemize}


\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/paper_structure.pdf}
  \caption{The RQs investigated in this article.}
  \label{fig:structure}
\end{figure}

\newpage

\subsection{Measuring Success in the Task} 
\label{subsec:task_success}

\paragraph*{Measuring task performance.} \label{subsubsec:task_performance}
We adopt a measure that is based on the costs of the submitted solutions compared to the cost of an optimal solution (which is always the same). For each proposed solution, we calculate the normalised cost as the difference between the cost of the solution and the cost of an optimal solution, normalised by the cost of the optimal solution. We define \measure{error} as the smallest normalised cost value among all submitted solutions, which represents the team's closest solution to an optimal solution. We use \measure{error} to measure task performance\footnote{We process logs (folder \folder{logs/} in the dataset at DOI:~\href{\datasetLinkDOI}{\datasetDOI}) with a script (\notebook{tools/1\_extract\_performance\_and\_other\_features\_from\_logs.ipynb} in the tools at DOI:~\href{\toolsLinkDOI}{\toolsDOI}) to compute the \measure{error} for each team (in table \notebook{processed\_data/log\_features/justhink19\_log\_features\_task\_level.csv}, available with the tools).}.

\paragraph*{Measuring learning outcomes.} 
\label{subsubsec:learning_outcomes}
Learning measures commonly build upon the difference between the post-test and pre-test results, e.g.\ in~\citep{sangin_facilitating_2011}; which indicates how much an interlocutor's knowledge on the subject has changed due to the activity. We measure the learning outcomes on the basis of the relative learning gain (\measure{learn\textsubscript{\textit{P}}}) of an interlocutor $P$, which essentially is the difference between pre-test and post-test, normalised by the margin of improvement or decline~\citep{sangin_facilitating_2011}. It is computed as:
\begin{equation}
\measure{learn\textsubscript{\textit{P}}} = 
    \begin{cases} 
      \frac{post - pre}{10 - pre} & post \geq pre \\
      \frac{post - pre}{pre} & post < pre,
    \end{cases}
\end{equation}
where 10 is the maximum score available. It indicates how much the interlocutor learnt as a fraction of how much the interlocutor could have learnt. We use \measure{learn}, the average relative learning gain of both interlocutors, to measure a team's learning outcomes\footnote{We process test responses (folder \folder{test\_responses/} in the dataset) with a script (\notebook{tools/2\_extract\_learning\_gain\_from\_test\_responses.ipynb} in the tools) to compute the \measure{learn} for each team (in table \notebook{processed\_data/learning\_features/justhink19\_learning\_features.csv}, available with the tools).}.

\subsection{Studying the Interlocutors' Use of Task-specific Referents (RQ1)} \label{subsec:studying_RQ1} 

\paragraph*{Detecting routines of task-specific referents.} \label{subsec:detecting_routines}
We formally define a \emph{routine} expression (adapted from \citet{dubuisson-duplessis_automatic_2017,dubuisson_duplessis_towards_2021,pickering_towards_2004}) as a referring expression shared by two interlocutors if \romannumeral 1)~the referring expression is produced by both interlocutors, and \romannumeral 2)~it is produced at least once without being part of a larger routine. A routine is based on the reuse of a referring expression, but is specific to the exact matching of token sequences in two utterance strings. Using the above terminology, `Montreux' is a task-specific referent, and an interlocutor might \textit{prime} the referring expression ``Mount Montreux". If the other interlocutor \textit{reuses} this referring expression, it thus becomes \emph{routine}. In particular, we define the utterance at which a referring expression becomes routine as the \emph{establishment} of that routine. We extract routines and the utterances at which the routines are primed and established from the transcripts as in~\citep{dubuisson-duplessis_automatic_2017,dubuisson_duplessis_towards_2021}. Then, we filter for the routines that contain a task-specific referent\footnote{We process the transcripts (folder \folder{transcripts/} in the dataset at DOI:~\href{\datasetLinkDOI}{\datasetDOI}) with a script (\notebook{tools/4\_extract\_routines\_from\_transcripts.ipynb} in the tools at DOI:~\href{\toolsLinkDOI}{\toolsDOI}) to extract routines (in tables in folder \folder{processed\_data/routines/}, available with the tools). We use the \texttt{dialign} package v1.0, available at \url{https://github.com/GuillaumeDD/dialign}, by~\citep{dubuisson-duplessis_automatic_2017,dubuisson_duplessis_towards_2021}.}.

\paragraph*{Studying the temporality of the establishment of the routines (H1.1).} \label{subsec:temporality_of_routines}
To investigate when the routine expressions become established, we study \romannumeral 1)~the \emph{establishment time} of a routine, i.e.\ the end time of the utterance at which the expression is established, and \romannumeral 2)~the \emph{collaborative period} of a team, i.e.\ the duration between first quartile (Q1) to third quartile (Q3), i.e.\ the interquartile range (IQR) of the establishment, where half of the establishments occur. 

To study H1.1, for task performance, we check if the median establishment times are significantly earlier for better-performing teams by Spearman's rank correlation and its statistical significance (between the median and the \measure{error}). For the learning outcomes, we compare the distribution of the median establishment times of teams with positive learning outcomes (Teams 7, 9, 10, 11, 17) and others (Teams 8, 18, 20, 28, 47) by Kruskal-Wallis H test\footnote{Since we have groups of 5 teams for learning, we use Kruskal-Wallis (\href{https://www.scipy.org/}{SciPy}'s implementation of Kruskal-Wallis works with $\geq5$ samples). This can not be used for performance.}. We consider \romannumeral 1)~the establishment times of all the routines in real time (as teams finished took different durations to complete the task), \romannumeral 2)~the establishment times of the routines that are established in the common time duration (of all the participants, the first $\approx 11$ mins, which was the time taken by the quickest team), and \romannumeral 3)~normalised establishment times, that are scaled by the duration of each team itself to reflect the `progress' of a team's interaction, from 0\% progress at the beginning of the activity, to 100\% when the interaction ends (either by finding an optimal solution, or by being intervened by the experimenters). To gain further insight, we compare the distribution of the establishment times (from \romannumeral 1) to \romannumeral 3)) of the teams, through inspecting the box plots of all teams that are compared side-by-side and sorted by decreasing task success\footnote{Our analysis on each hypothesis is publicly available online with a script \notebook{tools/7\_test\_the\_hypotheses.ipynb} among the tools, from the Zenodo Repository, DOI:~\href{https://sandbox.zenodo.org/record/742549}{10.5072/zenodo.742549}.}.

\paragraph*{Linking hesitation phenomena to the establishment of the routines (H1.2).} \label{subsec:hesitation_phenomena_and_establishment}
To measure hesitation phenomena, we choose fillers (in particular `uh' and `um') specifically due to their many links with the uncertainty of the interlocutor, be it by simple hesitation~\citep{Pickett2018_American}, deeper meanings of a speaker's feeling of how knowledgeable they are~\citep{smith1993_course}, or even the listener's impression of how knowledgeable is the speaker~\citep{Brennan1995_feeling}. Fillers can thus be used by the interlocutor to inform the listener about upcoming new information, or even production difficulties that they are facing. Particular to the establishment of referring expressions, research has shown that disfluency (studied with the filler `uh') biases listeners towards new referents~\citep{arnold2004old} rather than ones already introduced into the discourse, and helps listeners resolve reference ambiguities~\citep{arnold2007if}.

To investigate H1.2, we inspect the distribution of filler times, in relation to the \romannumeral 1)~establishment and \romannumeral 2)~priming times of routine expressions. This is done to account for when a speaker introduces a new task-specific referent into the dialogue, and when the listener makes this expression routine for the first time. In particular, we note the order of the tokens in the dialogue for the filler positions and the first token of the priming/establishment instance. Then, we check whether the distributions of filler times (by its token position) with establishment times and priming times are significantly different (by its first token's position), by utilising a Mann-Whitney U Test, and estimate the effect size by computing Cliff's Delta. Then, we compare these results for the teams as sorted by increasing task success: for task performance, we compute the Spearman's correlation and its significance between Cliff's Delta and \measure{error}. For learning outcomes, we perform Kruskal-Wallis H test to compare the distribution of Cliff's Delta values for the two groups of learning.

\subsection{Studying the follow up of task-specific referents with actions (RQ2)} \label{subsec:studying_RQ2}

\paragraph*{Detecting follow-up actions of the task-specific referents.} \label{subsec:detecting_follow_up_actions}
If an instruction is verbalised (for e.g.\ to connect ``Mount Basel to Montreux") by an interlocutor (IG), it could result in an action of connecting the two. We hence say an instruction \emph{match}es an action when the instruction is executed by the other interlocutor (IF) via an action in the situated environment\footnote{Within the period of a turn of views before they are swapped.}. We study the discrepancy created when the IF does not follow the IG, which we call \emph{mismatch} of instructions-to-actions. In Example~\ref{quote:justhink_task}, the instruction (to connect Gallen to Davos) matches the action (connecting these two). The following example illustrates a dialogue excerpt that results in a mismatch\footnote{From Team 8, extracted/detected by using our Algorithms~\ref{algo:recognise_instructions} and \ref{algo:match_instructions_actions}. The whole dialogue with the annotations is available in the annotated corpus (\folder{processed\_data/annotated\_corpus}, available with the tools).}:

\begin{idea}
\noindent\textbf{\textit{B}:} Go to Mount Basel. \hfill \textit{[Instruction to add an edge to Basel.]}
\newline \textbf{\textit{A}:} That's, it's expensive.
\newline \textbf{\textit{B}:} Just do it.
\newline \textbf{\textit{A}:} You can't, you can't, I can't because there's a mountain there \dots
\newline \textbf{\textit{A}:} So I'm going, so I'm going here.
\newline \textlangle \textit{A} connects Mount Interlaken to Mount Bern\textrangle \hfill \textit{[Mismatch!]}
\label{quote:mismatch_example}
\end{idea}

We extract instructions from the utterances through the interlocutors' use of task-specific referents\footnote{We design \textsc{Recognise-Instructions}, described in Algorithm~\ref{algo:recognise_instructions}, that uses Algorithm~\ref{algo:recognise_entities}, which automatically infers a sequence of instructions from an input utterance, via a rule-based algorithm. Its implementation is available with the tools.} and find (mis)matches of instructions-to-actions\footnote{We design \textsc{Match-Instructions-to-Actions}, described in  Algorithm~\ref{algo:match_instructions_actions}.}\textsuperscript{,}\footnote{In our implementation, we combine the transcripts and the logs (from the dataset at DOI:~\href{\datasetLinkDOI}{\datasetDOI}) via a script (\notebook{tools/5\_construct\_the\_corpus\_by\_combining\_transcripts\_with\_logs.ipynb} in the tools at DOI:~\href{\toolsLinkDOI}{\toolsDOI}) to generate a combined corpus (\folder{processed\_data/corpus/} available with the tools). Then, we process this corpus via a script (\notebook{tools/6\_recognise\_instructions\_detect\_follow-up\_actions.ipynb} in the tools) to generate an annotated corpus (\folder{processed\_data/annotated\_corpus}, available with the tools). The annotated corpus contains the inferred instructions, matches, mismatches, and nonmatches if there were no instructions to be matched.).}. Algorithm~\ref{algo:match_instructions_actions}, that uses Algorithm~\ref{algo:check_match}, accounts for partial matches of nodes, i.e.\ an IG need not explicitly say both node names. It builds up (``caches") pending instructions that have not been followed, clearing them once the views are swapped. The cache of instructions is also cleared if after an edit action a match or mismatch of instructions-to-actions is detected. This allows for matching of negotiated nodes: in Example~\ref{quote:justhink_task}, Gallen-Davos was the result of a negotiation, rather than a complete given instruction by the IG. B says in one utterance ``oh Mount Davos" and then in another ``to Mount Gallen yeah do that", resulting in two cached inferred instructions; (Davos,?) and (Gallen,?) respectively. This accounts for some amount of multiple speaker-turn negotiations, and possible other ways of referring to task-specific referents (e.g\ ``Now go from \textbf{there} to Davos")\footnote{Though an instruction could be carried out after the views swap again, i.e.\ in the following turn: in our algorithm, the pending instructions are cleared at every swap, resulting in a nonmatch.}. See Table~\ref{tab:algo_results} in Sec.~\ref{subsec:results_rq2} for another example.

\paragraph*{Studying the temporality of the follow-up actions (H2.1).} \label{subsubsec:temporality_of_follow_up_actions}
To investigate H2.1, we compare the distributions of the match and mismatch times of the teams, by following the same methodology stated for H1.1 (which investigated establishment and priming times). In particular, we check if the median match or mismatch times are significantly earlier for better-performing teams by Spearman's rank correlation, and for the two groups of learning, by Kruskal-Wallis H test.

\paragraph*{Linking information management phenomena to follow-up actions (H2.2).}  \label{subsubsec:info_management_phenomena_follow_up_actions}
We consider the use of `oh' as an information management marker, to mark a focus of speaker's attention, which then also becomes a candidate for the listener's attention. This creation of a joint focus of attention allows for transitions in the information state~\citep{schiffrin1987discourse}. We are interested in what is commonly known by the interlocutors regarding the task (as an information state). Instructions that contain `oh' in their surrounding context are used by the speaker to inform the listener about some change in their information state. This can either be done in speaker turn utterance (``Oh, this is how we do the task") or as a backchannel (typically by the listener: ``Oh okay, oh yeah \dots"). Ultimately this increase in shared information should lead to an increase in task success.

To investigate H2.2, we check if the distributions of (mis)matches and `oh' marker times are significantly different by Mann-Whitney U test, and estimate the effect size by computing Cliff's Delta. This calculation differs from H1.2, as actions are not part of an utterance (compared to establishment time for example); hence we cannot use the order of tokens as was previously used, and instead compare the end times of the utterance that contains the marker with the (mis)matched action times. Then, as H1.2, we calculate the relation to performance and learning.

==> sections/methodology_obsolete.tex <==
\section{Studying Verbal Alignment (RQ1)} \label{sec: methodology}
\subsection{Methodology} \label{subsec: studying_RQ1} 
\paragraph*{Studying how expressions related to the task contribute to verbal alignment.} \label{subsec: detecting_routines}
A routine is formed when a referring expression is commonly used by both interlocutors. For e.g.,  `Montreux' is a task-specific referent, and one interlocutor might \textit{prime} the referring expression ``Mount Montreux". If the other interlocutor \textit{reuses} this referring expression, it becomes \emph{routine}, or commonly part of the dialogue. 

For our methodology, a routine is specific to the exact matching of token sequences in two utterance strings. We thus formally define a \emph{routine} expression (adapted from \citet{dubuisson-duplessis_automatic_2017,dubuisson_duplessis_towards_2021,pickering_towards_2004}) as a referring expression shared by two interlocutors if \romannumeral 1)~the referring expression is produced by both interlocutors, and \romannumeral 2)~it is produced at least once without being part of a larger routine.  
In particular, we define the utterance at which a referring expression becomes routine as the \emph{establishment} of that routine. We extract the utterances at which the routines are primed and established from the transcripts as in~\citep{dubuisson-duplessis_automatic_2017,dubuisson_duplessis_towards_2021}. Then, we filter for the routines that contain a task-specific referent.


% \footnote{We process the transcripts (folder \folder{transcripts/} in the dataset at DOI:~\href{\datasetLinkDOI}{\datasetDOI}) with a script (\notebook{tools/4\_extract\_routines\_from\_transcripts.ipynb} in the tools at DOI:~\href{\toolsLinkDOI}{\toolsDOI}) to extract routines (in tables in folder \folder{processed\_data/routines/}, available with the tools). We use the \texttt{dialign} package v1.0, available at \url{https://github.com/GuillaumeDD/dialign}, by~\citep{dubuisson-duplessis_automatic_2017,dubuisson_duplessis_towards_2021}.}.

\paragraph*{Studying when interlocutors are verbally aligned and its association with task success (H1.1).} \label{subsec: temporality_of_routines}
To investigate when the routine expressions become established, we study \romannumeral 1)~the \emph{establishment time} of a routine, i.e.\ the end time of the utterance at which the expression is established, and \romannumeral 2)~the \emph{collaborative period} of a team, i.e.\ the duration between first quartile (Q1) to third quartile (Q3), i.e.\ the interquartile range (IQR) of the establishment, where half of the establishments occur. 

To then study H1.1, for task performance, we check if the median establishment times are significantly earlier for better-performing teams by Spearman's rank correlation and its statistical significance (between the median and the \measure{error}). For the learning outcomes, we compare the distribution of the median establishment times of teams with positive learning outcomes (Teams 7, 9, 10, 11, 17) and others (Teams 8, 18, 20, 28, 47) by Kruskal-Wallis H test\footnote{Since we have groups of 5 teams for learning, we use Kruskal-Wallis (\href{https://www.scipy.org/}{SciPy}'s implementation of Kruskal-Wallis works with $\geq5$ samples). This can not be used for performance.}. We consider \romannumeral 1)~the establishment times of all the routines in real time (as teams finished took different durations to complete the task), \romannumeral 2)~the establishment times of the routines that are established in the common time duration (of all the participants, the first $\approx 11$ mins, which was the time taken by the quickest team), and \romannumeral 3)~normalised establishment times, that are scaled by the duration of each team itself to reflect the `progress' of a team's interaction, from 0\% progress at the beginning of the activity, to 100\% when the interaction ends (either by finding an optimal solution, or by being intervened by the experimenters). To gain further insight, we compare the distribution of the establishment times (from \romannumeral 1) to \romannumeral 3)) of the teams, through inspecting the box plots of all teams that are compared side-by-side and sorted by decreasing task success\footnote{Our analysis on each hypothesis is publicly available online with a script \notebook{tools/7\_test\_the\_hypotheses.ipynb} among the tools, from the Zenodo Repository, DOI:~\href{https://sandbox.zenodo.org/record/742549}{10.5072/zenodo.742549}.}.

\paragraph*{Studying hesitation phenomena surrounding verbal alignment and its association with task success (H1.2).} \label{subsec: hesitation_phenomena_and_establishment}
To measure hesitation phenomena, we choose fillers (in particular `uh' and `um') specifically due to their many links with the uncertainty of the interlocutor, be it by simple hesitation~\citep{Pickett2018_American}, deeper meanings of a speaker's feeling of how knowledgeable they are~\citep{smith1993_course}, or even the listener's impression of how knowledgeable is the speaker~\citep{Brennan1995_feeling}. Fillers can thus be used by the interlocutor to inform the listener about upcoming new information, or even production difficulties that they are facing. Particular to the establishment of referring expressions, research has shown that disfluency (studied with the filler `uh') biases listeners towards new referents~\citep{arnold2004old} rather than ones already introduced into the discourse, and helps listeners resolve reference ambiguities~\citep{arnold2007if}.

To investigate H1.2, we inspect the distribution of filler times, in relation to the \romannumeral 1)~establishment and \romannumeral 2)~priming times of routine expressions. This considers when a speaker introduces a new task-specific referent into the dialogue, and when the listener makes this expression routine for the first time. In particular, we note the order of the tokens in the dialogue for the filler positions and the first token of the priming/establishment instance. Then, we check whether the distributions of filler times (by its token position) with establishment times and priming times are significantly different (by its first token's position), by utilising a Mann-Whitney U Test, and estimate the effect size by computing Cliff's Delta. Then, we compare these results for the teams as sorted by increasing task success: for task performance, we compute the Spearman's correlation and its significance between Cliff's Delta and \measure{error}. For learning outcomes, we perform Kruskal-Wallis H test to compare the distribution of Cliff's Delta values for the two groups of learning.

\subsection{Results} \label{subsec:results_rq1}

\subsubsection*{H1.1: Task-specific referents become routine early for more successful teams.} \label{subsec:results_h1_1}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/h1_1_time_absolute_plot.pdf}
    \caption{The team's establishment times for H1.1. The teams are sorted by decreasing task performance (i.e.\ increasing \measure{error}). The boxplots, with the same colour have the same \measure{error} (sorted by increasing duration for the ties). The thick, bold boxplots with whiskers with maximum 1.5 IQR show the distributions of the establishments that occurred in the common duration (i.e.\ as marked by the dashed green line), while the thin boxplots show the distributions through the total duration of interaction. The learning outcome of each team is indicated with a plus (`+') for $\measure{learn} > 0$, or a minus (`-') otherwise. Solid lines indicate the end of the interaction, by submitting a correct solution (in green) or timing out (in red). The thin blue lines indicate submission of a solution, with the number showing the error quantifying how far the submitted solution is from an optimal solution in terms of its cost (e.g.\ $\measure{error} = 0\%$ means the team has found an optimal solution). The red and blue dots indicate the utterance times of the interlocutors, to give an idea of when the interlocutors are speaking versus when are their establishment times.} \label{fig:h1_1_time_absolute_plot}
\end{figure}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/h1_1_time_plot.pdf}
    \caption{The teams' establishment times as normalised by the duration for each team separately, i.e.\ 100\% indicates the end of that team's interaction. Sorting is as in Fig.~\ref{fig:h1_1_time_absolute_plot}.} \label{fig:h1_1_plot}
\end{figure}

\paragraph{For task performance.}
Fig.~\ref{fig:h1_1_time_absolute_plot} shows for each team the distribution of the establishment times of the routines. The median establishment times for all of the routines is strongly positively correlated with the task performance measure \measure{error} (Spearman's $\rho =0.69$, $p < .05$), that is, better-performing teams establish routines earlier\footnote{The magnitude of Spearman's correlation coefficient ($\rho$) can be interpreted by using the thresholds e.g.\ from~\citet{evans_straightforward_1996}, i.e.\ $0.00-0.19$ ``very weak", $0.20-0.39$ ``weak", $0.40-0.59$ ``moderate", $0.60-0.79$ ``strong", and $0.80-1.00$ ``very strong" \label{foot:spearman_groups}.}. We see from the figure that the results are influenced by the variation in the duration of the activity: the interaction ends for the well-performing teams when they find a correct solution, whereas the badly-performing teams continue their interaction until the experimenters intervene and stop the activity. Inspecting the distribution of the routines that are established in the common duration, i.e.\ first $\approx 11$ mins, we see that there is a moderate correlation coefficient between the establishment times and \measure{error} ($\rho =0.52$, $p = .15$), neglecting Team 18, which established no routines at all during this period and spoke very little in this common duration. Once we normalise the establishment times by the duration for each team separately, we see that the normalised median establishment times has a positive, medium Spearman's correlation coefficient ($\rho =0.38$, $p = .28$), indicating a general trend that establishments occur earlier for the better-performing teams. Fig.~\ref{fig:h1_1_plot} shows the normalised establishment times.

While it is expected that better-performing teams have established routines, from the figures we observe even badly-performing teams still successfully established routines. All teams, regardless of performance, have aligned to some degree. Focusing on Fig.~\ref{fig:h1_1_plot}, the establishment tends to occur around the middle of the dialogue: establishment times have mean of the medians~$= 63.0\%$ (combined $SD = 22.2\%$). While we hypothesised that establishment will happen early in the dialogue, this is the case for an ideal dialogue; people will `share' expressions earlier. However, we observe that there is an \emph{exploratory} period (roughly the period before Q1), where the interlocutors take the time to understand the task, followed by a \emph{collaborative} period that corresponds to the establishment period (roughly the period between Q1 and Q3). We expect that if the interlocutors had to complete the task again, the establishment/collaborative period would be closer to the start of the dialogue.

We observe that five teams (7, 8, 10, 18, and 47) that could not find a correct solution started collaborating later in their dialogue, in terms of when they establish most of their routines (median establishment time~$> 60\%$). Though the measures of task performance would only reflect that these teams performed badly with a final overall score of performance, our alignment measures reflect details of the performance. Interlocutors are gently reminded a few minutes before the end of the task the remaining time, but were not rushed to find a solution: which could have changed the way they aligned by forcing an establishment period. Thus, we observe through our alignment measures that badly performing teams were simply slower to collaborate and establish routines. 

Two teams have established routines later in their dialogue: Team 17 that found a correct solution, and Team 18 that could not (their median establishment times are around 70\%). Yet, 17 has a focused establishment period (with a smaller IQR $= 18\%$ vs.\ $30\%$ of the time, respectively, see Fig.~\ref{fig:h1_1_plot}). We interpret that Team 17 was able to turn it around and find a correct solution, while Team 18 did not; ending up as the worst performing team. 17 has positive learning gain (\measure{learn} = 25\%), while it is negative for Team 18 (\measure{learn} = -56\%, the highest decrease among the transcribed teams, see Fig.~\ref{fig:transcribed_scatter}). While bad performance could be reflected through a collaborative period starting later in their dialogue (such as Team 18; with later establishment, and not finding a solution in time), Team 17 shows that there are exceptions to this. Team 18 also possibly got confused, reflected in the high and negative \measure{learn}.

The collaborative and exploratory periods can also be observed by examining the error progression of teams' submitted solutions during the task, as shown in Fig.~\ref{fig:h1_1_plot}. During the exploratory period, Nine out of ten teams had their highest error. For teams that performed well, their collaborative period had their lowest error before finding an optimal solution (thus ending the task), and for other teams; their closest solution to the optimal solution. There are 8 such teams that exhibit this behaviour. The teams that did not achieve a correct solution, never regressed to their largest error from the exploratory period. Looking at the number of attempts, for the well-performing teams, their collaborative period was productively used, with their next solution reaching an optimal cost (Teams 17 and 28), or one more attempt before their optimal cost (Team 20). Several teams that did not perform well have a greater number of attempts submitted after their collaborative period (Teams 9, 7, 8, 10, 47). Their submission pattern of attempts indicate a ``trial-and-error" strategy on how to solve the task, for example, Teams 8 and 9 increasing their submissions after their collaborative period, or Teams 7, 10 and 47 submitting throughout.

\paragraph{For learning outcomes.}
The distribution of the median establishment times are not statistically significantly different for teams with positive learning outcomes (Teams 7, 9, 10, 11, 17) vs.\ others (Teams 8, 18, 20, 28, 47) by Kruskal-Wallis H test ($H = 0.88$, $p = .35$ for times in absolute values, and $H = 0.10$, $p = .75$ for normalised times).

\paragraph{Synopsis.}
Overall, the results support H1.1 for task performance, while they are inconclusive for learning outcomes. Surprisingly, we see that all teams, regardless of task success, are (lexically) aligned to some degree. Thus, inspecting the distributions of the establishment times together with their proposed solutions gave further insight into the collaboration processes, specifically revealing a ``collaborative period" that most of the teams came up with their best solutions. This captures some patterns of alignment that might have otherwise been overlooked.

\subsubsection*{H1.2: Hesitation phenomena are more likely to occur in the vicinity of priming and establishment of task-specific referents for more successful teams.} \label{subsec:results_h1_2}

We consider hesitation phenomena as cued by the presence of a filler, and thus investigate how are the fillers distributed as compared to the priming and establishment of the routines. The results for Mann-Whitney U test and effect size as estimated by Cliff's Delta ($\delta$) are given in Table~\ref{tab:filler_priming_establishment}. $\delta$ ranges from $-1$ to $1$, where $0$ would indicate that the group distributions overlap completely; whereas values of $-1$ and $1$ indicate a complete absence of overlap with the groups. For example, $-1$ indicates that all fillers occur before priming times, and $1$ indicates that all fillers occur after priming.


We observe that filler and \textbf{priming times} differ significantly for most of the teams (for eight out of ten teams by Mann-Whitney U test $p < .05$). We see positive $\delta$ values, except for one team. Most teams thus have fillers that occur after priming times. We see that the magnitude of $\delta$ for most teams is large except for Team~7 (excluding Teams 20 and 8 that are not statistically significant)\footnote{The magnitude of Cliff's Delta ($\delta$) can be interpreted by using the thresholds from~\citet{romano_appropriate_2006}, i.e.\ $|\delta|<0.147$ ``negligible", $|\delta|<0.33$ ``small", $|\delta|<0.474$ ``medium", and otherwise ``large".}. We interpret that most fillers do occur visibly after priming times (with little overlap from the large effect sizes). We observe that filler and \textbf{establishment times} differ significantly for most of the teams (for seven out of ten teams by Mann-Whitney U test $p < .05$). We see $\delta$ ranging from $-0.67$ for Team 7, to $0.33$ for Team 11 (though most are negative). However, we see that the magnitude of $\delta$ for most teams is small, with the exception of two teams. This means that the distributions of fillers differ with a small effect size compared to the distributions of establishment times, especially considering that the token number values do not overlap; i.e.\ we do not expect an effect size of $0$. We thus interpret most fillers do occur around (from positive and negative $\delta$ values) establishment times (with larger overlap from small effect sizes).

\begin{table}[tbp]
    \centering
    \caption{The results for the Mann-Whitney U test that compares the distribution of filler times with  establishment and priming times for H1.2. The effect size is estimated by Cliff's Delta ($\delta$). Teams are sorted by decreasing task performance i.e.\ increasing \measure{error}. The horizontal line separates well-performing teams (that found a correct solution) from badly-performing teams. $U$ is the U statistic, and $p$ is the `two-sided' p-value of a Mann-Whitney U test (without continuity correction as there can be no ties, via our unique token number assignment).}
    \label{tab:filler_priming_establishment}
    \footnotesize
    \begin{tabular}{r|rr|rrr|rrr|rrr}
        {} & \multicolumn{2}{c}{count} & \multicolumn{3}{c}{median (\%)} & \multicolumn{3}{c}{priming} & \multicolumn{3}{c}{establishment} \\
        Team & filler & routine &     filler & priming & establishment &       $U$ &        $p$ &      $\delta$ &             $U$ &        $p$ &      $\delta$ \\
        \midrule
        28   &     38 &            58 &       11.6 &     3.5 &          15.2 &  1600.5 &  $< .05$ &   0.45 &         828.5 &  $< .05$ &  -0.25 \\
        17   &     27 &            41 &       14.0 &     6.2 &          17.1 &   823.0 &  $< .05$ &   0.49 &         431.0 &    $.12$ &  -0.22 \\
        20   &     59 &            51 &       20.7 &    18.1 &          22.8 &  1746.5 &    $.15$ &   0.16 &        1139.5 &  $< .05$ &  -0.24 \\ \hline
        11   &     35 &            70 &       34.5 &     3.5 &          24.4 &  2229.0 &  $< .05$ &   0.82 &        1624.0 &  $< .05$ &   0.33 \\
        9    &     81 &           131 &       46.3 &    11.4 &          37.4 &  8805.5 &  $< .05$ &   0.66 &        6561.5 &  $< .05$ &   0.24 \\
        47   &     56 &            74 &       19.5 &     6.7 &          21.9 &  3189.0 &  $< .05$ &   0.54 &        1627.0 &  $< .05$ &  -0.21 \\
        10   &     20 &            65 &       20.1 &     8.7 &          20.4 &   982.0 &  $< .05$ &   0.51 &         660.0 &    $.92$ &   0.02 \\
        8    &     26 &            62 &       19.8 &    15.7 &          36.0 &   883.0 &    $.48$ &   0.10 &         461.0 &  $< .05$ &  -0.43 \\
        7    &     27 &            59 &       24.9 &    25.9 &          37.8 &   562.0 &  $< .05$ &  -0.29 &         259.0 &  $< .05$ &  -0.67 \\
        18   &     52 &            57 &       10.8 &     4.3 &          11.8 &  2136.0 &  $< .05$ &   0.44 &        1326.0 &    $.34$ &  -0.11 \\
                
    \end{tabular}
\end{table}

These results indicate that in the process of routine formation, in between the priming and the establishment of the expression, there seems to be a period in which the interlocutors exhibit hesitation phenomena. This placement of fillers is of interest due to the potentially unfamiliar vocabulary of the task-specific referents that the interlocutors had to utilise in the situated environment. The results demonstrate a lack of hesitation phenomena at the start of the formation of a routine; i.e.\ they occur visibly after the priming of expressions that contain task-specific referents. The large effect size shows that this is predominantly the case for most teams. In addition to this, fillers were found to occur around establishment times. We suggest that a part of establishment is often a clarification request, as shown by the following example. Red indicates the routine expression, while blue indicates the filler.

\begin{idea}
\noindent\textbf{\textit{A}:} \textcolor{red}{\textit{Mount Zurich to Mount Bern}}.
\newline \textbf{\textit{\dots \dots}} 
\newline \textbf{\textit{B}:} \textcolor{blue}{uh} isn't already \textcolor{red}{\textit{Mount Zurich to Mount Bern}} isn't it connected?
\newline \textbf{\textit{\dots \dots}} 
\newline \textbf{\textit{A}:} So if we erase Mount \textcolor{red}{\textit{Zurich}} or Mount Ber- to Mount Bern or Mount \textcolor{red}{\textit{Zurich}} to Mount Gallen?
\newline \textbf{\textit{B}:} Wait \textcolor{blue}{uh} \textcolor{red}{\textit{Zurich}} to Mount \dots ?
\label{quote:clar_req}
\end{idea}

Speakers are able to prime these expressions without exhibiting this hesitation phenomena, but this does not guarantee that the primed expression was fully understood by the listener, as shown by the results of the Mann-Whitney U test. Following the idea of IF and IG pairs in the dialogue, the IG (speaker) tends to be in the abstract view, and can see the minimally represented names of gold mines. They need only concentrate on the gold mines that have the lowest cost to connect. Perhaps the reason why the IG does not exhibit (by our measures) this uncertainty is because they can see the task-specific referents available to them written down on the map. Expressions that contain task-specific referents could successfully become part of the IG's expression lexicon when given these new referents. The IG may also feel at ease to read out these expressions. The IF (listener) must follow the instructions with actions, and since they can not see the cost of adding and removing edges, they must search for the specific gold mine names given by the IG. This could create an uncertainty in the IG, and bring about a need to clarify.

\paragraph{For task performance.}
The distribution of the Cliff's Delta between filler times and both priming or establishment times has a very weak correlation coefficient with \measure{error} (Spearman's $\rho =-0.18$, $p = .62$ for priming, $\rho =0.06$, $p = .88$ for establishment). Therefore, we can not conclude that there is a significant relationship between how early are the priming or establishment times, and how well a team performs.

\paragraph{For learning outcomes.}
The distribution of the Cliff's Delta that quantifies how different are filler times from priming or establishment times are not statistically significantly different for teams with positive learning outcomes (Teams 7, 9, 10, 11, 17) vs.\ others (Teams 8, 18, 20, 28, 47) by Kruskal-Wallis H tests ($H = 1.32$, $p = .25$ for both). Therefore, we can not conclude that a significant difference exists, between how early fillers occur compared to priming (or establishments) between these two learning groups.

\paragraph{Synopsis.}
Regarding H1.2, we can not conclude that the usage of fillers occur in the vicinity of 
priming or establishments times for more successful teams (for neither better-performing teams, nor higher-learning teams). Overall, we see that for most of the teams, the fillers tend to occur visibly after priming times, and around establishment times. We still believe that this gives us a fascinating insight into the way the interlocutors use task-specific expressions in a situated environment.



\section{Studying Behavioural Alignment (RQ2)}
\subsection{Methodology} \label{subsec: studying_RQ2}

% \paragraph*{Detecting follow-up actions of the task-specific referents.} \label{subsec: detecting_follow_up_actions}
If an instruction is verbalised (for e.g.\ to connect ``Mount Basel to Montreux'') by an interlocutor (IG), it could result in an action of connecting the two. We hence say an instruction \emph{match}es an action when the instruction is executed by the other interlocutor (IF) via an action in the situated environment, and within the period of a turn of views before they are swapped. We study the discrepancy created when the IF does not follow the IG, which we call a \emph{mismatch} of instructions-to-actions. In \autoref{eq: justhink2_task}, the instruction (to connect Gallen to Davos) matches the action (connecting these two). In \autoref{eq: mismatch_example}, we illustrate a dialogue excerpt that results in a mismatch:

\begin{idea}
\noindent\textbf{\textit{A}:} What about Mount Davos to Mount, Saint Gallen? \hfill \textit{[Instruction to add an edge from Davos to Gallen.]}
\newline \textbf{\textit{B}:} Because what if, you did if we could do it?
\newline \textbf{\textit{A}:} What about Mount um Davos to Mount Gallen?
\newline \textbf{\textit{B}:} Mount \dots
\newline \textbf{\textit{B}:} {oh} Mount Davos
\newline \textbf{\textit{A}:} yeah to Mount Gallen.
\newline \textbf{\textit{B}:} to Mount Gallen yeah do that.
\newline \textlangle \textit{A} connects Mount Gallen to Mount Davos\textrangle
\newline \textbf{\textit{B}:} Okay my turn.
\hfill \textit{[Match!]}
\label{eq: justhink2_task}
\end{idea}

\begin{idea}
\noindent\textbf{\textit{B}:} Go to Mount Basel. \hfill \textit{[Instruction to add an edge to Basel.]}
\newline \textbf{\textit{A}:} That's, it's expensive.
\newline \textbf{\textit{B}:} Just do it.
\newline \textbf{\textit{A}:} You can't, you can't, I can't because there's a \newline mountain there \dots
\newline \textbf{\textit{A}:} So I'm going, so I'm going here.
\newline \textlangle \textit{A} connects Mount Interlaken to Mount Bern\textrangle \hfill \textit{[Mismatch!]}
\label{eq: mismatch_example}
\end{idea}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figs/schema_justhink.pdf}
    \caption{Schema for the dialogue flow, to annotate behavioural alignment between the interlocutors.}
  \label{fig: schema}
\end{figure}

\paragraph{Recognising Instructions} We firstly extract instructions from the utterances through the interlocutors' use of task-specific referents. 
In the schema as shown in \autoref{fig: schema}, our input consists timestamped dialogue transcripts and action logs. When the input is an utterance, it is processed to infer instructions using entity patterns. To check these entity patters, we employ named-entity recognition (NER) feature of the Python library \href{https://spacy.io/}{spaCy} that performs this entity recognition. We add the node names of the mountains (e.g. ``Montreux''), and also ``verbs''; i.e. ``add'', ``subtract'' \dots. Then, if the input utterance contains our custom entity patters, then we automatically infer instructions from the utterance by joining these entities together. For e.g. the result may be Add(Node{\textsubscript{1},Node{\textsubscript{2}}}), because the interlocutor explicitly said the verb ``add'' and also the names of the mountains. We give the complete algorithm in \autoref{sec: algorithms}.

\begin{table}[tbp]
    \centering
    % \scriptsize
    \footnotesize
    \caption[Output from the algorithm to recognise instructions and detect follow-up actions] {An example from the output of recognising instructions and detecting follow-up actions (by \textsc{Recognise-Instructions} (\autoref{algo: recognise_instructions}) and \textsc{Match-Instructions-To-Actions} (\autoref{algo: match_instructions_actions})), from Team 10. \emph{View} denotes which view the interlocutor is in (refer to \autoref{subsec: activity}), either \emph{abstract} (Ab) or \emph{visual} (V). \emph{Annotations} denotes the automatically inferred instructions and follow-up actions in the activity.
    For example, \emph{Instruct\textsubscript{A}} indicates that interlocutor A has given an instruction to add two nodes (inferred from referents), which can be partially recognised \emph{(Gallen,?)}. As shown, the algorithm builds up (or ``caches'') instructions until an edit action is performed (`\naannotation' in Utt.). Note, since B is in the visual view, their inferred instruction is deliberately not matched.}
    \label{table: algo_results}
    \begin{tabular}{ccccll}
    % \begin{tabular}{c|c|c|c|p{0.25\textwidth}|p{0.35\textwidth}}
          & Utt. & View & Verb & Utterance & Annotations\\
        \cline{1-6}
        \multirow{2}*{A} & \multirow{2}*{198} & \multirow{2}*{Ab} & \multirow{2}*{says} & Maybe we start from, & Instruct\textsubscript{A}(Add(Zermatt,?)) \\
        &&&& Mount Zermatt ? &  \\ 
        % \cline{5-6}
        \multirow{2}*{B} & \multirow{2}*{199} & \multirow{2}*{V} & \multirow{2}*{says} & No lets do Mount Davos to, & {Instruct\textsubscript{A}(Add(Zermatt,?),\\ &&&& &Instruct\textsubscript{B}(Add(Davos,?))
        % \textit{As prev.}
        } \\
        &&&& where do you wanna go? &  \\ 
        % \cline{5-6}
        \multirow{2}*{A} & \multirow{2}*{200} & \multirow{2}*{Ab} & \multirow{2}*{says} & \multirow{2}*{\dots to Mount, St Gallen.} & {Instruct\textsubscript{A}(Add(Zermatt,?),\\ &&&&& Instruct\textsubscript{B}(Add(Davos,?)}, \\
        % {\textit{As prev.} $+$}, \\
        &&&&& \textcolor{blue}{Instruct\textsubscript{A}(Add(Gallen,?))} \\ 
        % \cline{5-6}
        \multirow{1}*{B} & \multirow{1}*{201} & \multirow{1}*{V} & \multirow{1}*{says} & \multirow{1}*{Okay.} & {\textit{As previous}} \\

        % \cline{5-6}
        \multirow{1}*{B} & \multirow{1}*{\naannotation} & \multirow{1}*{V} & \multirow{1}*{adds} & \multirow{1}*{Gallen-Davos} 
        % &  \textcolor{red}{Match\textsubscript{B}}(\textcolor{blue}{Instruct\textsubscript{A}(Add(Gallen, ?))\textcolor{red}{)}} \\
        &  Instruct\textsubscript{A}(Add(Zermatt,?),\\ &&&&& \textcolor{teal}{Match\textsubscript{B}}\\&&&&&\textcolor{blue}{(Instruct\textsubscript{A}(Add(Gallen,?)))}\\
    \end{tabular}
\end{table}

\paragraph{Matching instructions-to-actions} To find (mis)matches of instructions-to-actions, we then follow the logic as given in the schema to determine whether there is an inferred instruction in the instructions list at the time an action was taken. Then, we check whether the action matches or mismatches the inferred instruction.  

In \autoref{eq: justhink2_task}, Gallen-Davos was the result of a negotiation, rather than a complete given instruction by the IG. B says in one utterance ``oh Mount Davos'' and then in another ``to Mount Gallen yeah do that'', resulting in two cached inferred instructions; (Davos,?) and (Gallen,?) respectively. This accounts for some amount of multiple speaker turn\footnote{Note, we specifically use ``speaker turn'' to distinguish from a turn in the collaborative activity; i.e.\ every swapping of views.} negotiations, and possible other ways of referring to task-specific referents (e.g\ ``Now go from \textbf{there} to Davos''). Though an instruction could be carried out after the views swap again, i.e.\ in the following turn, in our methodology, the pending instructions are cleared at every swap (if ``swap or submit'', then ``clear instructions''), resulting sometimes in a \emph{nonmatched} action, or when an action occurred but there was no inferred instruction. A full and concrete example of the added annotations of our automatically inferred instructions-to-actions is given in \autoref{table: algo_results}.


% We extract instructions from the utterances through the interlocutors' use of task-specific referents\footnote{We design \textsc{Recognise-Instructions}, described in Algorithm~\ref{algo:recognise_instructions}, that uses Algorithm~\ref{algo:recognise_entities}, which automatically infers a sequence of instructions from an input utterance, via a rule-based algorithm. Its implementation is available with the tools.} and find (mis)matches of instructions-to-actions\footnote{We design \textsc{Match-Instructions-to-Actions}, described in  Algorithm~\ref{algo:match_instructions_actions}.}\textsuperscript{,}\footnote{In our implementation, we combine the transcripts and the logs (from the dataset at DOI:~\href{\datasetLinkDOI}{\datasetDOI}) via a script (\notebook{tools/5\_construct\_the\_corpus\_by\_combining\_transcripts\_with\_logs.ipynb} in the tools at DOI:~\href{\toolsLinkDOI}{\toolsDOI}) to generate a combined corpus (\folder{processed\_data/corpus/} available with the tools). Then, we process this corpus via a script (\notebook{tools/6\_recognise\_instructions\_detect\_follow-up\_actions.ipynb} in the tools) to generate an annotated corpus (\folder{processed\_data/annotated\_corpus}, available with the tools). The annotated corpus contains the inferred instructions, matches, mismatches, and nonmatches if there were no instructions to be matched.).}. Algorithm~\ref{algo:match_instructions_actions}, that uses Algorithm~\ref{algo:check_match}, accounts for partial matches of nodes, i.e.\ an IG need not explicitly say both node names. It builds up (``caches") pending instructions that have not been followed, clearing them once the views are swapped. The cache of instructions is also cleared if after an edit action a match or mismatch of instructions-to-actions is detected. This allows for matching of negotiated nodes: in Example~\ref{quote:justhink_task}, Gallen-Davos was the result of a negotiation, rather than a complete given instruction by the IG. B says in one utterance ``oh Mount Davos" and then in another ``to Mount Gallen yeah do that", resulting in two cached inferred instructions; (Davos,?) and (Gallen,?) respectively. This accounts for some amount of multiple speaker-turn negotiations, and possible other ways of referring to task-specific referents (e.g\ ``Now go from \textbf{there} to Davos")\footnote{Though an instruction could be carried out after the views swap again, i.e.\ in the following turn: in our algorithm, the pending instructions are cleared at every swap, resulting in a nonmatch.}. See Table~\ref{tab:algo_results} in Sec.~\ref{subsec:results_rq2} for another example.

\paragraph*{Studying when interlocutors are behaviouraly aligned and its association with task success (H2.1).} 
% \label{subsubsec: temporality_of_follow_up_actions}
To investigate H2.1, we compare the distributions of the match and mismatch times of the teams, by following the same methodology stated for H1.1 (which investigated establishment and priming times). In particular, we check if the median match or mismatch times are significantly earlier for better-performing teams by Spearman's rank correlation, and for the two groups of learning, by Kruskal-Wallis H test.

\paragraph*{Studying information management phenomena surrounding behavioural alignment and its association with task success (H2.2).}  
% \label{subsubsec:info_management_phenomena_follow_up_actions}

We consider the use of ``oh'' as an information management marker, to mark a focus of a speaker's attention, which then also becomes a candidate for the listener's attention. This creation of a joint focus of attention allows for transitions in the information state~\citep{schiffrin1987discourse}. In general, changes in the information state -- or what is commonly known about the task -- of the participating interlocutors should be due to physical actions related to the task, particularly because the situated activity has an interdependence on the physical environment. 

``Oh'' as a marker for new information has been studied in various scenarios. \citet{aijmer1987oh} did a corpus analysis of ``oh'' to identify the contexts in which the marker is used, starting from a base general description of its usage as \emph{a mental reaction to a stimulus}; e.g. ``Oh, flowers!''. Among the specific contexts identified, the most relevant to this work is ``oh'' used as a marker to verbalise reactions to \emph{surprising information}. \citet{FOXTREE1999280} also studied the use of ``oh'' in online comprehension experiments to find that it is used by listener's to help them \emph{integrate information} in spontaneous speech. We are interested in the use of ``oh'' in the context of what is commonly known by the interlocutors regarding the task. Thus, we consider the verbalisation of ``oh'', as an update in the interlocutor's knowledge regarding how to solve the situated activity, resulting from actions taken. To the best of our knowledge, the use of `oh'' has been studied more in the context of integrating information at the verbal level, but not a behavioural one.

Thus, an increase in these information management markers associated with the task should lead to an increase in task success. To investigate H2.2, we check if the distributions of (mis)matches and `oh' marker times are significantly different by Mann-Whitney U test, and estimate the effect size by computing Cliff's Delta. This calculation differs from H1.2, as actions are not part of an utterance (compared to establishment time for example); hence we cannot use the order of tokens as was previously used, and instead compare the end times of the utterance that contains the marker with the (mis)matched action times. Then, as H1.2, we calculate the relation to performance and learning.

\subsection{Results}\label{subsec:results_rq2}

\subsubsection*{H2.1: Instructions are more likely to be followed by a corresponding action early in the dialogue for more successful teams.}

To investigate H2.1, we automatically infer (mis)matches\footnote{As described in Algorithm~\ref{algo:match_instructions_actions}. We process this combined dialogue and actions corpus via a script (\notebook{tools/6\_recognise\_instructions\_detect\_follow-up\_actions.ipynb} in the tools) to generate an annotated corpus (\folder{processed\_data/annotated\_corpus}, available with the tools). The annotated corpus contains the inferred instructions, their pending lists used for matching, matches, mismatches, and nonmatches if there were no instructions to be (mis)matched.}, where a verbal instructions' follow-up action is labelled as a (mis)match following the methodology described in Sec.~\ref{subsec:studying_RQ1}. Then, we inspect the distribution of the (mis)matches of the teams, and see how this is related to task success.

\paragraph{For task performance.}
The median match times has a moderate positive correlation coefficient with the task performance measure \measure{error} (Spearman's $\rho = 0.59$, $p = .08$), that is, better-performing teams have matches earlier. This follows the results in H1.1, regarding establishment times. For the matches in the common duration (i.e.\ first $\approx 11$ mins), there is a moderate correlation coefficient ($\rho = 0.45$, $p = .23$, ignoring Team 18 that has no matches in this common period). Fig.~\ref{fig:h2_1_time_absolute_plot} shows the the distribution of the (mis)match times for each team. When the times are normalised by the duration for each team separately, we observe a positive, moderate Spearman's correlation coefficient ($\rho = 0.54$, $p = .11$), that indicates a general trend that matches happen earlier for the better-performing teams.

Fig.~\ref{fig:h2_1_plot} shows for each team, the distribution of the match and mismatch times, normalised by the duration of each team itself. While it is natural to think that instructions will be followed by a match for more successful teams in a structured and organised manner, we observe that teams that performed badly and teams that did not learn also have a certain period of matches. Therefore, all teams, independent of their task success, have their IG's instructions matched to the IF's actions to some extent. Match times have mean of the medians~$= 62.6\%$ (combined $SD = 21.9\%$), and mismatches have mean of medians~$= 67.6\%$ (combined $SD = 26.0\%$).

By inspecting the outputs of the automatically inferred instructions in Table~\ref{tab:algo_results}, occasionally, we see that the traditional roles of IF and IG are not maintained, even for the brief fixed time of views (i.e.\ within a turn). The IF, having just been switched from IG, may have their own ideas about the next best edit action, as seen in Utt.\ no.\ $199$ (prior to  Utt.\ no.\ $198$, the views were swapped, with B being in the abstract view, meaning B was just previously the IG). Thus the interlocutors can also conduct a negotiation where they collaboratively decide which action to take. It is therefore not always the case that the IG is in the abstract view deciding and instructing what the IF in the visual view should do; and this is supported by the frequent swapping of views.

\begin{table}[tbp]
    \centering
    \scriptsize
    \caption{An example from the output of recognising instructions and detecting follow-up actions (by Algorithms~\ref{algo:recognise_instructions} and~\ref{algo:match_instructions_actions}), from Team 10. \textit{View} denotes which view the interlocutor is in (refer to Sec.~\ref{subsec:activity}). \textit{Annotations} denotes the automatically inferred instructions and follow-up actions in the activity.
    For example, \textit{Instruct\textsubscript{A}} indicates that interlocutor A has given an instruction to add two nodes (inferred from referents), which can be partially recognised \textit{(Gallen,?)}. As shown, the algorithm builds up (or ``caches") instructions until an edit action is performed (`\naannotation' in Utt.\ no.). Note, since B is in the visual view his/her inferred instruction is deliberately not matched.}
    \label{tab:algo_results}
    \begin{tabular}{c|c|c|c|l|l}
    % \begin{tabular}{c|c|c|c|p{0.25\textwidth}|p{0.35\textwidth}}
          & Utt. no. & View & Verb & Utterance & Annotations\\
        \cline{1-6}
        \multirow{2}*{A} & \multirow{2}*{198} & \multirow{2}*{Abstract} & \multirow{2}*{says} & Maybe we start from, & Instruct\textsubscript{A}(Add(Zermatt,?)) \\
        &&&& Mount Zermatt ? &  \\ 
        \cline{5-6}
        \multirow{2}*{B} & \multirow{2}*{199} & \multirow{2}*{Visual} & \multirow{2}*{says} & No lets do Mount Davos to, & {Instruct\textsubscript{A}(Add(Zermatt,?), Instruct\textsubscript{B}(Add(Davos,?))
        % \textit{As prev.}
        } \\
        &&&& where do you wanna go? &  \\ 
        \cline{5-6}
        \multirow{2}*{A} & \multirow{2}*{200} & \multirow{2}*{Abstract} & \multirow{2}*{says} & \multirow{2}*{\dots to Mount, St Gallen.} & {Instruct\textsubscript{A}(Add(Zermatt,?), Instruct\textsubscript{B}(Add(Davos,?)}, \\
        % {\textit{As prev.} $+$}, \\
        &&&&& \textcolor{blue}{Instruct\textsubscript{A}(Add(Gallen,?))} \\ 
        \cline{5-6}
        \multirow{1}*{B} & \multirow{1}*{201} & \multirow{1}*{Visual} & \multirow{1}*{says} & \multirow{1}*{Okay.} & {\textit{As previous}} \\

        \cline{5-6}
        \multirow{1}*{B} & \multirow{1}*{\naannotation} & \multirow{1}*{Visual} & \multirow{1}*{adds} & \multirow{1}*{Gallen-Davos} 
        % &  \textcolor{red}{Match\textsubscript{B}}(\textcolor{blue}{Instruct\textsubscript{A}(Add(Gallen, ?))\textcolor{red}{)}} \\
        &  Instruct\textsubscript{A}(Add(Zermatt,?), \textcolor{magenta}{Match\textsubscript{B}}\textcolor{blue}{(Instruct\textsubscript{A}(Add(Gallen,?)))}\\
        \cline{1-6}
    \end{tabular}
\end{table}


\begin{figure}[tbp]
    \centering %  Box and whiskers plots of the
    \includegraphics[width=\linewidth]{figs/h2_1_time_absolute_plot.pdf}
    \caption{The team's match and mismatch times in blue (`$+$') and red (`$\times$') respectively, to study H2.1. The teams are sorted by decreasing learning outcomes (i.e.\ decreasing \measure{learn}). See Fig.~\ref{fig:h1_1_time_absolute_plot} for a description of the green, red and blue lines.} \label{fig:h2_1_time_absolute_plot}
\end{figure}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/h2_1_time_plot.pdf}
    \caption{The teams’ match and mismatch times in green and red respectively, as normalised by the duration for each team separately. Sorting is as in Fig.~\ref{fig:h2_1_time_absolute_plot}.} \label{fig:h2_1_plot}
\end{figure}


\paragraph{For learning outcomes.}
By inspecting the median of the match times with \measure{learn}, we observe that they are not statistically significantly different for teams with positive learning outcomes (Teams 7, 9, 10, 11, 17) vs.\ others (Teams 8, 18, 20, 28, 47) by Kruskal-Wallis H tests ($H = 0.54$, $p = .47$ for times in absolute values, and $H = 0.10$, $p = .75$ for normalised times).

Though not statistically significant by these measures, from the Algorithm~\ref{algo:match_instructions_actions}'s results, we see that all teams have more inferred matches than mismatches (see Table~\ref{tab:oh_match_mismatch} for reference). Teams 18 and 20 that learnt the least, have the highest match-to-mismatch ratio ($3.6$ and $4.0$ matches of instructions-to-actions for every $1$ mismatch respectively.), as well as Team 7 ($3.3$). Teams 8 and 47, which are also amongst the teams that had a negative learning gain (but close to zero, substantially higher than 18 and 20), have lower match-to-mismatch ratio of $2.7$ and $1.3$ respectively. 
% Inspecting Fig.~\ref{fig:transcribed_scatter}, we observe that they are farther away from teams 18 and 20 in terms of \measure{learn}. 
We observe that Teams 10, 11 and 17, who had the highest learning gain, comparatively have a lower ratio of matches-to-mismatches of $2.4$, $1.8$ and $2.3$ respectively. We interpret that it is important for learning that interlocutors have a good ratio of matches-to-mismatches, and not just be in total (blind) agreement with the other. This is consistent with previous research, as stated in Sec.~\ref{subsec:structure}. By just inspecting performance, superficially, Team 20 performed well. However, they did not learn (in fact, ``unlearnt", as shown with a negative learning outcome). Observing their progression of costs for submitted solutions (from $191 \%$, to $109 \%$, to finding an optimal solution) informs us that they ``got lucky" in finding a solution, however did not learn, as is further evidenced by only a few, and sparse mismatched instructions-to-actions. Indeed, before finding an optimal solution, their previous error ($109 \%$) was substantially higher than any other team that performed badly.

From the results, we interpret that positive learning teams seem to have conflict(s) that they resolved collaboratively while building and submitting solutions (and receiving feedback from the robot), whereas the others either had less or unresolved conflicts. By inspecting how the (mis)matches are distributed, and how they are they positioned in relation to the costs of the submitted solutions, we observe nuances of conflicts and their resolutions. For instance, consider a high-learning Team 11. The team began with a high cost ($191\%$, i.e.\ they basically connected everything to each other, with many redundant connections). One interpretation is that they initially misunderstood the goal of the task of connecting the graph minimally\footnote{And are not only exploring the graph to see the costs and available connections, as is evidenced by their following submissions that had again a very high cost ($127\%$), only later decreasing further through several submissions.}. Then, they had many mismatches (``a mismatch period"), which is followed by many matches ending with (at Q3 of matches) their best solution, getting very close ($5\%$, i.e.\ they did not notice that they could replace a particular connection with a better/lower-cost one). Although the team could not find a correct solution, they learnt a lot from this interaction flow. In comparison, Team 20 also started with that high cost of $191\%$. Yet, they could not resolve the conflict, as their (mis)matches did not result in them getting closer to an optimal solution, but rather still keeping to high cost solutions, and repeating these high cost submissions (109\%, i.e. more than double the cost they could make with many redundant connections). Although they found a correct solution next, since they did not have the conflict resolution period that could be cued by (mis)matches, they did not end up learning.

\paragraph{Synopsis.}
We see that all teams have (mis)matches, irrespective of their task success; therefore, it is not necessary to follow-up with an action in order to succeed. In terms of task performance, we observe a general trend that supports the H2.1, i.e.\ better performing teams tend to follow up the instructions with actions (as matches) early overall (the absolute times), as well as in their dialogues (normalised times). For learning, although the general trend is not statistically confirmed, we gained insight into the nuances of the dynamics of interaction: by inspecting the normalised (mis)match time plots alongside with the submission costs. There seems to be conflicts that may be collaboratively resolved and resulted in learning, or may not be resolved and have adverse effects on the learning outcomes.

\subsubsection*{H2.2: When instructions are followed by a corresponding or a different action, the action is more likely to be in the vicinity of information management phenomena for more successful teams.}
% \subsubsection*{H2.2: When instructions are followed by a corresponding or a different action, the action is more likely to be in the vicinity of information management phenomena for more successful teams.}

To investigate H2.2, we consider the distribution of the information management marker `oh' through time\footnote{We note that the `oh' marker occurs 333 times in the transcripts (average per transcript $= 33.3$, $SD = 20.3$). See Table~\ref{tab:oh_match_mismatch} for the number of utterances that contain one or more `oh's for each team.}, in relation to the distribution of matches and mismatches. In particular, we check if the distributions of `oh' times and (mis)matches are significantly different by Mann-Whitney U test, and estimate the effect size by computing Cliff's Delta ($\delta$). The results of the tests for each team are given in Table~\ref{tab:oh_match_mismatch}. Here, $\delta = -1$ would mean that all `oh's occur earlier than (mis)match times, and $1$; that all `oh's occur later\footnote{As H1.2, $\delta$ ranges from  $-1$ to $1$, where $0$ would mean that the group distributions overlap completely; whereas values of $-1$ and $1$ indicate a absence of overlap between the groups. 
% However, due to the difference in calculation of H1.2 and H2.2 (please see Section~\ref{sec:methodology}), the small effect size in H2.1 is less negligible than in H1.1
}. For all teams except one, the value of $\delta$ is negative, indicating that the distribution of `oh' tends to occur earlier than (mis)match times. We observe that `oh' and (mis)match times do not significantly differ for half of the teams (Mann-Whitney U test $p < .05$). We see $\delta$ ranging from $-0.54$ for Team 8, to $0.09$ for Team 11: this indicates that `oh' occurs differently compared to the (mis)match times within the teams. We see that for the teams that had significantly different distributions, the effect size ranges from negligible ($|\delta|<0.147$) to medium ($|\delta|<0.474$), with the exception of Team 8, that has large effect size ($\delta = -0.54$).      

\begin{table}[tbp]
    \centering
    \caption{The results for Mann-Whitney U tests that compare the distribution of information marker (i.e.\ `oh') times, with (mis)match times for H2.2. The effect size estimated by Cliff's Delta ($\delta$). Teams are sorted by decreasing task performance, i.e.\ increasing \measure{error}. $U$ is the U statistic, and $p$ is the `two-sided' p-value of a Mann-Whitney U test (without continuity correction).}
    \label{tab:oh_match_mismatch}
    % \footnotesize
    \small
    \begin{tabular}{r|rrrr|rrr|rrr}
        {} & \multicolumn{4}{c|}{count (number of utterances)} & \multicolumn{3}{c|}{median (\%)} & \multicolumn{3}{c}{(mis)match} \\
        Team &  oh & match & mismatch & match/mism. &         oh & match & mismatch &      $U$ &        $p$ &      $\delta$ \\
        \midrule
        % 10   &  18 &    36 &       15 &       2.4 &       47.6 &  67.3 &     65.3 &          264.0 &  $< .05$ &  -0.42 \\
        % 11   &  15 &    34 &       18 &       1.8 &       57.3 &  59.5 &     38.5 &          427.0 &    $.58$ &   0.09 \\
        % 17   &  20 &    23 &       10 &       2.3 &       61.1 &  61.1 &     69.4 &          318.0 &    $.83$ &  -0.04\\
        % 9    &  29 &    28 &        9 &       3.1 &       42.9 &  59.9 &     70.2 &          429.0 &    $.16$ &  -0.20 \\
        % 7    &  51 &    43 &       13 &       3.3 &       49.7 &  65.5 &     79.7 &          841.0 &  $< .05$ &  -0.41 \\
        % \hline
        % 28   &  24 &    19 &       13 &       1.5 &       61.7 &  62.7 &     73.6 &          344.0 &    $.51$ &  -0.10 \\
        % 8    &  55 &    30 &       11 &       2.7 &       36.3 &  65.3 &     86.3 &          522.0 &  $< .05$ &  -0.54 \\
        % 47   &  29 &    28 &       21 &       1.3 &       53.4 &  56.8 &     75.7 &          488.0 &  $< .05$ &  -0.31 \\
        % 20   &  65 &    24 &        6 &       4.0 &       35.0 &  58.0 &     42.3 &          715.0 &  $< .05$ &  -0.27 \\
        % 18   &  12 &    25 &        7 &       3.6 &       69.6 &  69.5 &     75.0 &          157.0 &    $.36$ &  -0.18\\
        % \hline
        28   &  24 &    19 &       13 &       1.5 &       61.7 &  62.7 &     73.6 &          344.0 &    $.51$ &  -0.10 \\
        17   &  20 &    23 &       10 &       2.3 &       61.1 &  61.1 &     69.4 &          318.0 &    $.83$ &  -0.04\\
        20   &  65 &    24 &        6 &       4.0 &       35.0 &  58.0 &     42.3 &          715.0 &  $< .05$ &  -0.27 \\
        \hline
        11   &  15 &    34 &       18 &       1.8 &       57.3 &  59.5 &     38.5 &          427.0 &    $.58$ &   0.09 \\
        9    &  29 &    28 &        9 &       3.1 &       42.9 &  59.9 &     70.2 &          429.0 &    $.16$ &  -0.20 \\
        47   &  29 &    28 &       21 &       1.3 &       53.4 &  56.8 &     75.7 &          488.0 &  $< .05$ &  -0.31 \\
        10   &  18 &    36 &       15 &       2.4 &       47.6 &  67.3 &     65.3 &          264.0 &  $< .05$ &  -0.42 \\
        8    &  55 &    30 &       11 &       2.7 &       36.3 &  65.3 &     86.3 &          522.0 &  $< .05$ &  -0.54 \\
        7    &  51 &    43 &       13 &       3.3 &       49.7 &  65.5 &     79.7 &          841.0 &  $< .05$ &  -0.41 \\
        18   &  12 &    25 &        7 &       3.6 &       69.6 &  69.5 &     75.0 &          157.0 &    $.36$ &  -0.18
        % \\ \\ \\
        % 10   &  18 &    36 &       12 &       3\phantom{.000} &       47.6 &  67.3 &     67.0 &          242.0 &  $< .05$ &  -0.44 \\
        % 11   &  15 &    32 &       19 &       1.684 &       57.3 &  60.3 &     39.6 &          394.0 &    $.86$ &   0.03 \\
        % 17   &  20 &    21 &       10 &       2.1\phantom{00} &       61.1 &  54.3 &     74.7 &          291.0 &    $.71$ &  -0.06 \\
        % 9    &  29 &    27 &       10 &       2.7\phantom{00} &       42.9 &  60.1 &     69.0 &          429.0 &    $.16$ &  -0.20 \\
        % 7    &  51 &    43 &        8 &       5.375 &       49.7 &  65.5 &     85.0 &          759.0 &  $< .05$ &  -0.42 \\
        % 28   &  24 &    15 &       14 &       1.071 &       61.7 &  62.7 &     74.4 &          296.0 &    $.35$ &  -0.15 \\
        % 8    &  55 &    27 &       11 &       2.454 &       36.3 &  64.3 &     82.7 &          495.0 &  $< .05$ &  -0.53 \\
        % 47   &  29 &    27 &       20 &       1.35\phantom{0} &       53.4 &  59.1 &     66.6 &          479.0 &  $< .05$ &  -0.30 \\
        % 20   &  65 &    23 &        4 &       5.75\phantom{0} &       35.0 &  57.3 &     42.2 &          641.0 &  $< .05$ &  -0.27 \\
        % 18   &  12 &    24 &        6 &       4\phantom{.000} &       69.6 &  70.0 &     73.1 &          149.0 &    $.39$ &  -0.17 \\ 
        % \\ \\
        % \multicolumn{11}{l}{in increasing error order} \\
        % \\
        % 28   &  24 &    15 &       14 &       1.071429 &       61.7 &  62.7 &     74.4 &          296.0 &    $.35$ &  -0.15 \\
        % 17   &  20 &    21 &       10 &       2.1 &       61.1 &  54.3 &     74.7 &          291.0 &    $.71$ &  -0.06 \\
        % 20   &  65 &    23 &        4 &       5.75 &       35.0 &  57.3 &     42.2 &          641.0 &  $< .05$ &  -0.27 \\
        % 11   &  15 &    32 &       19 &       1.68 &       57.3 &  60.3 &     39.6 &          394.0 &    $.86$ &   0.03 \\
        % 9    &  29 &    27 &       10 &       2.7 &       42.9 &  60.1 &     69.0 &          429.0 &    $.16$ &  -0.20 \\
        % 47   &  29 &    27 &       20 &       1.35 &       53.4 &  59.1 &     66.6 &          479.0 &  $< .05$ &  -0.30 \\
        % 10   &  18 &    36 &       12 &       3. &       47.6 &  67.3 &     67.0 &          242.0 &  $< .05$ &  -0.44 \\
        % 8    &  55 &    27 &       11 &       2.45 &       36.3 &  64.3 &     82.7 &          495.0 &  $< .05$ &  -0.53 \\
        % 7    &  51 &    43 &        8 &       5.375 &       49.7 &  65.5 &     85.0 &          759.0 &  $< .05$ &  -0.42 \\
        % 18   &  12 &    24 &        6 &       4. &       69.6 &  70.0 &     73.1 &          149.0 &    $.39$ &  -0.17 \\
    \end{tabular}
\end{table}

\paragraph{For task performance.}
Since the $\delta$ values are varying from being around 0 to negative values (see Table~\ref{tab:oh_match_mismatch}), for all teams except one, oh's occur earlier than (mis)match times. Following this, the $\delta$ values between `oh' times and (mis)match times has a medium negative correlation coefficient with \measure{error} (Spearman's $\rho =-0.53$, $p = .12$). This means that the better the performance, the more the overlap between (mis)match times and `oh's. There is a general trend that for well-performing teams the `oh's occur more in the vicinity of (mis)match times with larger overlap between the two groups, and the badly-performing teams have comparably less overlap. Thus the results support H2.2. 
% , then for badly-performing teams they tend to occur earlier than the (mis)matches (with less and less overlap). 
% However, keeping in mind the negligible to medium $\delta$ values, 
% For most teams, `oh' does occur consistently before the (mis)matched instructions-to-actions (indicated by the negative $\delta$ values, except for one team), 
% just generally with more overlap for better-performing teams, and generally less overlap for worse-performing teams.
% just generally closer for better-performing teams, and generally farther away for worse-performing teams.


\begin{table}[tbp]
    \centering
    \footnotesize
    \caption{% Example utterances 
    Excerpts that contain information management marker `oh' from Team 20, who performed well but did not learn. 
    % We sample utterances from 2 teams at the start and end of the dialogue. 
    % We choose team 17, who had high task success (i.e.\ performed and learnt well), versus team 20, who performed well but did not learn. 
    Annotations could have the pending instructions, and (mis)matched or nonmatched actions.
     Note, \textcolor{blue}{Nonmatch\textsubscript{Interlocutor}} frequently occurs when the interlocutor follows their own intentions, as seen after Utterance 10, \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)), where A connects two nodes (for brevity, nodes given in Utterance column, unless partial (mis)match).
    }
    \label{tab:algo_results_oh_20}
    % \begin{tabular}{c|c|c|l|l}
    \begin{tabular}{P{.02\textwidth}|R{.04\textwidth}|P{0.06\textwidth}|p{.35\textwidth}|p{.4\textwidth}}
        Int. & Utt. & Verb & Utterance & Annotations \\ \hline
        \dots  & \dots  & \dots & \dots & \dots \\
        B & 10 & says & I'm just gonna \dots & \nautterance \\
        A & \nautterance & adds & Luzern-Zermatt & \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)) \\
        A & 11 & says & Uh \dots & \nautterance \\
        A & 12 & says & Uh \dots & \nautterance \\
        B & 13 & says & \textcolor{red}{Oh} there. & \nautterance \\
        A & 14 & says & \textcolor{red}{Oh} two three. & \nautterance \\
        B & 15 & says & \textcolor{red}{Oh} that's what you've been doing this all time. & \nautterance \\
        \dots  & \dots  & \dots & \dots & \dots \\
        % A & \nautterance & adds & Interlaken-Neuchatel &
        % \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)) \\
        % A & 39 & says & \textcolor{red}{Oh} we, \textcolor{red}{oh} wait \textcolor{red}{oh} wait. & \naannotation \\
        % B & 40 & says & Let me see this. & \naannotation \\ 
        % A & \nautterance & adds & Basel-Neuchatel & \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)) \\
        % B & 41 & says & We've got \dots & \naannotation \\ 
        % A & 42 & says & \textcolor{red}{Oh} it's your turn. & \naannotation \\
        % B & 43 & says & \dots um that was quick. & \naannotation  \\      
        % \dots  & \dots  & \dots & \dots & \dots \\
        B & 56 & says & \textcolor{red}{Oh} I think we have to connect all of them. & Instruct\textsubscript{A}(Add(Gallen,?)) \\  
        B & \nautterance & adds & Luzern-Interlaken & % Do\textsubscript{B}(Add),  
        \textcolor{magenta}{Mismatch\textsubscript{B}}(Instruct\textsubscript{A}(Add(Gallen,?))) \\
        % &&&& \textcolor{magenta}{Mismatch\textsubscript{B}}(Instruct\textsubscript{A}(Add(Gallen,?))\textcolor{magenta}{)}\\
        B & \nautterance & adds & Luzern-Zurich & \textcolor{blue}{Nonmatch\textsubscript{B}}(Do\textsubscript{B}(Add)) \\
        A & 57 & says & \textcolor{red}{Oh}. & \naannotation \\
        B & 58 & says & Okay I did some & \multirow[t]{2}{*}{\naannotation}  \\ 
        A & 59 && okay for me.  & \\
        A & \nautterance & adds & Luzern-Davos & \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)) \\
        A & 60 & says & \textcolor{red}{Oh} no. & \naannotation \\
        B & 61 & says & I think we are doing terrible. & \naannotation \\
        \dots & \dots & \dots & \dots & \dots \\
        A & 450 & says & \textcolor{red}{Oh}. & \naannotation  \\ 
        B & 451 & \multirow[t]{2}{*}{says} & 3. & \multirow[t]{2}{*}{\naannotation}  \\ 
        B & 452 && What?  &\\ 
        A & 453 & says & Let me \dots & \naannotation  \\ 
        A & \nautterance & removes & Luzern-Zermatt & \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Remove)) \\
        A & 454 & \multirow[t]{2}{*}{says} & There you go. & \multirow[t]{2}{*}{\naannotation} \\
        A & 455 && What no. & \\
        B & 456 & \multirow[t]{2}{*}{says} & You are erasing my mistake. & \multirow[t]{2}{*}{\naannotation} \\ 
        B & 457 && How dare you. & \\
        \multirow[t]{6}{*}{A} & 458 & \multirow[t]{6}{*}{says} & I know. & \multirow[t]{6}{*}{\naannotation} \\
        & 459 && Wait, what? &\\
        & 460 && Can I get pencil again? &\\
        & 461 && \textcolor{red}{Oh oh}. &\\
        & 462 && \textcolor{red}{Oh}. &\\
        & 463 && Okay. &\\
        B & 464 & says & We messed up again didn't we? & \naannotation \\
        \dots  & \dots  & \dots & \dots & \dots \\ 
        % \bottomrule
        \hline
    \end{tabular}
\end{table}


\begin{table}[tbp]
    \centering
    \footnotesize
    \caption{
    Excerpts that contain information management marker `oh' from Team 17, who had high task success (i.e.\ performed and learnt well). Utt.\ stands for the utterance number, which is not applicable for the edit actions. See the caption of Table~\ref{tab:algo_results_oh_20} for further details.
    % Example utterances that contain information management marker ``oh'' . We sample utterances from 2 teams at the start and end of the dialogue. We choose team 17, who had high task success, versus team 20, who performed well but did not learn. Note, Nonmatch\textsubscript{Int.} frequently occurs when the interlocutor follows their own intentions, as seen in the first utterance given for Team 20, \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}), where A connects two nodes (for brevity, nodes given in Utterance column, unless partial match/mismatch).
    }
    \label{tab:algo_results_oh_17}
    % \begin{tabular}{c|c|c|c|l|l}
    \begin{tabular}{P{.02\textwidth}|R{.04\textwidth}|P{0.06\textwidth}|p{.35\textwidth}|p{.4\textwidth}}
        Int. & Utt. & Verb & Utterance  & Annotations \\ \hline
        \dots & \dots & \dots & \dots & \dots \\
        I & 4 & says & So you only build from something & \naannotation \\
        &&& that is already connected. &\\
        B & 5 & says & \textcolor{red}{Oh}. & \naannotation \\
        A & 6 & says & \textcolor{red}{Oh} okay. & \naannotation \\ 
        B & \nautterance & adds & Zermatt-Davos & \textcolor{blue}{Nonmatch\textsubscript{B}}(Do\textsubscript{B}(Add)) \\
        B & \nautterance & adds & Gallen-Davos & \textcolor{blue}{Nonmatch\textsubscript{B}}(Do\textsubscript{B}(Add)) \\
        A & \nautterance & adds & Zurich-Davos & \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)) \\
        \dots & \dots & \dots & \dots & \dots \\
        B & \nautterance & adds & Basel-Bern & \textcolor{magenta}{Match\textsubscript{B}(}Instruct\textsubscript{A}(Add(Basel,?))) \\
        A & 61 & says & Yeah, and then go to Mount Zurich. & Instruct\textsubscript{A}(Add(Zurich,?)) \\ 
        % \dots & \dots & \dots & \dots & \dots \\
        B & \nautterance & adds & Basel-Zurich & \textcolor{magenta}{Match\textsubscript{B}}(Instruct\textsubscript{A}(Add(Zurich,?))) \\
        \multirow[t]{3}{*}{A} & 62 & \multirow[t]{3}{*}{says} & Yeah. & \naannotation \\ 
         & 63 && \textcolor{red}{Oh} no that costs more. & \\   
         & 64 && uh \dots & \\ 
        B & 65 & says & We should erase it. & \naannotation \\
        \dots & \dots & \dots & \dots & \dots \\ 
        A & 266 & says & Then do Mount Bern to Mount Zermatt. & Instruct\textsubscript{A}(Add(Bern,Zermatt)) \\
        A & 267 & says & Maybe that's better. & \naannotation \\
        B & 268 & says & You can't do that. & \naannotation \\
        A & 269 & says & \textcolor{red}{Oh}. & \naannotation \\
        A & 270 & says & Then do \dots & \naannotation \\
        B & 271 & says & Mount Bern to Mount Interlaken? & Instruct\textsubscript{B}(Add(Bern,Interlaken)) \\
        A & 272 & says & Yeah. & \naannotation \\
        A & 273 & says & I think that's 4 though. & \naannotation \\
        B & \nautterance & adds & Interlaken-Bern & \textcolor{magenta}{Mismatch\textsubscript{B}}(Instruct\textsubscript{A}(Add(Bern,Zermatt))) \\
        A & 274 & says & So don't do that. & \naannotation \\
        B & 275 & says & Is that 4? & \naannotation \\
        A & 276 & says & \textcolor{red}{Oh} yeah it's, it is 4. & \naannotation \\
        \dots & \dots & \dots & \dots & \dots \\
        % \bottomrule
        \hline
    \end{tabular}
\end{table}


\paragraph{For learning outcomes.}
The distribution of the Cliff's Delta, that quantifies how different `oh' times are from (mis)match times, is not statistically significantly different for teams with positive learning outcomes (Teams 7, 9, 10, 11, 17) vs.\ others (Teams 8, 18, 20, 28, 47) by Kruskal-Wallis H test ($H = 0.27$, $p = .60$). 

We see from Table~\ref{tab:oh_match_mismatch} there is a delicate balance between performance and learning. Team 20 for example, performed well but learnt nothing, and differ with statistical significance in their distribution of `oh' versus (mis)match times compared to other better performing teams. For comparison, we thus choose Team 17, who had high task success (i.e.\ performed and learnt well), vs.\ Team 20, who performed well but did not learn, and then we sample utterances from these two teams at the start and end of their dialogue. See Table~\ref{tab:algo_results_oh_20} and Table~\ref{tab:algo_results_oh_17} for excerpts from Teams 20 and 17, respectively. For both teams, we see the first occurrences of `oh' in the tables (corresponding to the exploratory period, from H1.1) and a period of nonmatched instructions for both teams, as they individually figure out the constraints of the task and navigate the situated environment. Keeping in mind the stylistic differences amongst interlocutors (for example, in Team 20 we clearly see that interlocutor A tends to use `oh' frequently), we still see interesting differences between the teams in terms of their usage of `oh's and their instructions-to-actions.

In Team 20 (Utt.\ no.\ $56-61$), we see both interlocutors using `oh' traditionally as an information management marker (e.g.\ ``Oh I think we have to connect all of them"); but from the mismatch/nonmatch of instructions-to-actions, we see that this information state of the interlocutor is not transferred to the collective information state of both interlocutors. Essentially, the interlocutors are working in isolation, individually gaining (perceived) information about the situated environment (measured by use of `oh'), and then following up with their own intentions in isolation (e.g.\ mismatch and nonmatch between utt.\ no.\ 56 and 57). To contrast, we clearly see that Team 17 (Utt.\ no.\ $61-65$) has this transition of information from the interlocutor to the listener with their use of `oh', signalling information in a shared focus of attention (with A saying ``Oh no that costs more" and B responding ``We should erase it"). We see similar patterns of behaviour towards the end of the dialogue (by this point, interlocutors have had opportunity to build a collaboration with each other). 

The intuition behind H2.2 seems reasonable here; Team 20 for example, had 65 occurrences of the information marker `oh', but they significantly differ from the 30 times the instructions given by the IG was (mis)matched by the IF. Interestingly, we observe in the last period for Team 20 a lack of inferred instructions. Inferred instructions are a precursor to an action being (mis)matched or nonmatched. Indeed, there is also a lack of nonmatched actions, which typically occur when the interlocutor takes the liberty to follow their own intentions. Here, they do not even verbalise their own intentions, visible from the lack of inferred instructions. This indicates a strong tendency of working in isolation despite the design of the task.

\paragraph{Synopsis.}
Overall, regardless of a team's task success, we see that `oh' does occur earlier than (mis)matched instructions-to-actions, as evidenced by the negative effect sizes of Cliff's Delta. Specifically for performance, there is a general trend that for well-performing teams the `oh's occur more in the vicinity of (mis)match times with larger overlap between the two groups, and the badly-performing teams have comparably less overlap. This result supports H2.2. While we cannot conclude on the results for learning, using our automatically annotated instructions-to-actions and occurrences of `oh', we still gain some insight into the way the teams collaborate\footnote{Future work could expand more on the inferred instructions and nonmatches and their implications of collaboration, rather than only focusing on (mis)matched actions.}.

==> sections/results.tex <==
\section[Results and Discussion]{Results and Discussion\footnote{The code that reproduces all the results and figures given in this paper are available from the Zenodo Repository, DOI:~\href{https://sandbox.zenodo.org/record/742549}{10.5072/zenodo.742549}}} \label{sec:results}

\subsection{RQ1: How do the interlocutors use task-specific referents? Does this link to task success?} \label{subsec:results_rq1}

\subsubsection*{H1.1: Task-specific referents become routine early for more successful teams.} \label{subsec:results_h1_1}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/h1_1_time_absolute_plot.pdf}
    \caption{The team's establishment times for H1.1. The teams are sorted by decreasing task performance (i.e.\ increasing \measure{error}). The boxplots, with the same colour have the same \measure{error} (sorted by increasing duration for the ties). The thick, bold boxplots with whiskers with maximum 1.5 IQR show the distributions of the establishments that occurred in the common duration (i.e.\ as marked by the dashed green line), while the thin boxplots show the distributions through the total duration of interaction. The learning outcome of each team is indicated with a plus (`+') for $\measure{learn} > 0$, or a minus (`-') otherwise. Solid lines indicate the end of the interaction, by submitting a correct solution (in green) or timing out (in red). The thin blue lines indicate submission of a solution, with the number showing the error quantifying how far the submitted solution is from an optimal solution in terms of its cost (e.g.\ $\measure{error} = 0\%$ means the team has found an optimal solution). The red and blue dots indicate the utterance times of the interlocutors, to give an idea of when the interlocutors are speaking versus when are their establishment times.} \label{fig:h1_1_time_absolute_plot}
\end{figure}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/h1_1_time_plot.pdf}
    \caption{The teams' establishment times as normalised by the duration for each team separately, i.e.\ 100\% indicates the end of that team's interaction. Sorting is as in Fig.~\ref{fig:h1_1_time_absolute_plot}.} \label{fig:h1_1_plot}
\end{figure}

\paragraph{For task performance.}
Fig.~\ref{fig:h1_1_time_absolute_plot} shows for each team the distribution of the establishment times of the routines. The median establishment times for all of the routines is strongly positively correlated with the task performance measure \measure{error} (Spearman's $\rho =0.69$, $p < .05$), that is, better-performing teams establish routines earlier\footnote{The magnitude of Spearman's correlation coefficient ($\rho$) can be interpreted by using the thresholds e.g.\ from~\citet{evans_straightforward_1996}, i.e.\ $0.00-0.19$ ``very weak", $0.20-0.39$ ``weak", $0.40-0.59$ ``moderate", $0.60-0.79$ ``strong", and $0.80-1.00$ ``very strong" \label{foot:spearman_groups}.}. We see from the figure that the results are influenced by the variation in the duration of the activity: the interaction ends for the well-performing teams when they find a correct solution, whereas the badly-performing teams continue their interaction until the experimenters intervene and stop the activity. Inspecting the distribution of the routines that are established in the common duration, i.e.\ first $\approx 11$ mins, we see that there is a moderate correlation coefficient between the establishment times and \measure{error} ($\rho =0.52$, $p = .15$), neglecting Team 18, which established no routines at all during this period and spoke very little in this common duration. Once we normalise the establishment times by the duration for each team separately, we see that the normalised median establishment times has a positive, medium Spearman's correlation coefficient ($\rho =0.38$, $p = .28$), indicating a general trend that establishments occur earlier for the better-performing teams. Fig.~\ref{fig:h1_1_plot} shows the normalised establishment times.

While it is expected that better-performing teams have established routines, from the figures we observe even badly-performing teams still successfully established routines. All teams, regardless of performance, have aligned to some degree. Focusing on Fig.~\ref{fig:h1_1_plot}, the establishment tends to occur around the middle of the dialogue: establishment times have mean of the medians~$= 63.0\%$ (combined $SD = 22.2\%$). While we hypothesised that establishment will happen early in the dialogue, this is the case for an ideal dialogue; people will `share' expressions earlier. However, we observe that there is an \emph{exploratory} period (roughly the period before Q1), where the interlocutors take the time to understand the task, followed by a \emph{collaborative} period that corresponds to the establishment period (roughly the period between Q1 and Q3). We expect that if the interlocutors had to complete the task again, the establishment/collaborative period would be closer to the start of the dialogue.

We observe that five teams (7, 8, 10, 18, and 47) that could not find a correct solution started collaborating later in their dialogue, in terms of when they establish most of their routines (median establishment time~$> 60\%$). Though the measures of task performance would only reflect that these teams performed badly with a final overall score of performance, our alignment measures reflect details of the performance. Interlocutors are gently reminded a few minutes before the end of the task the remaining time, but were not rushed to find a solution: which could have changed the way they aligned by forcing an establishment period. Thus, we observe through our alignment measures that badly performing teams were simply slower to collaborate and establish routines. 

Two teams have established routines later in their dialogue: Team 17 that found a correct solution, and Team 18 that could not (their median establishment times are around 70\%). Yet, 17 has a focused establishment period (with a smaller IQR $= 18\%$ vs.\ $30\%$ of the time, respectively, see Fig.~\ref{fig:h1_1_plot}). We interpret that Team 17 was able to turn it around and find a correct solution, while Team 18 did not; ending up as the worst performing team. 17 has positive learning gain (\measure{learn} = 25\%), while it is negative for Team 18 (\measure{learn} = -56\%, the highest decrease among the transcribed teams, see Fig.~\ref{fig:transcribed_scatter}). While bad performance could be reflected through a collaborative period starting later in their dialogue (such as Team 18; with later establishment, and not finding a solution in time), Team 17 shows that there are exceptions to this. Team 18 also possibly got confused, reflected in the high and negative \measure{learn}.

The collaborative and exploratory periods can also be observed by examining the error progression of teams' submitted solutions during the task, as shown in Fig.~\ref{fig:h1_1_plot}. During the exploratory period, Nine out of ten teams had their highest error. For teams that performed well, their collaborative period had their lowest error before finding an optimal solution (thus ending the task), and for other teams; their closest solution to the optimal solution. There are 8 such teams that exhibit this behaviour. The teams that did not achieve a correct solution, never regressed to their largest error from the exploratory period. Looking at the number of attempts, for the well-performing teams, their collaborative period was productively used, with their next solution reaching an optimal cost (Teams 17 and 28), or one more attempt before their optimal cost (Team 20). Several teams that did not perform well have a greater number of attempts submitted after their collaborative period (Teams 9, 7, 8, 10, 47). Their submission pattern of attempts indicate a ``trial-and-error" strategy on how to solve the task, for example, Teams 8 and 9 increasing their submissions after their collaborative period, or Teams 7, 10 and 47 submitting throughout.

\paragraph{For learning outcomes.}
The distribution of the median establishment times are not statistically significantly different for teams with positive learning outcomes (Teams 7, 9, 10, 11, 17) vs.\ others (Teams 8, 18, 20, 28, 47) by Kruskal-Wallis H test ($H = 0.88$, $p = .35$ for times in absolute values, and $H = 0.10$, $p = .75$ for normalised times).

\paragraph{Synopsis.}
Overall, the results support H1.1 for task performance, while they are inconclusive for learning outcomes. Surprisingly, we see that all teams, regardless of task success, are (lexically) aligned to some degree. Thus, inspecting the distributions of the establishment times together with their proposed solutions gave further insight into the collaboration processes, specifically revealing a ``collaborative period" that most of the teams came up with their best solutions. This captures some patterns of alignment that might have otherwise been overlooked.

\subsubsection*{H1.2: Hesitation phenomena are more likely to occur in the vicinity of priming and establishment of task-specific referents for more successful teams.} \label{subsec:results_h1_2}

We consider hesitation phenomena as cued by the presence of a filler, and thus investigate how are the fillers distributed as compared to the priming and establishment of the routines. The results for Mann-Whitney U test and effect size as estimated by Cliff's Delta ($\delta$) are given in Table~\ref{tab:filler_priming_establishment}. $\delta$ ranges from $-1$ to $1$, where $0$ would indicate that the group distributions overlap completely; whereas values of $-1$ and $1$ indicate a complete absence of overlap with the groups. For example, $-1$ indicates that all fillers occur before priming times, and $1$ indicates that all fillers occur after priming.


We observe that filler and \textbf{priming times} differ significantly for most of the teams (for eight out of ten teams by Mann-Whitney U test $p < .05$). We see positive $\delta$ values, except for one team. Most teams thus have fillers that occur after priming times. We see that the magnitude of $\delta$ for most teams is large except for Team~7 (excluding Teams 20 and 8 that are not statistically significant)\footnote{The magnitude of Cliff's Delta ($\delta$) can be interpreted by using the thresholds from~\citet{romano_appropriate_2006}, i.e.\ $|\delta|<0.147$ ``negligible", $|\delta|<0.33$ ``small", $|\delta|<0.474$ ``medium", and otherwise ``large".}. We interpret that most fillers do occur visibly after priming times (with little overlap from the large effect sizes). We observe that filler and \textbf{establishment times} differ significantly for most of the teams (for seven out of ten teams by Mann-Whitney U test $p < .05$). We see $\delta$ ranging from $-0.67$ for Team 7, to $0.33$ for Team 11 (though most are negative). However, we see that the magnitude of $\delta$ for most teams is small, with the exception of two teams. This means that the distributions of fillers differ with a small effect size compared to the distributions of establishment times, especially considering that the token number values do not overlap; i.e.\ we do not expect an effect size of $0$. We thus interpret most fillers do occur around (from positive and negative $\delta$ values) establishment times (with larger overlap from small effect sizes).

\begin{table}[tbp]
    \centering
    \caption{The results for the Mann-Whitney U test that compares the distribution of filler times with  establishment and priming times for H1.2. The effect size is estimated by Cliff's Delta ($\delta$). Teams are sorted by decreasing task performance i.e.\ increasing \measure{error}. The horizontal line separates well-performing teams (that found a correct solution) from badly-performing teams. $U$ is the U statistic, and $p$ is the `two-sided' p-value of a Mann-Whitney U test (without continuity correction as there can be no ties, via our unique token number assignment).}
    \label{tab:filler_priming_establishment}
    \footnotesize
    \begin{tabular}{r|rr|rrr|rrr|rrr}
        {} & \multicolumn{2}{c}{count} & \multicolumn{3}{c}{median (\%)} & \multicolumn{3}{c}{priming} & \multicolumn{3}{c}{establishment} \\
        Team & filler & routine &     filler & priming & establishment &       $U$ &        $p$ &      $\delta$ &             $U$ &        $p$ &      $\delta$ \\
        \midrule
        28   &     38 &            58 &       11.6 &     3.5 &          15.2 &  1600.5 &  $< .05$ &   0.45 &         828.5 &  $< .05$ &  -0.25 \\
        17   &     27 &            41 &       14.0 &     6.2 &          17.1 &   823.0 &  $< .05$ &   0.49 &         431.0 &    $.12$ &  -0.22 \\
        20   &     59 &            51 &       20.7 &    18.1 &          22.8 &  1746.5 &    $.15$ &   0.16 &        1139.5 &  $< .05$ &  -0.24 \\ \hline
        11   &     35 &            70 &       34.5 &     3.5 &          24.4 &  2229.0 &  $< .05$ &   0.82 &        1624.0 &  $< .05$ &   0.33 \\
        9    &     81 &           131 &       46.3 &    11.4 &          37.4 &  8805.5 &  $< .05$ &   0.66 &        6561.5 &  $< .05$ &   0.24 \\
        47   &     56 &            74 &       19.5 &     6.7 &          21.9 &  3189.0 &  $< .05$ &   0.54 &        1627.0 &  $< .05$ &  -0.21 \\
        10   &     20 &            65 &       20.1 &     8.7 &          20.4 &   982.0 &  $< .05$ &   0.51 &         660.0 &    $.92$ &   0.02 \\
        8    &     26 &            62 &       19.8 &    15.7 &          36.0 &   883.0 &    $.48$ &   0.10 &         461.0 &  $< .05$ &  -0.43 \\
        7    &     27 &            59 &       24.9 &    25.9 &          37.8 &   562.0 &  $< .05$ &  -0.29 &         259.0 &  $< .05$ &  -0.67 \\
        18   &     52 &            57 &       10.8 &     4.3 &          11.8 &  2136.0 &  $< .05$ &   0.44 &        1326.0 &    $.34$ &  -0.11 \\
                
    \end{tabular}
\end{table}

These results indicate that in the process of routine formation, in between the priming and the establishment of the expression, there seems to be a period in which the interlocutors exhibit hesitation phenomena. This placement of fillers is of interest due to the potentially unfamiliar vocabulary of the task-specific referents that the interlocutors had to utilise in the situated environment. The results demonstrate a lack of hesitation phenomena at the start of the formation of a routine; i.e.\ they occur visibly after the priming of expressions that contain task-specific referents. The large effect size shows that this is predominantly the case for most teams. In addition to this, fillers were found to occur around establishment times. We suggest that a part of establishment is often a clarification request, as shown by the following example. Red indicates the routine expression, while blue indicates the filler.

\begin{idea}
\noindent\textbf{\textit{A}:} \textcolor{red}{\textit{Mount Zurich to Mount Bern}}.
\newline \textbf{\textit{\dots \dots}} 
\newline \textbf{\textit{B}:} \textcolor{blue}{uh} isn't already \textcolor{red}{\textit{Mount Zurich to Mount Bern}} isn't it connected?
\newline \textbf{\textit{\dots \dots}} 
\newline \textbf{\textit{A}:} So if we erase Mount \textcolor{red}{\textit{Zurich}} or Mount Ber- to Mount Bern or Mount \textcolor{red}{\textit{Zurich}} to Mount Gallen?
\newline \textbf{\textit{B}:} Wait \textcolor{blue}{uh} \textcolor{red}{\textit{Zurich}} to Mount \dots ?
\label{quote:clar_req}
\end{idea}

Speakers are able to prime these expressions without exhibiting this hesitation phenomena, but this does not guarantee that the primed expression was fully understood by the listener, as shown by the results of the Mann-Whitney U test. Following the idea of IF and IG pairs in the dialogue, the IG (speaker) tends to be in the abstract view, and can see the minimally represented names of gold mines. They need only concentrate on the gold mines that have the lowest cost to connect. Perhaps the reason why the IG does not exhibit (by our measures) this uncertainty is because they can see the task-specific referents available to them written down on the map. Expressions that contain task-specific referents could successfully become part of the IG's expression lexicon when given these new referents. The IG may also feel at ease to read out these expressions. The IF (listener) must follow the instructions with actions, and since they can not see the cost of adding and removing edges, they must search for the specific gold mine names given by the IG. This could create an uncertainty in the IG, and bring about a need to clarify.

\paragraph{For task performance.}
The distribution of the Cliff's Delta between filler times and both priming or establishment times has a very weak correlation coefficient with \measure{error} (Spearman's $\rho =-0.18$, $p = .62$ for priming, $\rho =0.06$, $p = .88$ for establishment). Therefore, we can not conclude that there is a significant relationship between how early are the priming or establishment times, and how well a team performs.

\paragraph{For learning outcomes.}
The distribution of the Cliff's Delta that quantifies how different are filler times from priming or establishment times are not statistically significantly different for teams with positive learning outcomes (Teams 7, 9, 10, 11, 17) vs.\ others (Teams 8, 18, 20, 28, 47) by Kruskal-Wallis H tests ($H = 1.32$, $p = .25$ for both). Therefore, we can not conclude that a significant difference exists, between how early fillers occur compared to priming (or establishments) between these two learning groups.

\paragraph{Synopsis.}
Regarding H1.2, we can not conclude that the usage of fillers occur in the vicinity of 
priming or establishments times for more successful teams (for neither better-performing teams, nor higher-learning teams). Overall, we see that for most of the teams, the fillers tend to occur visibly after priming times, and around establishment times. We still believe that this gives us a fascinating insight into the way the interlocutors use task-specific expressions in a situated environment.

% By inspecting how are the fillers distributed in comparison to establishment times, we see that  \dots.
% Further investigation of comparing the filler distribution with priming times indicate \dots
% when task-specific referents become routine, they are more likely to be surrounded by hesitation phenomena, particularly around establishment times and not around priming times.

\subsection{RQ2: How do the interlocutors follow up the use of task-specific referents with actions? Does this link to task success?}\label{subsec:results_rq2}

\subsubsection*{H2.1: Instructions are more likely to be followed by a corresponding action early in the dialogue for more successful teams.}

To investigate H2.1, we automatically infer (mis)matches\footnote{As described in Algorithm~\ref{algo:match_instructions_actions}. We process this combined dialogue and actions corpus via a script (\notebook{tools/6\_recognise\_instructions\_detect\_follow-up\_actions.ipynb} in the tools) to generate an annotated corpus (\folder{processed\_data/annotated\_corpus}, available with the tools). The annotated corpus contains the inferred instructions, their pending lists used for matching, matches, mismatches, and nonmatches if there were no instructions to be (mis)matched.}, where a verbal instructions' follow-up action is labelled as a (mis)match following the methodology described in Sec.~\ref{subsec:studying_RQ1}. Then, we inspect the distribution of the (mis)matches of the teams, and see how this is related to task success.

\paragraph{For task performance.}
The median match times has a moderate positive correlation coefficient with the task performance measure \measure{error} (Spearman's $\rho = 0.59$, $p = .08$), that is, better-performing teams have matches earlier. This follows the results in H1.1, regarding establishment times. For the matches in the common duration (i.e.\ first $\approx 11$ mins), there is a moderate correlation coefficient ($\rho = 0.45$, $p = .23$, ignoring Team 18 that has no matches in this common period). Fig.~\ref{fig:h2_1_time_absolute_plot} shows the the distribution of the (mis)match times for each team. When the times are normalised by the duration for each team separately, we observe a positive, moderate Spearman's correlation coefficient ($\rho = 0.54$, $p = .11$), that indicates a general trend that matches happen earlier for the better-performing teams.

Fig.~\ref{fig:h2_1_plot} shows for each team, the distribution of the match and mismatch times, normalised by the duration of each team itself. While it is natural to think that instructions will be followed by a match for more successful teams in a structured and organised manner, we observe that teams that performed badly and teams that did not learn also have a certain period of matches. Therefore, all teams, independent of their task success, have their IG's instructions matched to the IF's actions to some extent. Match times have mean of the medians~$= 62.6\%$ (combined $SD = 21.9\%$), and mismatches have mean of medians~$= 67.6\%$ (combined $SD = 26.0\%$).

By inspecting the outputs of the automatically inferred instructions in Table~\ref{tab:algo_results}, occasionally, we see that the traditional roles of IF and IG are not maintained, even for the brief fixed time of views (i.e.\ within a turn). The IF, having just been switched from IG, may have their own ideas about the next best edit action, as seen in Utt.\ no.\ $199$ (prior to  Utt.\ no.\ $198$, the views were swapped, with B being in the abstract view, meaning B was just previously the IG). Thus the interlocutors can also conduct a negotiation where they collaboratively decide which action to take. It is therefore not always the case that the IG is in the abstract view deciding and instructing what the IF in the visual view should do; and this is supported by the frequent swapping of views.

\begin{table}[tbp]
    \centering
    \scriptsize
    \caption{An example from the output of recognising instructions and detecting follow-up actions (by Algorithms~\ref{algo:recognise_instructions} and~\ref{algo:match_instructions_actions}), from Team 10. \textit{View} denotes which view the interlocutor is in (refer to Sec.~\ref{subsec:activity}). \textit{Annotations} denotes the automatically inferred instructions and follow-up actions in the activity.
    For example, \textit{Instruct\textsubscript{A}} indicates that interlocutor A has given an instruction to add two nodes (inferred from referents), which can be partially recognised \textit{(Gallen,?)}. As shown, the algorithm builds up (or ``caches") instructions until an edit action is performed (`\naannotation' in Utt.\ no.). Note, since B is in the visual view his/her inferred instruction is deliberately not matched.}
    \label{tab:algo_results}
    \begin{tabular}{c|c|c|c|l|l}
    % \begin{tabular}{c|c|c|c|p{0.25\textwidth}|p{0.35\textwidth}}
          & Utt. no. & View & Verb & Utterance & Annotations\\
        \cline{1-6}
        \multirow{2}*{A} & \multirow{2}*{198} & \multirow{2}*{Abstract} & \multirow{2}*{says} & Maybe we start from, & Instruct\textsubscript{A}(Add(Zermatt,?)) \\
        &&&& Mount Zermatt ? &  \\ 
        \cline{5-6}
        \multirow{2}*{B} & \multirow{2}*{199} & \multirow{2}*{Visual} & \multirow{2}*{says} & No lets do Mount Davos to, & {Instruct\textsubscript{A}(Add(Zermatt,?), Instruct\textsubscript{B}(Add(Davos,?))
        % \textit{As prev.}
        } \\
        &&&& where do you wanna go? &  \\ 
        \cline{5-6}
        \multirow{2}*{A} & \multirow{2}*{200} & \multirow{2}*{Abstract} & \multirow{2}*{says} & \multirow{2}*{\dots to Mount, St Gallen.} & {Instruct\textsubscript{A}(Add(Zermatt,?), Instruct\textsubscript{B}(Add(Davos,?)}, \\
        % {\textit{As prev.} $+$}, \\
        &&&&& \textcolor{blue}{Instruct\textsubscript{A}(Add(Gallen,?))} \\ 
        \cline{5-6}
        \multirow{1}*{B} & \multirow{1}*{201} & \multirow{1}*{Visual} & \multirow{1}*{says} & \multirow{1}*{Okay.} & {\textit{As previous}} \\

        \cline{5-6}
        \multirow{1}*{B} & \multirow{1}*{\naannotation} & \multirow{1}*{Visual} & \multirow{1}*{adds} & \multirow{1}*{Gallen-Davos} 
        % &  \textcolor{red}{Match\textsubscript{B}}(\textcolor{blue}{Instruct\textsubscript{A}(Add(Gallen, ?))\textcolor{red}{)}} \\
        &  Instruct\textsubscript{A}(Add(Zermatt,?), \textcolor{magenta}{Match\textsubscript{B}}\textcolor{blue}{(Instruct\textsubscript{A}(Add(Gallen,?)))}\\
        \cline{1-6}
    \end{tabular}
\end{table}


\begin{figure}[tbp]
    \centering %  Box and whiskers plots of the
    \includegraphics[width=\linewidth]{figs/h2_1_time_absolute_plot.pdf}
    \caption{The team's match and mismatch times in blue (`$+$') and red (`$\times$') respectively, to study H2.1. The teams are sorted by decreasing learning outcomes (i.e.\ decreasing \measure{learn}). See Fig.~\ref{fig:h1_1_time_absolute_plot} for a description of the green, red and blue lines.} \label{fig:h2_1_time_absolute_plot}
\end{figure}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/h2_1_time_plot.pdf}
    \caption{The teams’ match and mismatch times in green and red respectively, as normalised by the duration for each team separately. Sorting is as in Fig.~\ref{fig:h2_1_time_absolute_plot}.} \label{fig:h2_1_plot}
\end{figure}


\paragraph{For learning outcomes.}
By inspecting the median of the match times with \measure{learn}, we observe that they are not statistically significantly different for teams with positive learning outcomes (Teams 7, 9, 10, 11, 17) vs.\ others (Teams 8, 18, 20, 28, 47) by Kruskal-Wallis H tests ($H = 0.54$, $p = .47$ for times in absolute values, and $H = 0.10$, $p = .75$ for normalised times).

Though not statistically significant by these measures, from the Algorithm~\ref{algo:match_instructions_actions}'s results, we see that all teams have more inferred matches than mismatches (see Table~\ref{tab:oh_match_mismatch} for reference). Teams 18 and 20 that learnt the least, have the highest match-to-mismatch ratio ($3.6$ and $4.0$ matches of instructions-to-actions for every $1$ mismatch respectively.), as well as Team 7 ($3.3$). Teams 8 and 47, which are also amongst the teams that had a negative learning gain (but close to zero, substantially higher than 18 and 20), have lower match-to-mismatch ratio of $2.7$ and $1.3$ respectively. 
% Inspecting Fig.~\ref{fig:transcribed_scatter}, we observe that they are farther away from teams 18 and 20 in terms of \measure{learn}. 
We observe that Teams 10, 11 and 17, who had the highest learning gain, comparatively have a lower ratio of matches-to-mismatches of $2.4$, $1.8$ and $2.3$ respectively. We interpret that it is important for learning that interlocutors have a good ratio of matches-to-mismatches, and not just be in total (blind) agreement with the other. This is consistent with previous research, as stated in Sec.~\ref{subsec:structure}. By just inspecting performance, superficially, Team 20 performed well. However, they did not learn (in fact, ``unlearnt", as shown with a negative learning outcome). Observing their progression of costs for submitted solutions (from $191 \%$, to $109 \%$, to finding an optimal solution) informs us that they ``got lucky" in finding a solution, however did not learn, as is further evidenced by only a few, and sparse mismatched instructions-to-actions. Indeed, before finding an optimal solution, their previous error ($109 \%$) was substantially higher than any other team that performed badly.

From the results, we interpret that positive learning teams seem to have conflict(s) that they resolved collaboratively while building and submitting solutions (and receiving feedback from the robot), whereas the others either had less or unresolved conflicts. By inspecting how the (mis)matches are distributed, and how they are they positioned in relation to the costs of the submitted solutions, we observe nuances of conflicts and their resolutions. For instance, consider a high-learning Team 11. The team began with a high cost ($191\%$, i.e.\ they basically connected everything to each other, with many redundant connections). One interpretation is that they initially misunderstood the goal of the task of connecting the graph minimally\footnote{And are not only exploring the graph to see the costs and available connections, as is evidenced by their following submissions that had again a very high cost ($127\%$), only later decreasing further through several submissions.}. Then, they had many mismatches (``a mismatch period"), which is followed by many matches ending with (at Q3 of matches) their best solution, getting very close ($5\%$, i.e.\ they did not notice that they could replace a particular connection with a better/lower-cost one). Although the team could not find a correct solution, they learnt a lot from this interaction flow. In comparison, Team 20 also started with that high cost of $191\%$. Yet, they could not resolve the conflict, as their (mis)matches did not result in them getting closer to an optimal solution, but rather still keeping to high cost solutions, and repeating these high cost submissions (109\%, i.e. more than double the cost they could make with many redundant connections). Although they found a correct solution next, since they did not have the conflict resolution period that could be cued by (mis)matches, they did not end up learning.

\paragraph{Synopsis.}
We see that all teams have (mis)matches, irrespective of their task success; therefore, it is not necessary to follow-up with an action in order to succeed. In terms of task performance, we observe a general trend that supports the H2.1, i.e.\ better performing teams tend to follow up the instructions with actions (as matches) early overall (the absolute times), as well as in their dialogues (normalised times). For learning, although the general trend is not statistically confirmed, we gained insight into the nuances of the dynamics of interaction: by inspecting the normalised (mis)match time plots alongside with the submission costs. There seems to be conflicts that may be collaboratively resolved and resulted in learning, or may not be resolved and have adverse effects on the learning outcomes.

\subsubsection*{H2.2: When instructions are followed by a corresponding or a different action, the action is more likely to be in the vicinity of information management phenomena for more successful teams.}
% \subsubsection*{H2.2: When instructions are followed by a corresponding or a different action, the action is more likely to be in the vicinity of information management phenomena for more successful teams.}

To investigate H2.2, we consider the distribution of the information management marker `oh' through time\footnote{We note that the `oh' marker occurs 333 times in the transcripts (average per transcript $= 33.3$, $SD = 20.3$). See Table~\ref{tab:oh_match_mismatch} for the number of utterances that contain one or more `oh's for each team.}, in relation to the distribution of matches and mismatches. In particular, we check if the distributions of `oh' times and (mis)matches are significantly different by Mann-Whitney U test, and estimate the effect size by computing Cliff's Delta ($\delta$). The results of the tests for each team are given in Table~\ref{tab:oh_match_mismatch}. Here, $\delta = -1$ would mean that all `oh's occur earlier than (mis)match times, and $1$; that all `oh's occur later\footnote{As H1.2, $\delta$ ranges from  $-1$ to $1$, where $0$ would mean that the group distributions overlap completely; whereas values of $-1$ and $1$ indicate a absence of overlap between the groups. 
% However, due to the difference in calculation of H1.2 and H2.2 (please see Section~\ref{sec:methodology}), the small effect size in H2.1 is less negligible than in H1.1
}. For all teams except one, the value of $\delta$ is negative, indicating that the distribution of `oh' tends to occur earlier than (mis)match times. We observe that `oh' and (mis)match times do not significantly differ for half of the teams (Mann-Whitney U test $p < .05$). We see $\delta$ ranging from $-0.54$ for Team 8, to $0.09$ for Team 11: this indicates that `oh' occurs differently compared to the (mis)match times within the teams. We see that for the teams that had significantly different distributions, the effect size ranges from negligible ($|\delta|<0.147$) to medium ($|\delta|<0.474$), with the exception of Team 8, that has large effect size ($\delta = -0.54$).      

\begin{table}[tbp]
    \centering
    \caption{The results for Mann-Whitney U tests that compare the distribution of information marker (i.e.\ `oh') times, with (mis)match times for H2.2. The effect size estimated by Cliff's Delta ($\delta$). Teams are sorted by decreasing task performance, i.e.\ increasing \measure{error}. $U$ is the U statistic, and $p$ is the `two-sided' p-value of a Mann-Whitney U test (without continuity correction).}
    \label{tab:oh_match_mismatch}
    % \footnotesize
    \small
    \begin{tabular}{r|rrrr|rrr|rrr}
        {} & \multicolumn{4}{c|}{count (number of utterances)} & \multicolumn{3}{c|}{median (\%)} & \multicolumn{3}{c}{(mis)match} \\
        Team &  oh & match & mismatch & match/mism. &         oh & match & mismatch &      $U$ &        $p$ &      $\delta$ \\
        \midrule
        % 10   &  18 &    36 &       15 &       2.4 &       47.6 &  67.3 &     65.3 &          264.0 &  $< .05$ &  -0.42 \\
        % 11   &  15 &    34 &       18 &       1.8 &       57.3 &  59.5 &     38.5 &          427.0 &    $.58$ &   0.09 \\
        % 17   &  20 &    23 &       10 &       2.3 &       61.1 &  61.1 &     69.4 &          318.0 &    $.83$ &  -0.04\\
        % 9    &  29 &    28 &        9 &       3.1 &       42.9 &  59.9 &     70.2 &          429.0 &    $.16$ &  -0.20 \\
        % 7    &  51 &    43 &       13 &       3.3 &       49.7 &  65.5 &     79.7 &          841.0 &  $< .05$ &  -0.41 \\
        % \hline
        % 28   &  24 &    19 &       13 &       1.5 &       61.7 &  62.7 &     73.6 &          344.0 &    $.51$ &  -0.10 \\
        % 8    &  55 &    30 &       11 &       2.7 &       36.3 &  65.3 &     86.3 &          522.0 &  $< .05$ &  -0.54 \\
        % 47   &  29 &    28 &       21 &       1.3 &       53.4 &  56.8 &     75.7 &          488.0 &  $< .05$ &  -0.31 \\
        % 20   &  65 &    24 &        6 &       4.0 &       35.0 &  58.0 &     42.3 &          715.0 &  $< .05$ &  -0.27 \\
        % 18   &  12 &    25 &        7 &       3.6 &       69.6 &  69.5 &     75.0 &          157.0 &    $.36$ &  -0.18\\
        % \hline
        28   &  24 &    19 &       13 &       1.5 &       61.7 &  62.7 &     73.6 &          344.0 &    $.51$ &  -0.10 \\
        17   &  20 &    23 &       10 &       2.3 &       61.1 &  61.1 &     69.4 &          318.0 &    $.83$ &  -0.04\\
        20   &  65 &    24 &        6 &       4.0 &       35.0 &  58.0 &     42.3 &          715.0 &  $< .05$ &  -0.27 \\
        \hline
        11   &  15 &    34 &       18 &       1.8 &       57.3 &  59.5 &     38.5 &          427.0 &    $.58$ &   0.09 \\
        9    &  29 &    28 &        9 &       3.1 &       42.9 &  59.9 &     70.2 &          429.0 &    $.16$ &  -0.20 \\
        47   &  29 &    28 &       21 &       1.3 &       53.4 &  56.8 &     75.7 &          488.0 &  $< .05$ &  -0.31 \\
        10   &  18 &    36 &       15 &       2.4 &       47.6 &  67.3 &     65.3 &          264.0 &  $< .05$ &  -0.42 \\
        8    &  55 &    30 &       11 &       2.7 &       36.3 &  65.3 &     86.3 &          522.0 &  $< .05$ &  -0.54 \\
        7    &  51 &    43 &       13 &       3.3 &       49.7 &  65.5 &     79.7 &          841.0 &  $< .05$ &  -0.41 \\
        18   &  12 &    25 &        7 &       3.6 &       69.6 &  69.5 &     75.0 &          157.0 &    $.36$ &  -0.18
        % \\ \\ \\
        % 10   &  18 &    36 &       12 &       3\phantom{.000} &       47.6 &  67.3 &     67.0 &          242.0 &  $< .05$ &  -0.44 \\
        % 11   &  15 &    32 &       19 &       1.684 &       57.3 &  60.3 &     39.6 &          394.0 &    $.86$ &   0.03 \\
        % 17   &  20 &    21 &       10 &       2.1\phantom{00} &       61.1 &  54.3 &     74.7 &          291.0 &    $.71$ &  -0.06 \\
        % 9    &  29 &    27 &       10 &       2.7\phantom{00} &       42.9 &  60.1 &     69.0 &          429.0 &    $.16$ &  -0.20 \\
        % 7    &  51 &    43 &        8 &       5.375 &       49.7 &  65.5 &     85.0 &          759.0 &  $< .05$ &  -0.42 \\
        % 28   &  24 &    15 &       14 &       1.071 &       61.7 &  62.7 &     74.4 &          296.0 &    $.35$ &  -0.15 \\
        % 8    &  55 &    27 &       11 &       2.454 &       36.3 &  64.3 &     82.7 &          495.0 &  $< .05$ &  -0.53 \\
        % 47   &  29 &    27 &       20 &       1.35\phantom{0} &       53.4 &  59.1 &     66.6 &          479.0 &  $< .05$ &  -0.30 \\
        % 20   &  65 &    23 &        4 &       5.75\phantom{0} &       35.0 &  57.3 &     42.2 &          641.0 &  $< .05$ &  -0.27 \\
        % 18   &  12 &    24 &        6 &       4\phantom{.000} &       69.6 &  70.0 &     73.1 &          149.0 &    $.39$ &  -0.17 \\ 
        % \\ \\
        % \multicolumn{11}{l}{in increasing error order} \\
        % \\
        % 28   &  24 &    15 &       14 &       1.071429 &       61.7 &  62.7 &     74.4 &          296.0 &    $.35$ &  -0.15 \\
        % 17   &  20 &    21 &       10 &       2.1 &       61.1 &  54.3 &     74.7 &          291.0 &    $.71$ &  -0.06 \\
        % 20   &  65 &    23 &        4 &       5.75 &       35.0 &  57.3 &     42.2 &          641.0 &  $< .05$ &  -0.27 \\
        % 11   &  15 &    32 &       19 &       1.68 &       57.3 &  60.3 &     39.6 &          394.0 &    $.86$ &   0.03 \\
        % 9    &  29 &    27 &       10 &       2.7 &       42.9 &  60.1 &     69.0 &          429.0 &    $.16$ &  -0.20 \\
        % 47   &  29 &    27 &       20 &       1.35 &       53.4 &  59.1 &     66.6 &          479.0 &  $< .05$ &  -0.30 \\
        % 10   &  18 &    36 &       12 &       3. &       47.6 &  67.3 &     67.0 &          242.0 &  $< .05$ &  -0.44 \\
        % 8    &  55 &    27 &       11 &       2.45 &       36.3 &  64.3 &     82.7 &          495.0 &  $< .05$ &  -0.53 \\
        % 7    &  51 &    43 &        8 &       5.375 &       49.7 &  65.5 &     85.0 &          759.0 &  $< .05$ &  -0.42 \\
        % 18   &  12 &    24 &        6 &       4. &       69.6 &  70.0 &     73.1 &          149.0 &    $.39$ &  -0.17 \\
    \end{tabular}
\end{table}

\paragraph{For task performance.}
Since the $\delta$ values are varying from being around 0 to negative values (see Table~\ref{tab:oh_match_mismatch}), for all teams except one, oh's occur earlier than (mis)match times. Following this, the $\delta$ values between `oh' times and (mis)match times has a medium negative correlation coefficient with \measure{error} (Spearman's $\rho =-0.53$, $p = .12$). This means that the better the performance, the more the overlap between (mis)match times and `oh's. There is a general trend that for well-performing teams the `oh's occur more in the vicinity of (mis)match times with larger overlap between the two groups, and the badly-performing teams have comparably less overlap. Thus the results support H2.2. 
% , then for badly-performing teams they tend to occur earlier than the (mis)matches (with less and less overlap). 
% However, keeping in mind the negligible to medium $\delta$ values, 
% For most teams, `oh' does occur consistently before the (mis)matched instructions-to-actions (indicated by the negative $\delta$ values, except for one team), 
% just generally with more overlap for better-performing teams, and generally less overlap for worse-performing teams.
% just generally closer for better-performing teams, and generally farther away for worse-performing teams.


\begin{table}[tbp]
    \centering
    \footnotesize
    \caption{% Example utterances 
    Excerpts that contain information management marker `oh' from Team 20, who performed well but did not learn. 
    % We sample utterances from 2 teams at the start and end of the dialogue. 
    % We choose team 17, who had high task success (i.e.\ performed and learnt well), versus team 20, who performed well but did not learn. 
    Annotations could have the pending instructions, and (mis)matched or nonmatched actions.
     Note, \textcolor{blue}{Nonmatch\textsubscript{Interlocutor}} frequently occurs when the interlocutor follows their own intentions, as seen after Utterance 10, \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)), where A connects two nodes (for brevity, nodes given in Utterance column, unless partial (mis)match).
    }
    \label{tab:algo_results_oh_20}
    % \begin{tabular}{c|c|c|l|l}
    \begin{tabular}{P{.02\textwidth}|R{.04\textwidth}|P{0.06\textwidth}|p{.35\textwidth}|p{.4\textwidth}}
        Int. & Utt. & Verb & Utterance & Annotations \\ \hline
        \dots  & \dots  & \dots & \dots & \dots \\
        B & 10 & says & I'm just gonna \dots & \nautterance \\
        A & \nautterance & adds & Luzern-Zermatt & \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)) \\
        A & 11 & says & Uh \dots & \nautterance \\
        A & 12 & says & Uh \dots & \nautterance \\
        B & 13 & says & \textcolor{red}{Oh} there. & \nautterance \\
        A & 14 & says & \textcolor{red}{Oh} two three. & \nautterance \\
        B & 15 & says & \textcolor{red}{Oh} that's what you've been doing this all time. & \nautterance \\
        \dots  & \dots  & \dots & \dots & \dots \\
        % A & \nautterance & adds & Interlaken-Neuchatel &
        % \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)) \\
        % A & 39 & says & \textcolor{red}{Oh} we, \textcolor{red}{oh} wait \textcolor{red}{oh} wait. & \naannotation \\
        % B & 40 & says & Let me see this. & \naannotation \\ 
        % A & \nautterance & adds & Basel-Neuchatel & \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)) \\
        % B & 41 & says & We've got \dots & \naannotation \\ 
        % A & 42 & says & \textcolor{red}{Oh} it's your turn. & \naannotation \\
        % B & 43 & says & \dots um that was quick. & \naannotation  \\      
        % \dots  & \dots  & \dots & \dots & \dots \\
        B & 56 & says & \textcolor{red}{Oh} I think we have to connect all of them. & Instruct\textsubscript{A}(Add(Gallen,?)) \\  
        B & \nautterance & adds & Luzern-Interlaken & % Do\textsubscript{B}(Add),  
        \textcolor{magenta}{Mismatch\textsubscript{B}}(Instruct\textsubscript{A}(Add(Gallen,?))) \\
        % &&&& \textcolor{magenta}{Mismatch\textsubscript{B}}(Instruct\textsubscript{A}(Add(Gallen,?))\textcolor{magenta}{)}\\
        B & \nautterance & adds & Luzern-Zurich & \textcolor{blue}{Nonmatch\textsubscript{B}}(Do\textsubscript{B}(Add)) \\
        A & 57 & says & \textcolor{red}{Oh}. & \naannotation \\
        B & 58 & says & Okay I did some & \multirow[t]{2}{*}{\naannotation}  \\ 
        A & 59 && okay for me.  & \\
        A & \nautterance & adds & Luzern-Davos & \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)) \\
        A & 60 & says & \textcolor{red}{Oh} no. & \naannotation \\
        B & 61 & says & I think we are doing terrible. & \naannotation \\
        \dots & \dots & \dots & \dots & \dots \\
        A & 450 & says & \textcolor{red}{Oh}. & \naannotation  \\ 
        B & 451 & \multirow[t]{2}{*}{says} & 3. & \multirow[t]{2}{*}{\naannotation}  \\ 
        B & 452 && What?  &\\ 
        A & 453 & says & Let me \dots & \naannotation  \\ 
        A & \nautterance & removes & Luzern-Zermatt & \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Remove)) \\
        A & 454 & \multirow[t]{2}{*}{says} & There you go. & \multirow[t]{2}{*}{\naannotation} \\
        A & 455 && What no. & \\
        B & 456 & \multirow[t]{2}{*}{says} & You are erasing my mistake. & \multirow[t]{2}{*}{\naannotation} \\ 
        B & 457 && How dare you. & \\
        \multirow[t]{6}{*}{A} & 458 & \multirow[t]{6}{*}{says} & I know. & \multirow[t]{6}{*}{\naannotation} \\
        & 459 && Wait, what? &\\
        & 460 && Can I get pencil again? &\\
        & 461 && \textcolor{red}{Oh oh}. &\\
        & 462 && \textcolor{red}{Oh}. &\\
        & 463 && Okay. &\\
        B & 464 & says & We messed up again didn't we? & \naannotation \\
        \dots  & \dots  & \dots & \dots & \dots \\ 
        % \bottomrule
        \hline
    \end{tabular}
\end{table}


\begin{table}[tbp]
    \centering
    \footnotesize
    \caption{
    Excerpts that contain information management marker `oh' from Team 17, who had high task success (i.e.\ performed and learnt well). Utt.\ stands for the utterance number, which is not applicable for the edit actions. See the caption of Table~\ref{tab:algo_results_oh_20} for further details.
    % Example utterances that contain information management marker ``oh'' . We sample utterances from 2 teams at the start and end of the dialogue. We choose team 17, who had high task success, versus team 20, who performed well but did not learn. Note, Nonmatch\textsubscript{Int.} frequently occurs when the interlocutor follows their own intentions, as seen in the first utterance given for Team 20, \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}), where A connects two nodes (for brevity, nodes given in Utterance column, unless partial match/mismatch).
    }
    \label{tab:algo_results_oh_17}
    % \begin{tabular}{c|c|c|c|l|l}
    \begin{tabular}{P{.02\textwidth}|R{.04\textwidth}|P{0.06\textwidth}|p{.35\textwidth}|p{.4\textwidth}}
        Int. & Utt. & Verb & Utterance  & Annotations \\ \hline
        \dots & \dots & \dots & \dots & \dots \\
        I & 4 & says & So you only build from something & \naannotation \\
        &&& that is already connected. &\\
        B & 5 & says & \textcolor{red}{Oh}. & \naannotation \\
        A & 6 & says & \textcolor{red}{Oh} okay. & \naannotation \\ 
        B & \nautterance & adds & Zermatt-Davos & \textcolor{blue}{Nonmatch\textsubscript{B}}(Do\textsubscript{B}(Add)) \\
        B & \nautterance & adds & Gallen-Davos & \textcolor{blue}{Nonmatch\textsubscript{B}}(Do\textsubscript{B}(Add)) \\
        A & \nautterance & adds & Zurich-Davos & \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)) \\
        \dots & \dots & \dots & \dots & \dots \\
        B & \nautterance & adds & Basel-Bern & \textcolor{magenta}{Match\textsubscript{B}(}Instruct\textsubscript{A}(Add(Basel,?))) \\
        A & 61 & says & Yeah, and then go to Mount Zurich. & Instruct\textsubscript{A}(Add(Zurich,?)) \\ 
        % \dots & \dots & \dots & \dots & \dots \\
        B & \nautterance & adds & Basel-Zurich & \textcolor{magenta}{Match\textsubscript{B}}(Instruct\textsubscript{A}(Add(Zurich,?))) \\
        \multirow[t]{3}{*}{A} & 62 & \multirow[t]{3}{*}{says} & Yeah. & \naannotation \\ 
         & 63 && \textcolor{red}{Oh} no that costs more. & \\   
         & 64 && uh \dots & \\ 
        B & 65 & says & We should erase it. & \naannotation \\
        \dots & \dots & \dots & \dots & \dots \\ 
        A & 266 & says & Then do Mount Bern to Mount Zermatt. & Instruct\textsubscript{A}(Add(Bern,Zermatt)) \\
        A & 267 & says & Maybe that's better. & \naannotation \\
        B & 268 & says & You can't do that. & \naannotation \\
        A & 269 & says & \textcolor{red}{Oh}. & \naannotation \\
        A & 270 & says & Then do \dots & \naannotation \\
        B & 271 & says & Mount Bern to Mount Interlaken? & Instruct\textsubscript{B}(Add(Bern,Interlaken)) \\
        A & 272 & says & Yeah. & \naannotation \\
        A & 273 & says & I think that's 4 though. & \naannotation \\
        B & \nautterance & adds & Interlaken-Bern & \textcolor{magenta}{Mismatch\textsubscript{B}}(Instruct\textsubscript{A}(Add(Bern,Zermatt))) \\
        A & 274 & says & So don't do that. & \naannotation \\
        B & 275 & says & Is that 4? & \naannotation \\
        A & 276 & says & \textcolor{red}{Oh} yeah it's, it is 4. & \naannotation \\
        \dots & \dots & \dots & \dots & \dots \\
        % \bottomrule
        \hline
    \end{tabular}
\end{table}


\paragraph{For learning outcomes.}
The distribution of the Cliff's Delta, that quantifies how different `oh' times are from (mis)match times, is not statistically significantly different for teams with positive learning outcomes (Teams 7, 9, 10, 11, 17) vs.\ others (Teams 8, 18, 20, 28, 47) by Kruskal-Wallis H test ($H = 0.27$, $p = .60$). 

We see from Table~\ref{tab:oh_match_mismatch} there is a delicate balance between performance and learning. Team 20 for example, performed well but learnt nothing, and differ with statistical significance in their distribution of `oh' versus (mis)match times compared to other better performing teams. For comparison, we thus choose Team 17, who had high task success (i.e.\ performed and learnt well), vs.\ Team 20, who performed well but did not learn, and then we sample utterances from these two teams at the start and end of their dialogue. See Table~\ref{tab:algo_results_oh_20} and Table~\ref{tab:algo_results_oh_17} for excerpts from Teams 20 and 17, respectively. For both teams, we see the first occurrences of `oh' in the tables (corresponding to the exploratory period, from H1.1) and a period of nonmatched instructions for both teams, as they individually figure out the constraints of the task and navigate the situated environment. Keeping in mind the stylistic differences amongst interlocutors (for example, in Team 20 we clearly see that interlocutor A tends to use `oh' frequently), we still see interesting differences between the teams in terms of their usage of `oh's and their instructions-to-actions.

In Team 20 (Utt.\ no.\ $56-61$), we see both interlocutors using `oh' traditionally as an information management marker (e.g.\ ``Oh I think we have to connect all of them"); but from the mismatch/nonmatch of instructions-to-actions, we see that this information state of the interlocutor is not transferred to the collective information state of both interlocutors. Essentially, the interlocutors are working in isolation, individually gaining (perceived) information about the situated environment (measured by use of `oh'), and then following up with their own intentions in isolation (e.g.\ mismatch and nonmatch between utt.\ no.\ 56 and 57). To contrast, we clearly see that Team 17 (Utt.\ no.\ $61-65$) has this transition of information from the interlocutor to the listener with their use of `oh', signalling information in a shared focus of attention (with A saying ``Oh no that costs more" and B responding ``We should erase it"). We see similar patterns of behaviour towards the end of the dialogue (by this point, interlocutors have had opportunity to build a collaboration with each other). 

The intuition behind H2.2 seems reasonable here; Team 20 for example, had 65 occurrences of the information marker `oh', but they significantly differ from the 30 times the instructions given by the IG was (mis)matched by the IF. Interestingly, we observe in the last period for Team 20 a lack of inferred instructions. Inferred instructions are a precursor to an action being (mis)matched or nonmatched. Indeed, there is also a lack of nonmatched actions, which typically occur when the interlocutor takes the liberty to follow their own intentions. Here, they do not even verbalise their own intentions, visible from the lack of inferred instructions. This indicates a strong tendency of working in isolation despite the design of the task.

\paragraph{Synopsis.}
Overall, regardless of a team's task success, we see that `oh' does occur earlier than (mis)matched instructions-to-actions, as evidenced by the negative effect sizes of Cliff's Delta. Specifically for performance, there is a general trend that for well-performing teams the `oh's occur more in the vicinity of (mis)match times with larger overlap between the two groups, and the badly-performing teams have comparably less overlap. This result supports H2.2. While we cannot conclude on the results for learning, using our automatically annotated instructions-to-actions and occurrences of `oh', we still gain some insight into the way the teams collaborate\footnote{Future work could expand more on the inferred instructions and nonmatches and their implications of collaboration, rather than only focusing on (mis)matched actions.}.

==> sections/revised/related_work_papers.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% (not necessarily alignment) expand verbal analysis (automatic coding schemas) of dialogue in an educational context 
\section{Related Work Papers} \label{sec: related_work_papers}
Mostly verbatim from abstract (or here and there).

\subsection{Verbal analysis of dialogue in educational contexts} \label{subsec: verbal_analysis_papers}
% Reviewer 1: ``The review of verbal analysis of collaborative learning, with the associated claim that coding is still basically only manual, is too restrictive. Some methods for automatically coding educational dialogue in collaborative scenarios do exist (e.g., text analyses of online collaborative learning scenarios, speech and text analysis of classroom discussions and of student-social robot dialogues) and a review of this literature should be included. 
% Some researchers to start with might include Erin Walker, Carolyn Rose, Sidney D’Mello, and Kristy Boyer. As for examining both dialogue and learning outcomes at the same time, I suggest the authors review the tutorial dialogue literature."

\subsubsection{Related Reviews (mostly by other authors)}

\paragraph{Computer Supported Collaborative Learning and Intelligent Tutoring Systems \citep{tchounikine_computer_2010}}
\begin{enumerate}
    \item Three ``hot" CSCL research topics are used as examples: analyzing individual’s and group’s interactions, providing students with adaptive intelligent support, and providing students with adaptive technological means.
    \item In CSCL, interaction analysis refers to analyzing what students are doing as they communicate and collaborate with one another, at a relatively fine-grain level.
    \item  ARGUNAUT system provides the teachers with online, automated feedback regarding important aspects and characteristics of each discussion, explicitly focusing attention on events or situations that may require the teacher's intervention or support. The key idea is to analyze student contributions and e-discussions using machine learning, shallow text processing \citep{rose_analyzing_2008}, and case-based graph matching (McLaren 2003). 
    \item \citet{rose_analyzing_2008} did interaction analysis research to the work described above; in fact, they developed the text analysis tool, \textbf{TagHelper}. Rose and colleagues originally intended to assist coders in analyzing protocols after the fact; but, \dots
    \item \citet{kumar_tutorial_2007} have focused on providing real-time support to dyads collaborating on a problem-solving task: they describe an evaluation of a simple but fully-automatic approach to adaptive collaborative learning support. 
    \item \citet{donmez_supporting_2005} automate the application of a well established collaborative learning process analysis coding scheme~\citep{weinberger_framework_2006}, and demonstrate that patterns that indicate trouble in collaborative discourse can be detected with a high degree of reliability, and thus that a more dynamic support approach for collaborative learning is feasible.
\end{enumerate}

% \paragraph{Adaptive and Intelligent Systems for Collaborative Learning Support: A Review of the Field \citep{magnisalis_adaptive_2011}}

% \paragraph{Tutorial dialogue as adaptive collaborative learning support \citep{kumar_tutorial_2007}}

% Though for argumentation, they review nicely topics in automated analyses in "discussion analyses"; dstinct/separate from "argument analyses" (out of our scope)
\paragraph{Computer-supported argumentation: A review of the state of the art \citep{scheuer_computer-supported_2010}}
\begin{enumerate}
    \item Discussion analyses:
    \begin{enumerate}
        \item Discussion process: System analyzes the discussion process and automatically codes contributions (and more complex interaction patterns), for instance, with dialogue acts. [Epsilon \citep{goodman_using_2005}, ARGUNAUT \citep{de_groot_computer_2007,mclaren_supporting_2010}, Group Leader Tutor \citep{israel_supporting_2007}, \citep{rose_analyzing_2008}]
        \item Discussion topics: System identifies specific contents (i.e., topics) discussed. [Epsilon, Pedabot, ~\citep{kumar_tutorial_2007}]
        \item Problems while discussing: System detects possible problems in the students’ interaction. [Epsilon \citep{goodman_using_2005}, ARGUNAUT \citep{de_groot_computer_2007,mclaren_supporting_2010}, \citep{ravi_profiling_2007}]
        \item Student and group models: System aggregates and classifies student behavior over a period of time in student and group models. [Epsilon \citep{goodman_using_2005}, Group Leader Tutor \citep{israel_supporting_2007}]
        \item Discussion phases: System classifies the current process state and phase according to a hypothesized theoretical model. [Group Leader Tutor \citep{israel_supporting_2007}]
\end{enumerate}
\end{enumerate}


\paragraph{International Handbook of Computer-Supported Collaborative Learning \citep{cress_international_2021}}
Summary of the handbook: \citep{cress_foundations_2021} (its first chapter)

\paragraph{Artifact Analysis \citep{trausan-matu_artifact_2021} (in \cite{cress_international_2021})}
% For any given learning context, the produced artifacts such as spoken or written words and physical interactions e.g.\ gaze or gestures can serve as a basis for assessment, to evaluate interventions and inform an understanding of the learning processes~\citep{trausan-matu_artifact_2021}.
\begin{enumerate}
    \item ``a short review of relevant theoretical perspectives and prior research and describes different forms of language and text artifact analysis that are presently applied within the learning sciences."
    \item ``These include dialog analysis; conversation analysis; content analysis of verbal, textual, and other forms of data; social network analysis; and polyphonic analysis."
    \item ``Applications to the analysis of online discussions and classroom discourse are discussed, as well as future directions for research."
    \item ``\dots content-based approaches should be combined with process-based analytics to enhance the quality and scope of analytic approaches for CSCL."
    \item their classification according to communication media with three categories: \romannumeral 1)~spoken or written words (i.e.\ speech or text-based artifacts), \romannumeral 2)~physical interactions (e.g.\ gestures or gaze % —see Schneider et al. this volume),
    and \romannumeral 3)~digital artifacts (e.g., sequences of interactions) % —see Halatchliyski et al. 2014)
\end{enumerate}


\paragraph{Quantitative Approaches to Language in CSCL \citep{borge_quantitative_2021}}
\begin{enumerate}
    \item ``provide a survey of language quantification practices in CSCL"
    \item ``provide a review of articles published in IJCSCL from 2006 to 2018 to provide the reader with an understanding of who is quantifying language, in what contexts, how they are quantifying it, and for what purpose"
    language quantification is ``conceptualized as the quantification of verbal or written communications between individuals from video, audio, or online chat or textual data for the purpose of measuring, comparing, or describing patterns in language or language-dependent activities. This quantification can be accomplished through frequency counts, an analysis of when in time events occurred, statistical analysis, or computational modeling practices."
    \item ``Both quantitative and qualitative researchers can quantify language. Quantitative researchers may quantify language as a means to look for mathematical patterns, whereas qualitative researchers may quantify language as a means to select representative data or look for cultural patterns."
    \item ``As a measurement tool, quantification becomes an end in itself as researchers quantify language for the purpose of creating new methods for evaluating collaborative interactions or learning outcomes."
    \item ``As a pattern recognition tool, quantification becomes a means to an end. Quantification can be used to identify common trends and problems that occur during collaboration or associations between specific language patterns and their impact on learning processes and outcomes."
    \item ``As a descriptive tool, quantification can help to unpack important activity to help us develop a deeper understanding of it."

\end{enumerate}

\paragraph{Educational dialogues and computer supported collaborative learning: critical analysis and research perspectives \citep{baker_educational_2021}}
\begin{enumerate}
    \item (An interesting critique, maybe see if we could get something), with sections like: (Educational) dialogue: a brief yet in-depth discussion of foundational issues; Thinking in and through dialogue \dots
    \item ``Our main conclusion is thus that it would be fruitful for research to develop approaches that deal with multiple levels involved in a CSCL environment that are based on digital platforms and have educational dialogues as the analytic unit to be understand and explained."
\end{enumerate}


\subsubsection{Sidney D’Mello}

%%%%%%%%%% Overview/Introduction to D'Mello's work [OVERVIEW] 
\paragraph{An overview of dialog-based intelligent tutoring systems (ITSs): Design of Dialog-Based Intelligent Tutoring Systems to Simulate Human-to-Human Tutoring \citep{dmello_design_2013}}
\begin{enumerate}
    \item They give \emph{an analysis of human–human tutorial dialogs} followed with a discussion of the six major components of most dialog-based ITSs: input transformation, speech-act classification, learner modeling, dialog management, output rendering, and domain modeling.
    \item These abstract components are concretized within the context of one of the first dialog-based ITSs, \textbf{AutoTutor}. 
    \item We conclude the chapter by discussing some of the open issues in dialog-based ITSs, such as identifying benefits of spoken versus typed input, understanding when imperfect natural-language understanding is sufficient \dots
    \item One class of technologies that would benefit from natural-language interactions is intelligent tutoring. Intelligent tutoring systems (ITSs) mimic one-on-one human tutoring, a proven method for promoting active construction of knowledge beyond textbooks and traditional classroom environments (Graesser et al. 2009a; VanLehn 2011; Woolf 2009).
    \item ITSs are effective in promoting learning because they are continually assessing learner knowledge and tailoring the instruction in a manner that is sensitive to individual learners.
    \item This chapter discusses a subset of ITSs that implement natural-language dialogs that mimic conversations found in human tutoring.
    \item These computer tutors vary in the extent to which they simulate human dialog mechanisms, \emph{but all of them attempt to comprehend natural language}, formulate adaptive responses, and implement pedagogical strategies to facilitate learning
    \item Major Components of Dialog-Based ITSs
    \begin{enumerate}
        \item ``\textbf{Input Transformation}: transforms learners' responses into a form that can be interpreted by the ITS. ITSs that process spoken input \citep{dmello_toward_2010,litman_spoken_2004} need an additional step of translating learner speech into text via automatic speech recognition."
        \item ``\textbf{Speech Act Classification}: In most cases, learners' responses primarily consist of answers to questions posed by the tutor. 
        These responses (called contributions) have substantive content potentially relevant to the answer and therefore are analyzed in the subsequent learner modeling"
        learners occasionally provide content-free frozen expressions that signify particular discourse functions. These might include conversational acknowledgements (e.g., “ok”), short responses (e.g., “yes,” “no”), metacognitive statements (e.g., “I need help,” “I don’t know”), metacommunicative statements (e.g., “please repeat,” “could you say that in another way”),"
        \item ``\textbf{Learner Modeling}: Modeling at a \textbf{local level} involves comparing learners' immediate contribution to the expected answer (i.e., a specific keyword or phrase). Learner modeling at the \textbf{global level} consists of assessing the learners' evolution of knowledge of the topic being tutored. 
        Modeling at both levels might also involve comparing the extent to which learners' responses align with specific misconceptions, so that these might be immediately or eventually corrected. Many ITSs in well-defined domains like mathematics use some form of Bayesian knowledge tracing (Conati et al. 2002; Corbett and Anderson 1994) for learner modeling; the task is considerably more difficult for dialog-based ITSs in ill-defined domains. We have addressed the problem of modeling learner knowledge in certain ill-defined domains with semantic processing algorithms."
        \item Dialog Management
        \item Output Rendering
    \end{enumerate}
\end{enumerate}

\paragraph{Toward Spoken Human–Computer Tutorial Dialogues \citep{dmello_toward_2010}}
\begin{enumerate}
    \item Oral discourse is the primary form of human–human communication, hence, computer interfaces that communicate via unstructured spoken dialogues will presumably provide a more efficient, meaningful, and naturalistic interaction experience.
    \item Within the context of learning environments, there are theoretical positions supporting a speech facilitation hypothesis that predicts that spoken tutorial dialogues will increase learning more than typed dialogues.
    \item We evaluated this hypothesis in an experiment where 24 participants learned computer literacy via a spoken and a typed conversation with AutoTutor, an intelligent tutoring system with conversational dialogues. 
    \item The results indicated that (a) enhanced content coverage was achieved in the spoken condition; (b) learning gains for both modalities were on par and greater than a no-instruction control; (c) although speech recognition errors were unrelated to learning gains, they were linked to participants’ evaluations of the tutor; (d) participants adjusted their conversational styles when speaking compared to typing; (e) semantic and statistical natural language understanding approaches to comprehending learners’ responses were more resilient to speech recognition errors than syntactic and symbolic-based approaches; and (f) simulated speech recognition errors had differential impacts on the fidelity of different semantic algorithms.
    
    %%% Background
    \item One class of technologies that might greatly benefit from spoken input is intelligent tutoring systems (ITSs). These systems mimic one-on-one human tutoring, which is a powerful method of promoting active construction of knowledge beyond textbooks and traditional classroom environments (Bloom, 1984; P. Cohen, Kulik, \& Kulik, 1982; Corbett, 2002; VanLehn, 2006). 
    
    \item There is the question of determining the appropriate level to analyze spoken utterances when the utterances are confounded with ASR errors.  
    \textbf{shallow and deep NLU}, which are the two broad categories of models that interpret a user’s utterance. Unlike deep NLU, shallow NLU techniques do not perform a thorough linguistic analysis of the user’s utterance. Shallow NLU relies on techniques such as keyword matching, matching decomposed morphemes, regular expressions, simple rule-based grammars, ngrams, and statistical approaches to semantics, syntax, and world knowledge (Jurafsky \& Martin, 2008; Landauer, McNamara, Dennis, \& Kintsch, 2007).

    In contrast, deep NLU approaches attempt to achieve a precise, complete, well-formed analysis of the syntax, semantics, and discourse. Deep NLU requires computational linguistic tools such as syntactic parsers, part-of-speech taggers, morphological transducers, lemmatizers, reference resolution, semantic decomposition, and sometimes discourse analyzers (Jurafsky \& Martin, 2008). These algorithms work best when the utterance is syntactically intact, a feat that is exceedingly difficult to achieve in spoken conversations because of the disfluencies, hesitations, and perturbations that routinely accompany natural speech (Levinson, 1983; Lickley, 1994; Shriberg, 1994).
    Imperfect ASR systems undoubtedly add to the degraded quality of learners’ speech. Therefore, it is conceivable that ASR errors may severely impact the function- ality of deep NLU systems. Although shallow NLU modules may conceivably be resilient to ASR errors, the ASR system must have a modicum of accuracy. But the degree of errors that can be tolerated before the interaction is compromised is an important, yet open research question.
\end{enumerate}

%%%%%%%%%% Updated new recent works that automate
\paragraph{I Say, You Say, We Say: Using Spoken Language to Model Socio-Cognitive Processes during Computer-Supported Collaborative Problem Solving \citep{stewart_i_2019}}
\begin{enumerate}
    \item We investigate automated detection of three critical CPS process – construction of shared knowledge, negotiation/coordination, and maintaining team function – derived from a validated CPS framework. 
    \item Our data consists of 32 triads who were tasked with collaboratively solving a challenging visual computer programming task for 20 minutes using commercial videoconferencing software.
    \item We used automatic speech recognition to generate transcripts of 11,163 utterances, which trained humans coded for evidence of the above three CPS processes using a set of behavioral indicators. 
    \item We aimed to automate the trained human-raters' codes in a team-independent fashion (current study) in order to provide automatic real-time or offline feedback (future work).
    \item We used Random Forest classifiers trained on the words themselves (bag of n-grams) or with word categories (e.g., emotions, thinking styles, social constructs) from the Linguistic Inquiry Word Count (LIWC) tool. 
    \item Results: Despite imperfect automatic speech recognition, the n-gram models achieved AUROC (area under the receiver operating characteristic curve) scores of .85, .77, and .77 for construction of shared knowledge, negotiation/coordination, and maintaining team function, respectively; these reflect 70\%, 54\%, and 54\% improvements over chance
    \item  Further, the LIWC model-derived scores predicted CPS outcomes more similar to human codes, \textbf{demonstrating predictive validity}. 
    We discuss embedding our models in collaborative interfaces \item{for assessment and dynamic intervention} aimed at improving CPS outcomes. 
\end{enumerate}

\paragraph{Say What? Automatic Modeling of Collaborative Problem Solving Skills from Student Speech in the Wild \citep{pugh_say_2021}}
\begin{enumerate}
    \item We investigated the feasibility of using automatic speech recognition (ASR) and natural language processing (NLP) to classify collaborative problem solving (CPS) skills from recorded speech in noisy environments
    \item We analyzed data from 44 dyads of middle and high school students who used videoconferencing to collaboratively solve physics and math problems
    \item Trained coders identified seven cognitive and social CPS skills (e.g., sharing information) in 8,660 utterances. 
    \item We used a state-of-the-art deep transfer learning approach for NLP, Bidirectional Encoder Representations from Transformers (BERT), with a special input representation enabling the model to analyze adjacent utterances for contextual cues. % We adopted a supervised classification approach to predict the ground truth CPS skill for each utterance.  Random Forest N-Grams
    \item Our findings suggest that despite significant speech recognition error in school environments, it is possible to predict expert-coded CPS skills using automatically generated transcripts. 
    (We achieved a micro-average AUROC score (across seven CPS skills) of .80 using ASR transcripts, compared to .91 for human transcripts, indicating a decrease in performance attributable to ASR error)
\end{enumerate}

\paragraph{Multimodal modeling of collaborative problem‐solving facets in triads \citep{stewart_multimodal_2021}}
\begin{enumerate}
    \item We build automated detectors of three critical CPS facets—construction of shared knowledge, negotiation and coordination, and maintaining team function—derived from a validated CPS framework. 
    \item We used data of 32 triads who collaborated via a commercial videoconferencing software, to solve challenging problems in a visual programming task. 
    \item We generated transcripts of 11,163 utterances using automatic speech recognition, which were then coded by trained humans for evidence of the three CPS facets. 
    \item We used both standard and deep sequential learning classifiers to model the human-coded facets from linguistic, task context, facial expressions, and acoustic–prosodic features in a team-independent fashion.
    \item There were no advantages of deep sequential learning methods over standard classifiers. 
    \item Overall, Random Forest classifiers using language and task context features performed best, achieving AUROC scores of .86, .78, and .79 for construction of shared knowledge, negotiation/coordination, and maintaining team function, respectively. 
\end{enumerate}



\subsubsection{Carolyn Rose}

Works of Carolyn on automated collaborative process analysis \citep{rose_analyzing_2008,mu_acodea_2012,gweon_measuring_2013}

\paragraph{Analyzing collaborative learning processes automatically: Exploiting the advances of computational linguistics in computer-supported collaborative learning \citep{rose_analyzing_2008}}
\begin{enumerate}
    \item ``We describe the emerging area of text classification research focused on the problem of collaborative learning process analysis"
    \item ``[W]e report on an interdisciplinary research project, which has been investigating the effectiveness of applying text classification technology to a large CSCL corpus that has been analyzed by human coders using a theory-based multi-dimensional coding scheme."
    \item ``One major technical contribution of this work is a demonstration that an important piece of the work towards making text classification technology effective for this purpose is designing and building linguistic pattern detectors, otherwise known as features, that can be extracted reliably from texts and that have high predictive power for the categories of discourse actions that the CSCL community is interested in."
    \item ``we report on an interdisciplinary research project, which has been investigating the effectiveness of applying text classification technology to a large CSCL corpus that has been analyzed by human coders using a theory-based multi-dimensional coding scheme" from  \citep{weinberger_framework_2006}
    \item ``making text classification technology effective for this purpose is designing and building linguistic pattern detectors, otherwise known as features, that can be extracted reliably from texts and that have high predictive power for the categories of discourse actions that the CSCL community is interested in"
    \item used ``pre-segmented discourse material, i.e., the smallest units to be coded on the seven dimensions were still identified by human analysts"
     one of the most challenging aspects of the~\citet{weinberger_framework_2006} coding scheme, both for human annotation and automatic annotation, is the type of fine-grained segmentation
\end{enumerate}

\paragraph{The ACODEA framework: Developing segmentation and classification schemes for fully automatic analysis of online discussions \citep{mu_acodea_2012}}
\begin{enumerate}
    \item We present a framework for developing coding schemes optimized for automatic segmentation and context-independent coding that builds on this segmentation. 
    \item The key idea is to extract the semantic and syntactic features of each single word by using the techniques of part-of-speech tagging and named-entity recognition before the raw data can be segmented and classified. 
    \item Our results show that the coding on the micro-argumentation dimension can be fully automated.
    \item Finally, we discuss how fully automated analysis can enable context-sensitive support for collaborative learning.
\end{enumerate}

\paragraph{Measuring prevalence of other-oriented transactive contributions using an automated measure of speech style accommodation \citep{gweon_measuring_2013}}
\begin{enumerate}
    \item This paper contributes to a theory-grounded methodological foundation for automatic collaborative learning process analysis. 
    \item It does this by illustrating how insights from the social psychology and sociolinguistics of speech style provide a theoretical framework to inform the design of a computational model. 
    \item The purpose of that model is to detect prevalence of an important group knowledge integration process in raw speech data.
    \item Specifically, this paper focuses on assessment of transactivity in dyadic discussions, where a transactive contribution is operationalized as one where reasoning is made explicit, and where that reasoning builds on a prior reasoning statement within the discussion. 
    \item An unsupervised Dynamic Bayesian Network model motivated by concepts from Speech Accommodation Theory is presented and then evaluated on the task of estimating prevalence of other-oriented transacts in dyadic discussions. 
    \item The evaluation demonstrates a significant positive correlation between an automatic measure of speech style accommodation and prevalence of other-oriented transacts.
\end{enumerate}

\paragraph{Exploring the Effect of Student Confusion in Massive Open Online Courses \citep{yang_exploring_2016}}
% Also conference version: \citep{yang_exploring_2015}
\begin{enumerate}
    \item ``automatically estimate students' confusion by looking at their clicking behavior on course content and participation in the course discussion forums"
    \item ``created a human annotated corpus to develop an automated measurement of student confusion"
    a forum-level confusion classifier, a machine learning model that predicts confusion trained on a human-annotated sample of forum post: ... we extract the input features both from students’ click behaviors and their posting behaviors, including clicking patterns in courses, presence of domain-specific content words, and high-level linguistic features."
\end{enumerate}

\paragraph{Modeling Dialogue Acts with Content Word Filtering and Speaker Preferences \citep{jo_modeling_2017}}
\begin{enumerate}
    \item ``present an unsupervised model of dialogue act sequences in conversation"
    \item ``By modeling topical themes as transitioning more slowly than dialogue acts in conversation, our model de-emphasizes content-related words in order to focus on conversational function words that signal dialogue acts."
    \item They compare with \citep{ezen-can_understanding_2015} that uses Markov Random Field as their unsupervised model. (+2 others that are based on Hidden Markov Models)
\end{enumerate}

\paragraph{Towards Careful Practices for Automated Linguistic Analysis of Group Learning \citep{howley_towards_2016}}
\begin{enumerate}
    \item This paper reviews work in progress towards bridging the field of linguistics and its operationalizations of discourse, and that of frameworks for studying collaborative learning that are rooted directly in the learning sciences.
    \item  We begin with the vision of a multi-dimensional coding and counting analysis approach that might serve as a boundary object between the variety of methodological approaches to analysis of collaborative learning that exist within the Learning Sciences. 
    \item  We outline what we have discovered from a combination of hand coding, comparison with alternative analytic approaches including network analytic and qualitative approaches, correlational analyses in connection with learning-relevant extralinguistic variables, and computational modeling.
    \item We explore both the contribution of work to date as well as the many remaining challenges.
\end{enumerate}




\subsubsection{Erin Walker}

\paragraph{Using Problem-Solving Context to Assess Help Quality in Computer-Mediated Peer Tutoring \citep{walker_using_2010}}

\paragraph{Using Automated Dialog Analysis to Assess Peer Tutoring and Trigger Effective Support \citep{walker_using_2011}}
\begin{enumerate}
    \item ``One of the main challenges in automated support for collaboration is the machine classification of dialogue, giving the system an ability to know when and how to intervene."
    \item ``We have developed an automated detector of conceptual content that is used as a basis for providing adaptive prompts to peer tutors in high-school algebra."
    \item ``We conducted an after-school study with 61 participants where we compared this adaptive support to two non-adaptive support conditions, and found that adaptive prompts significantly increased conceptual help and peer tutor domain learning."
    \item ``The amount of conceptual help students gave, as determined by either human coding or machine classification, was predictive of learning."
    \item ``Thus, machine classification was effective both as a basis for feedback and predictor of success."
\end{enumerate}

% \paragraph{Modeling Helping Behavior in an Intelligent Tutor for Peer Tutoring \citep{walker_modeling_2009}} 
% \begin{enumerate}
%     \item ``We [manually] coded tutee utterances for help requests and self-explanations, and coded tutor utterances for elaborated help, unelaborated help, prompts and feedback. We also coded student dialog for general behaviors not found in the model. Table 1 describes the full coding of tutee and tutor behaviors."
% \end{enumerate}

\paragraph{Using Intelligent Tutor Technology to Implement Adaptive Support for Student Collaboration \citep{diziol_using_2010}}
\begin{enumerate}
    \item ``due to limitations of natural language processing, the development of adaptive support based on an analysis of \emph{student dialogue} is difficult."
    \item `` we propose to leverage existing intelligent tutoring technology to provide support based on student problem-solving actions"
    \item ``Thus, automated dialogue assessment solutions are beginning to be developed~\citep{israel_supporting_2007}. So far, this technology has only been used successfully in limited ways, such as for classifying the topic of conversation~\citep{kumar_tutorial_2007}, or for assessing student accuracy when they use sentence starters~\citep{israel_supporting_2007} Some researchers try to circumvent the problems of assessing dialogue by relying on simple metrics like participation to trigger feedback. For instance, these systems evaluate the amount or length of contributions collaborators make to a shared workspace or to a dialogue and support the interaction by directly encouraging the non-contributors to participate more (Constantino-Gonzalez et al. 2003)"
    \item ``we propose to leverage existing intelligent tutoring technology to provide support based on student problem-solving actions."
\end{enumerate}

\paragraph{Designing automated adaptive support to improve student helping behaviors in a peer tutoring activity \citep{walker_designing_2011}}
\begin{enumerate}
    \item ``Adaptive collaborative learning support systems analyze student collaboration as it occurs and provide targeted assistance to the collaborators"
    \item ``Too little is known about how to design adaptive support to have a positive effect on interaction and learning"
    \item ``we designed adaptive assistance for improving peer tutor help-giving, and deployed it in a classroom, comparing it to traditional fixed support."
    \item ``We found that the assistance improved the conceptual content of help and the use of interface features."
    \item  ``[We] used TagHelper \citep{rose_analyzing_2008}, a toolkit for automated text classification that has been successfully deployed in educational contexts, to build a machine classifier trained on previous study data (Cohen’s kappa = .82 for the previous dataset). The classifier could automatically determine whether students were giving help, and whether the help was conceptual."
\end{enumerate}



\subsubsection{Kristy Boyer}

\paragraph{Dialogue act modeling in a complex task-oriented domain \citep{boyer_dialogue_2010}}
\begin{enumerate}
    \item Classifying the dialogue act of a user utterance is a key functionality of a dialogue management system. 
    \item This paper presents a data-driven dialogue act classifier that is learned from a corpus of human textual dialogue in a task-oriented domain
    \item While engaging in the task, students generate a task event stream that is separate from and in parallel with the dialogue. To deal with this complex task-oriented dialogue, we propose a vector-based representation that encodes features from both the dialogue and the hierarchically structured task for training a maximum likelihood classifier.
    \item The corpus was manually annotated with dialogue act labels and task/subtask features. Lexical and syntactic features were extracted automatically.
    \item Experiments with the data-driven classifiers presented in this paper demonstrate that lexical/syntactic features can effectively classify student dialogue acts in the task-oriented tutoring domain.
    \item Data: ``The corpus was collected during a controlled human-human tutoring study in which tutors and
students worked through textual dialogue to solve an introductory computer programming problem"
\end{enumerate}	

\paragraph{Understanding Student Language: An Unsupervised Dialogue Act Classification Approach \citep{ezen-can_understanding_2015}}
\begin{enumerate}
    \item ``Automatic dialogue act modeling has long been addressed with supervised classification techniques that require substantial manual time and effort."
    \item ``there is emerging interest in unsupervised dialogue act classification, which addresses the challenges related to manually labeling corpora."
    \item this work ``builds on the growing body of work in unsupervised dialogue act classification and reports on the novel application of an information retrieval technique, the Markov Random Field, for the task of unsupervised dialogue act classification."
    \item ``Evaluation against manually labeled dialogue acts on a tutorial dialogue corpus in the domain of introductory computer science demonstrates that the proposed technique outperforms existing approaches to education-centered unsupervised dialogue act classification"
\end{enumerate}

\paragraph{A Tutorial Dialogue System for Real-Time Evaluation of Unsupervised Dialogue Act Classifiers: Exploring System Outcomes \citep{ezen-can_tutorial_2015}}
\begin{enumerate}
    \item ``We compare two versions of the tutorial dialogue system for introductory computer science: one that relies on a supervised dialogue act classifier and one that depends on an unsupervised dialogue act classifier"
\end{enumerate}

\paragraph{Combining Task and Dialogue Streams in Unsupervised Dialogue Act Models \citep{ezen-can_combining_2014}}
\begin{enumerate}
    \item  ``However, some dialogues, such as task-oriented dialogues with parallel task streams, hold rich information that has not yet been leveraged within unsupervised dialogue act models."
    \item They ``investigate incorporating task features into an unsupervised dialogue act model trained on a corpus of human tutoring in introductory computer science."
    \item ``results show that incorporating task features and dialogue history features significantly improve unsupervised dialogue act classification, particularly within a hierarchical framework that gives prominence to dialogue history"
\end{enumerate}

\paragraph{Unsupervised modeling for understanding MOOC discussion forums: a learning analytics approach \citep{ezen-can_unsupervised_2015}}
\begin{enumerate}
    \item ``most MOOCs include a rich textual dialogue forum, and these textual interactions are largely unexplored."
    \item They apply ``unsupervised student understanding models originally developed for synchronous tutorial dialogue to MOOC forums.
    \item ``They use a clustering approach to group similar posts, compare the clusters with manual annotations by MOOC researchers, and further investigate clusters qualitatively."
    A review that covers this: Systematic Review of Discussion Forums in Massive Open Online Courses (MOOCs) \citep{almatrafi_systematic_2018}: ``Many papers developed models that automatically classify the topic of the post. ... Content analysis, topic and feature extraction were conducted using bag-of-words, Latent Dirichlet Allocation (LDA), structural topic modelling or tools such as LIWC, Coh-metrix, and OpinionFinder. Clustering is another technique to group similar examples together (e.g. cluster posts with similar topics~\citep{ezen-can_unsupervised_2015}"
\end{enumerate}

\paragraph{Prompting collaborative and exploratory discourse: An epistemic network analysis study \citep{vandenberg_prompting_2021}}
\begin{enumerate}
    \item ``Epistemic Network Analysis (ENA) is an analytic technique that provides an alternative to more typical approaches to analyzing and synthesizing coded dialogue."
    \item ``This study used an easy-to-implement prompting intervention in the context of collaborative (pair) programming with upper elementary students to demonstrate the potential of ENA to understand the impact of the intervention." 
    \item ``We found that intervention students—those given empirically-derived prompts in support of collaborative and exploratory talk—asked questions, justified their thinking, and offered alternative ideas in ways that were both qualitatively and quantitatively different from control students."
\end{enumerate}

\paragraph{Discovering Co-creative Dialogue States During Collaborative Learning \citep{griffith_discovering_2021}}
\begin{enumerate}
    \item ``Many important forms of collaborative learning are co-creative in nature."
    \item ``AI systems to support co-creativity in learning are highly underinvestigated"
    \item To address this need, we analyzed the structure of collaborative dialogue between pairs of high school students who co-created music by writing code."
    \item ``We used hidden Markov models to analyze 68 co-creative dialogues consisting of 3,305 total utterances."
    \item ``The results distinguish seven hidden states: three of the hidden states are characterized by conversation, such as social, aesthetic, or technical dialogue. The remaining four hidden states are characterized by task actions including code editing, accessing the curriculum, running the code successfully, and receiving an error when running the code."
    \item ``These findings reveal processes of human co-creativity and can inform the design of intelligent co-creative agents that support human collaboration and learning.`
\end{enumerate}

\paragraph{Expressing and Addressing Uncertainty: A Study of Collaborative Problem-Solving Dialogues \citep{rodriguez_expressing_2017}}
\begin{enumerate}
    \item ``focuses on one important aspect of collaborative dialogue: expressions of uncertainty"
    \item ``In a study of undergraduate novice computer science students working in pairs, we observed that the students who produced the lowest quality solutions expressed uncertainty more often than those who produced middle-quality solutions"
    \item: They manually did dialogue act tagging scheme (based on~\citep{rodriguez_exploring_2017}) on written dialogue. ``We extracted the textual dialogue messages and split them into utterances based on punctuation marks. Uncertainty utterances were tagged as part of a broader dialogue labeling study that included thirteen distinct tags such as direct and indirect instructions, questions and answers, and partner feedback."
\end{enumerate}

\paragraph{Exploring the Pair Programming Process: Characteristics of Effective Collaboration \citep{rodriguez_exploring_2017}}
\begin{enumerate}
    \item ``examines the collaboration process, comparing important outcomes with how students' dialogue and problem-solving approaches unfolded"
    \item ``The results show that the collaboration is more effective when both partners make substantive dialogue contributions, express uncertainty, and resolve it."
    \item A collaborative programming Task: ``They collaborated following the pair programming paradigm: one student created and edited the program (the driver), and the other student provided guidance and feedback (the navigator). These roles remained constant throughout the one-hour study session."
    \item Data: ``logged students’ programming actions within Snap! and their chat conversations"
    \item (manual) Dialogue Analysis: ``manually tagged the dialogues with dialogue act tags"`
\end{enumerate}

\paragraph{Semantic Grounding in Dialogue for Complex Problem Solving \citep{li_semantic_2015}}
\begin{enumerate}
    \item ``Our approach performs joint segmentation and labeling of the noun phrases to link them to attributes of entities within the problem-solving environment."
    \item ``Evaluation results on a corpus of tutorial dialogue for Java programming demonstrate that a Conditional Random Field model performs well, achieving an accuracy of 89.3\% for linking semantic segments to the correct entity attributes"
    has nice Related Work on Language Understanding in Tutorial Dialogue Systems
\end{enumerate}


% \paragraph{In-context evaluation of unsupervised dialogue act models for tutorial dialogue \citep{ezen-can_-context_2013}}
% \begin{enumerate}
%     \item  presents an in-context evaluation framework for an un- supervised dialogue act model within tutorial dialogue.
%     \item The clusters generated by the model are mapped to tutor responses by a handcrafted policy
%     \item The results demonstrate that in-context evaluation of an unsupervised dialogue act model, rather than accuracy against manual labels, may better reflect the usefulness of the model for dialogue management. (The results demonstrate that this in-context evaluation may be equally useful as comparing against gold standard dialogue act labels, while substantially reducing the time required for human annotation.)
% \end{enumerate}


	
% Collaborative Dialogue and Types of Conflict: An Analysis of Pair Programming Interactions between Upper Elementary Students \citep{tsan_collaborative_2021}
% \begin{enumerate}
%     \item ``To investigate collaborative dialogue that elementary learners use and the conflicts that they encounter, we analyzed videos of twelve pairs of fifth grade students completing pair programming activities.
%     \item \emph{manual} annotation
%     \item ``developed a novel annotation scheme with a focus on collaborative dialogue and conflicts."
%     \item ``All pairs exhibited some conflicts about the task, but high-conflict pairs also engaged in conflicts about control of the computer and their partner's contributions."
%     \item ``results provide insights into the collaborative process of young learners in CS problem solving"
% \end{enumerate}


%%%%%%%%%%%%%%% other authors, relevant work, e.g. 


\subsubsection{Others} 

e.g.\ by Gautam Biswas

\paragraph{Examining Student Regulation of Collaborative, Computational, Problem-Solving Processes in Open-Ended Learning Environments \citep{emara_examining_2021}}
\begin{enumerate}
    \item ``present a systematic analysis framework that combines natural language processing (NLP) of collaborative dialogue, log file analyses of students' model-building actions, and final model scores. This analysis is used to better understand students' regulation of collaborative problem solving (CPS) processes over a series of computational modelling tasks of varying complexity."
    \item ``The results suggest that the computational modelling challenges afford opportunities for students to \dots learn from each other using socially shared regulation (SSR) and productive collaboration."
\end{enumerate}

Others

\paragraph{What’s in a Cluster? Automatically Detecting Interesting Interactions in Student E-Discussion \citep{miksatko_whats_2008}}
\begin{enumerate}
    \item We focused on the identification of clusters of contributions representing interaction patterns that are of pedagogical interest (e.g., a student clarifies his or her opinion and then gets feedback from other students). 
    \item We designed an algorithm that takes an example cluster as input and uses inexact graph matching, text analysis, and machine learning classifiers to search for similar patterns in a given corpus. 
    \item The method was evaluated on an annotated dataset of real e-discussions and was able to detect almost 80\% of the annotated clusters while providing acceptable precision performance.
\end{enumerate}

\paragraph{What Do You Mean by Collaboration Analytics? A Conceptual Model \citep{martinez-maldonado_what_2021}}
\begin{enumerate}
    \item ``Collaboration analytics partially or fully automate the analysis of data captured from group/team settings. These include co-located, face-to-face groups and platform-mediated groups (synchronous and asynchronous)."
\end{enumerate}

\paragraph{Conversation-Based Learning and Assessment Environments \citep{graesser_conversation-based_2020}}
\begin{enumerate}
    \item we focus on conversation-based learning and assessment environments via the AutoTutor system, in which one or more computerized agents interact with human learners across multiple turns for a given task.
\end{enumerate}

\paragraph{Group communication analysis: A computational linguistics approach for detecting sociocognitive roles in multiparty interactions \citep{dowell_group_2019}}
\begin{enumerate}
    \item we propose and validate a novel approach for detecting emergent roles from participants’ contributions and patterns of interaction.
    \item Specifically, we developed a group communication analysis (GCA) by combining automated computational linguistic techniques with analyses of the sequential interactions of online group communication.
    \item The results indicated that participants’ patterns of linguistic coordination and cohesion are representative of the roles that individuals play in collaborative discussions. M
\end{enumerate}

\paragraph{Challenges of Assessing Collaborative Problem Solving~\citep{graesser_challenges_2018}}
\begin{enumerate}
    \item the use of computer agents in the assessment of CPS proficiency
    \item ``At one extreme are fully embodied conversational agents in a virtual environment with speech recognition (e.g., the Tactical Language and Culture System, see Johnson and Valente 2008) and tutorial learning environments that hold conversations with the student with talking heads, such as AutoTutor~\citep{graesser_learning_2014,lehman_inducing_2013}, Betty’s Brain (Biswas et al. 2010), Operation ARIES/ARA (Halpern et al. 2012; Millis et al. 2011), and iSTART (Jackson and McNamara 2013).
    \item Such environments are motivating to 15-year old students, but the solution is impractical. There would be major challenges in technology, costs, and cultural variations in language and discourse. The more appropriate solution for assessments like PISA is minimalist agents that consist of printed messages in windows on the computer display, such as email messages, chat facilities, print in bubbles besides icons, and documents in various social communication media (Rouet 2006). These forms of agent-based social communication media have already been implemented in PIAAC (OECD 2009) on problem solving in electronically rich environments."
\end{enumerate}



% % Possible citations - summarised
% \begin{enumerate}
%     %%%%%% reviews: 
%     % \citep{dillenbourg_evolution_2009} 
%     \item In research on educational dialogue, the unit of analysis to be understood and explained  is \emph{the processes of development of collective thinking in and by dialogue}~\citep{baker_educational_2021}.
%     % \item Analysis of language and text artifacts produced in a learning context is basis for assessment~\citep{trausan-matu_artifact_2021}. %considers ``different forms of language and text artifact analysis that are presently applied within the learning sciences."
%     \item Automated analysis of discussion is one of the approaches in computer-supported argumentation systems to guide the students' activities~\citep{scheuer_computer-supported_2010}. For instance, the system can analyzes the discussion process, and automatically annotate the contributions with for instance dialogue acts, e.g.\ in~\citep{goodman_using_2005,mclaren_supporting_2010, israel_supporting_2007,rose_analyzing_2008}, or classify the content of the discussion, e.g.\ in ~\citep{kumar_tutorial_2007}.
%     \item Collaboration analytics partially or fully automate the analysis of data captured from group/team settings. \dots In order to provide intelligent interfaces that support collaboration and teamwork, designers of collaboration analytics require a methodology for imbuing low-level data with contextual meaning and interfaces that communicate insights at a higher-order level"~\citep{martinez-maldonado_what_2021}.
%     \item Interaction analysis investigates ``what students are doing as they communicate and collaborate with one another, at a relatively fine-grain level": it has served ``as a basis for providing adaptive guidance and feedback"~\citep{tchounikine_computer_2010}.
    
%     % \item International Handbook of Computer-Supported Collaborative Learning \citep{cress_international_2021} Summary of the handbook: \citep{cress_foundations_2021}

%     %%%%%%  Carolyn Rose: 
%     % Manual to automatic: \cite{donmez_supporting_2005,rose_analyzing_2008} Carolyn summarising these: \cite{rummel_new_2008}

%     \item \citet{weinberger_framework_2006} manually coded online, written discussions along multiple process dimensions, such as the participation dimension that accounts for to what extent learners contribute to the dialogue, and epistemic dimension that also considers the content of learners' contributions, in order to analyse the process of how learners construct arguments through dialogue. \citet{donmez_supporting_2005} automated the process of coding from \cite{weinberger_framework_2006} by using natural language processing with high levels of agreement with human annotations. Then, \citet{rose_analyzing_2008} demonstrated that the automatic extraction can be done reliably from texts. % Carolyn summarises Manual to automatic: \cite{donmez_supporting_2005,rose_analyzing_2008} in \cite{rummel_new_2008}
%     % \citet{kumar_tutorial_2007} have focused on providing real-time support to dyads collaborating on a problem-solving task: they describe an evaluation of a simple but fully-automatic approach to adaptive collaborative learning support. 
%     \item \citet{mu_acodea_2012} ``present a framework for developing coding schemes optimized for automatic segmentation and extract context-independent coding that builds on this segmentation"
%     \item \citet{gweon_measuring_2013} ``do assessment of transactivity in dyadic discussions, where a transactive contribution is operationalized as one where reasoning is made explicit, and where that reasoning builds on a prior reasoning statement within the discussion"
%     \item \citet{howley_towards_2016} ``reviews work in progress towards bridging the field of linguistics and its operationalizations of discourse, and that of frameworks for studying collaborative learning that are rooted directly in the learning sciences."
%     \item To analyse student behavior in Massive Open Online Courses (MOOCs), \citet{yang_exploring_2016} automatically predict a confusion level for students from their participation in th course discussion forums along with their clicking behavior: in the student's posts, they check the presence of domain-specific content words, and high-level linguistic features.
%     \item \citet{jo_modeling_2017} ``present an unsupervised model of dialogue act sequences in conversation" They compare with \citep{ezen-can_understanding_2015} that uses Markov Random Field as their unsupervised model
%     \item \citet{howley_towards_2016} ``reviews work in progress towards bridging the field of linguistics and its operationalizations of discourse"

%     %%%%%% Sidney D'Mello: 
%     \item \citet{dmello_design_2013} presents an overview of dialog-based intelligent tutoring systems. 
%     % , within the context of one of the first dialog-based ITSs named AutoTutor~\citep{graesser_learning_2014,lehman_inducing_2013,graesser_conversation-based_2020}
%     \citet{dmello_toward_2010,litman_spoken_2004} investigate ITSs that automatically process spoken input. 
%     \item \citet{stewart_i_2019} investigate automatic detection of critical collaborative problem solving (CPS) processes, on transcripts obtained via automatic speech recognition, and 
%     \citet{pugh_say_2021} targets recorded speech in noisy environments: they show ``despite significant speech recognition error, it is possible to predict expert-coded CPS skills using automatically generated transcripts". Furthermore, \citet{stewart_multimodal_2021} ``builds automated detectors of three critical CPS facets—construction of shared knowledge, negotiation and coordination" from ``linguistic, task context, facial expressions, and acoustic–prosodic features." 
%     For CPS assessment at scale, \citep{graesser_challenges_2018} suggested using minimalist Computer agents as a means to assessment.
    
%     %%%%%% Erin Walker:
%     \item \citet{walker_using_2011} presents ``an automated detector of conceptual content that is used as a basis for providing adaptive prompts to peer tutors" .
%     \item  \citet{walker_designing_2011} ``designed adaptive assistance for improving peer tutor help-giving", where they ``used TagHelper \citep{rose_analyzing_2008}, a toolkit for automated text classification that has been successfully deployed in educational contexts, to build a machine classifier trained on previous study data (Cohen’s kappa = .82 for the previous dataset). The classifier could automatically determine whether students were giving help, and whether the help was conceptual."

%     % \item Kristy Boyer:
%     \item \citet{boyer_dialogue_2010} show that dialogue acts can be effectively classified
%     on a corpus of human textual dialogue in a task-oriented domain, via a vector-based representation that encodes features from both the dialogue and the task events.
%     \item Since supervised classification techniques need substantial effort to scale, \citet{ezen-can_understanding_2015} apply a(n) (unsupervised) clustering approach  to group dialogue utterances with the same dialogue act, on a tutorial dialogue corpus
%     %(an information retrieval technique,  Markov Random Field)
%     \item \citet{ezen-can_tutorial_2015} compares a supervised and an unsupervised dialogue act classifier.
%     \item \citet{ezen-can_combining_2014} show that incorporating task features into an unsupervised dialogue act model on a tutorial dialogue corpus improves unsupervised dialogue act classification
%     \item For MOOCs, models have been developed to automatically classify the topic of the post \citet{almatrafi_systematic_2018}, for instance, citet{ezen-can_unsupervised_2015} use a clustering approach to group similar posts.
%     \item \citet{vandenberg_prompting_2021} showed that a graph-theoretic technique (Epistemic Network Analysis) to prompt intervention ``permit comparative analysis visually and quantitatively, with the support of direct qualitative evidence" as insights into a collaborative dialogue.
%     \item \citet{griffith_discovering_2021} showed that hidden Markov models to characterize the structure of a collaborative dialogue can reveal processes of human co-creativity.
%     \item [MANUAL and LINK TO OUTCOMES] \citep{rodriguez_exploring_2017} examined the collaboration process by manually tagging the dialogues with dialogue act tags in a collaborative programming task with fixed roles. Then, they ``compared the outcomes with how students' dialogue and problem-solving approaches unfolded". by manual dialogue act tagging (based on the same scheme) on written dialogue, \citet{rodriguez_expressing_2017} studied expressions of uncertainty, and linked it with the quality of their solutions.
    
%     %%%%%% Other authors
%     \item{emara_examining_2021} ``present a systematic analysis framework that combines natural language processing (NLP) of collaborative dialogue, log file analyses of students' model-building actions, and final model scores."
%     \item \citep{miksatko_whats_2008}  identify ``clusters of contributions representing interaction patterns that are of pedagogical interest (e.g., a student clarifies his or her opinion and then gets feedback from other students).", by ``taking an example cluster as input and uses inexact graph matching, text analysis, and machine learning classifiers to search for similar patterns in a given corpus." for an annotated dataset of real e-discussions
%     \item \citet{dowell_group_2019} developed a group communication analysis (GCA) by combining automated computational linguistic techniques with analyses of the sequential interactions of online group communication.
% \end{enumerate}


\subsection{Alignment in educational data} \label{subsec: alignment_in_education_papers}
% Reviewer 1: ``And for alignment (and variants such as entrainment, convergence, priming, coordination) and educational data, I suggest the authors review the work of Nichola Lubold, Diane Litman, and Justine Cassell as a starting point."

\subsubsection{Nichola Lubold}

\paragraph{Acoustic-Prosodic Entrainment and Rapport in Collaborative Learning Dialogues \citep{lubold_acoustic-prosodic_2014}}
\begin{enumerate}
    \item ``We explore in this paper how low level features of the speech signal, such as pitch, loudness, and speaking rate, can inform a model of student interaction in collaborative learning dialogues."
    \item ``By detecting interaction qualities such as rapport, we can better support collaborative interactions, which have been shown to be highly conducive to learning."
    \item ``We focus on one particular phenomenon of spoken conversation, known as \textbf{acoustic-prosodic entrainment}, where dialogue partners become more similar to each other in their pitch, loudness, or speaking rate during the course of a conversation."
    \item ``We examine whether acoustic-prosodic entrainment is present in a novel corpus of collaborative learning dialogues, how people appear to entrain, to what degree, and report on the acoustic-prosodic features which people entrain on the most."
    \item ``We then investigate whether entrainment can facilitate detection of rapport, a social quality of the interaction."
    \item ``We find that entrainment does correlate to rapport; speakers appear to entrain primarily by matching their prosody on a turn-by-turn basis, and pitch is the most significant acoustic-prosodic feature people entrain on when rapport is present."
\end{enumerate}

\paragraph{Effects of voice-adaptation and social dialogue on perceptions of a robotic learning companion \citep{lubold_effects_2016}}
\begin{enumerate}
    \item ``This paper presents a socially responsive speech interface for an embodied, robotic learning companion. We explore two methods of social responsiveness. The first method introduces social responses into the dialogue, while the second method \textbf{augments these responses with voice-adaptation based on acoustic-prosodic entrainment}."
    \item ``We evaluate the effect of a social, voice-adaptive robotic learning companion on social variables such as social presence and rapport, and we compare this to a companion with only social dialogue and one with neither social dialogue nor voice-adaptions." \item We contrast the effects against those of individual factors, such as gender."
    \item ``We find (1) that social presence is significantly higher with a social voice-adaptive speech interface than with purely social dialogue"
\end{enumerate}

\paragraph{Effects of adapting to user pitch on rapport perception, behavior, and state with a social robotic learning companion \citep{lubold_effects_2021}}
\begin{enumerate}
    \item ``People rarely communicate with just words alone; facial expressions, gaze, gesture, and prosodic cues like tone of voice and speaking rate combine to help individuals express their words and convey emotion."
    \item ``One way that individuals communicate a sense of connection with one another is \textbf{entrainment, where interaction partners adapt their way of speaking, facial expressions, or gestures to each other}; entrainment has been linked to trust, liking, and task success and is thought to be a vital phenomenon in how people build rapport."
    \item ``In this work, we introduce a social robot that combines multiple channels of rapport-building behavior, including forms of social dialog and prosodic entrainment."
    \item ``We explore how social dialog and entrainment contribute to both self-reported and behavioral rapport responses." 
    \item ``We find prosodic adaptation enhances perceptions of social dialog, and that social dialog and entrainment combined build rapport."
\end{enumerate}

\paragraph{Automated Pitch Convergence Improves Learning in a Social, Teachable Robot for Middle School Mathematics \citep{lubold_automated_2018}}
\begin{enumerate}
    \item ``Several social behaviors have been explored with pedagogical agents including facial expressions, movement, and social dialogue; social dialogue has especially been shown to positively influence interactions. 
    \item ``In this work, we explore \textbf{the role of paraverbal social behavior} or social behavior \textbf{in the form of paraverbal cues such as tone of voice and intensity}. To do this, we focus on the phenomenon of \textbf{entrainment, where individuals adapt their paraverbal features of speech to one another}."
    \item ``Paraverbal entrainment in human-human studies has been found to be correlated with rapport and learning." ?? Could not find a pointer to a study
    \item ``In a study with 72 middle school students, we evaluate the effects of entrainment with a teachable robot, a pedagogical agent that learners teach how to solve ratio problems."
    \item ``We explore how a teachable robot which entrains and introduces social dialogue influences rapport and learning; we compare with two baseline conditions: a social condition, in which the robot speaks socially, and a non-social condition, in which the robot neither entrains nor speaks socially."
    \item ``We find that a robot that does entrain and speaks socially results in significantly more learning."
\end{enumerate}

\paragraph{Naturalness and rapport in a pitch adaptive learning companion \citep{lubold_naturalness_2015}} + Erin Walker
\begin{enumerate}
    \item ``In an application like the learning companion, such a socially responsive dialogue system may improve learning and motivation. However, it is not clear how to produce entrainment in an automatic dialogue system in ways that produce the effects seen in human-human dialogue."
    \item ``In this paper, we take the first steps towards implementing a spoken dialogue system which can entrain. We propose three methods of pitch adaptation based on analysis of human entrainment, and design and implement a system which can manipulate the pitch of text-to-speech output adaptively." 
    \item ``We find a clear relationship between perceptions of rapport and different forms of pitch adaptations. Certain adaptations are perceived as significantly more natural and rapport-like. Ultimately, adapting by shifting the pitch contour of the text-to-speech output by the mean pitch of the user results in the highest reported measures of rapport and naturalness."
\end{enumerate}

\paragraph{Comfort with Robots Influences Rapport with a Social, Entraining Teachable Robot \citep{lubold_comfort_2019}}
\begin{enumerate}
    \item ``Teachable agents are pedagogical agents that employ the `learning-by-teaching' strategy, which facilitates learning by encouraging students to construct explanations, reflect on misconceptions, and elaborate on what they know. Teachable agents present unique opportunities to maximize the benefits of a `learning-by-teaching' experience."
    \item ``Prior work has found that a teachable agent which \textbf{engages learners socially through social dialogue and paraverbal adaptation on pitch can have positive effects on rapport and learning}."
    \item ``In this work, we introduce Emma, \textbf{a teachable robotic agent that can speak socially and adapt on both pitch and loudness}. Based on the phenomenon of entrainment, multi-feature adaptation on tone and loudness has been found in human-human interactions to be highly correlated to learning and social engagement."
    \item ``In a study with 48 middle school participants, we performed a novel exploration of how multi-feature adaptation can influence learner rapport and learning as an independent social behavior and combined with social dialogue."
    \item ``We found significantly more rapport for Emma when the robot both adapted and spoke socially than when Emma only adapted and indications of a similar trend for learning. Additionally, it appears that an individual’s initial comfort level with robots may influence how they respond to such behavior, suggesting that for individuals who are more comfortable interacting with robots, social behavior may have a more positive influence."
\end{enumerate}

\paragraph{Relating Entrainment, Grounding, and Topic of Discussion in Collaborative Learning Dialogues \citep{lubold_relating_2015}}
\begin{enumerate}
    \item ``In conversational dialogue, grounding refers to the joint activity of speakers and listeners establishing common ground—a shared understanding of their mutual knowledge, beliefs, and assumptions. Grounding is a critical component of successful collaborative interactions and plays an important role in collaborative learning."
    \item ``In this work, we \textbf{investigate grounding utilizing acoustic-prosodic entrainment}. Acoustic-prosodic entrainment occurs in spoken dialogue when speakers adapt their tone, loudness, voice quality, or speaking rate to that of their partner."
    \item ``We explore the relationship between grounding and acoustic-prosodic entrainment within on-task and off-task dialogue, and we \textbf{find that grounding behaviors in both on-task and off-task dialogue are differentiated by how speakers entrain.}"
\end{enumerate}

\paragraph{Building Rapport through Dynamic Models of Acoustic-Prosodic Entrainment \citep{lubold_building_2017}}
\begin{enumerate}
    \item ``As dialogue systems become more prevalent in the form of personalized assistants, there is an increasingly important role for systems which can socially engage the user by influencing social factors like rapport. For example, learning companions enhance learning through socio-motivational support and are more successful when users feel rapport."
    \item ``In this work, I \textbf{explore social engagement in dialogue systems in terms of acoustic-prosodic entrainment}.
    \item ``entrainment is a phenomenon where over the course of a conversation, speakers adapt their acoustic-prosodic features, becoming more similar in their pitch, intensity, or speaking.  Correlated with rapport and task success, entrainment plays a significant role in how individuals connect; a system which can entrain has potential to improve social engagement by enhancing these factors."
    \item ``As a result of this work, I introduce a dialogue system which can entrain and investigate its effects on social factors like rapport."
\end{enumerate}

% \paragraph{Do Conversational Partners Entrain on Articulatory Precision? \citep{lubold_conversational_2019}}
% \begin{enumerate}
%     \item ``The communication phenomenon known as \textbf{conversational entrainment} occurs when dialogue partners \textbf{align or adapt their behavior to one another while conversing}. Associated with rapport, trust, and communicative efficiency, entrainment appears to facilitate conversational success."
%     \item ``In this work, we explore how conversational partners entrain or align on articulatory precision or the clarity with which speakers articulate their spoken productions. Articulatory precision also has implications for conversational success as precise articulation can enhance speech understanding and intelligibility."
%     \item ``However, in conversational speech, speakers tend to reduce their articulatory precision, preferring low-cost, imprecise speech. Speakers may adapt their articulation and become more precise depending on feedback from their listeners." \item ``Given the potential of entrainment, \textbf{we are interested in how conversational partners adapt or entrain their articulatory precision to one another}. We explore this phenomenon in 57 task-based dialogues."
%     \item ``Controlling for the influence of speaking rate, we find that speakers entrain on articulatory precision, with significant alignment on articulation of consonants. We discuss the potential applications that speaker alignment on precision might have for modeling conversation and implementing strategies for enhancing communicative success in human-human and human-computer interactions."
% \end{enumerate}

\paragraph{[Thesis] Producing Acoustic-Prosodic Entrainment in a Robotic Learning Companion to Build Learner Rapport \citep{lubold_producing_2018}}
\begin{enumerate}
    \item In human-human interactions, rapport is critical to patient-doctor communication, conflict resolution, educational interactions, and social engagement. Rapport between people promotes successful collaboration, motivation, and task success. 
    Dialogue systems which can build rapport with their user may produce similar effects, personalizing interactions to create better outcomes. 
    This dissertation focuses on \textbf{how dialogue systems can build rapport utilizing acoustic-prosodic entrainment}. Acoustic-prosodic entrainment occurs when individuals adapt their acoustic-prosodic features of speech, such as tone of voice or loudness, to one another over the course of a conversation. 
    \item ``Correlated with liking and task success,  \textbf{a dialogue system which entrains} may enhance rapport. Entrainment, however, is very challenging to model. People entrain on different features in many ways and how to design entrainment to build rapport is unclear. 
    \item ``The first goal of this dissertation is to explore how acoustic-prosodic entrainment can be modeled to build rapport. Towards this goal, this work presents a series of studies comparing, evaluating, and iterating on the design of entrainment, motivated and informed by human-human dialogue. These models of entrainment are implemented in the dialogue system of a robotic learning companion. Learning companions are educational agents that engage students socially to increase motivation and facilitate learning. As a learning companion's ability to be socially responsive increases, so do vital learning outcomes. 
    \item ``A second goal of this dissertation is to explore the effects of entrainment on concrete outcomes such as learning in interactions with robotic learning companions
    \item ``Technical contributions include a robust and modular dialogue system capable of producing prosodic entrainment and other socially-responsive behavior.
    \item ``One of the first systems of its kind, the results demonstrate that an entraining, social learning companion can positively build rapport and increase learning. This dissertation provides support for exploring phenomena like entrainment to enhance factors such as rapport and learning and provides a platform with which to explore these phenomena in future work."
\end{enumerate}



\subsubsection{Diane Litman}

\paragraph{Dialog Convergence and Learning \citep{ward_dialog_2007}}
\begin{enumerate}
    \item ``In this paper we examine whether the student-to-tutor convergence of lexical and speech features is a useful predictor of learning in a corpus of spoken tutorial dialogs. This possibility is raised by the Interactive Alignment Theory, which suggests a connection between convergence of speech features and the amount of semantic alignment between partners in a dialog."
    \item ``A number of studies have shown that users converge their speech productions toward dialog systems. If, as we hypothesize, semantic alignment between a student and a tutor (or tutoring system) is associated with learning, then this convergence may be correlated with learning gains."
    \item ``We present evidence that both lexical convergence and convergence of an acoustic/prosodic feature are useful features for predicting learning in our corpora."
    \item ``We also find that our measure of lexical convergence provides a stronger correlation with learning in a human/computer corpus than did a previous measure of lexical cohesion."
\end{enumerate}

\paragraph{Automatically measuring lexical and acoustic/prosodic convergence in tutorial dialog corpora \citep{ward_automatically_2007}}
\begin{enumerate}
    \item ``We show that these measures successfully discriminate randomized from naturally ordered data, and demonstrate both lexical and acoustic/prosodic convergence in our corpus of human/human tutoring dialogs."
\end{enumerate}

% \paragraph{The Teams Corpus and Entrainment in Multi-Party Spoken Dialogues \citep{litman_teams_2016}}
% \begin{enumerate}
%     \item ``To support research on entrainment in cooperative multi-party dialogues, we have created a corpus where teams of three or four speakers play two rounds of a cooperative board game."
%     \item ``We illustrate the use of our corpus as a novel resource for studying team entrainment by 1) developing and evaluating team- level acoustic-prosodic entrainment measures that extend existing dyad measures, and 2) investigating relationships between team entrainment and participation dominance."
% \end{enumerate}

\paragraph{Prosodic Entrainment and Tutoring Dialogue Success \citep{thomason_prosodic_2013}}
\begin{enumerate}
    \item ``This study investigates the relationships between student entrainment to a tutoring dialogue system and learning."
    \item ``By finding the features of prosodic entrainment which correlate with learning, we hope to inform educational dialogue systems aiming to leverage entrainment."
    \item ``We propose a novel method to measure prosodic entrainment and find specific features which correlate with user learning. We also find differences in user entrainment with respect to tutor voice and user gender."
\end{enumerate}

\paragraph{Entrainment in Multi-Party Spoken Dialogues at Multiple Linguistic Levels \citep{rahimi_entrainment_2017}}
\begin{enumerate}
    \item lexical entrainment~\citep{levitan_entrainment_2011,gonzales_language_2010,nenkova_high_2008,niederhoffer_linguistic_2002}
    \item ``While there is considerable evidence for both lexical and acoustic-prosodic entrainment, little work has been conducted to investigate the relationship between these two different modalities using the same measures in the same dialogues, specifically in multi-party dialogue."
    \item ``[W]e measure lexical and acoustic-prosodic entrainment for multi-party teams to explore whether entrainment occurs at multiple levels during conversation and to understand the relationship between these two modalities."
\end{enumerate}

\paragraph{Entrainment2Vec: Embedding Entrainment for Multi-Party Dialogues \citep{rahimi_entrainment2vec_2020}}
\begin{enumerate}
    \item Extending the adaptive pairwise entrainment measure in~\citep{danescu-niculescu-mizil_computational_2012} for dyadic to multi-party
    \item ``Entrainment is the propensity of speakers to begin behaving like one another in conversation."
    \item ``While most entrainment studies have focused on dyadic interactions, researchers have also started to investigate multi-party conversations. In these studies, multi-party entrainment has typically been estimated by averaging the pairs' entrainment values or by averaging individuals' entrainment to the group. While such multi-party measures utilize the strength of dyadic entrainment, they have not yet exploited different aspects of the dynamics of entrainment relations in multi-party groups."
    \item ``In this paper, utilizing an existing pairwise asymmetric entrainment measure, we propose a novel graph-based vector representation of multi-party entrainment that incorporates both strength and dynamics of pairwise entrainment relations."
    \item ``The proposed kernel approach and weakly-supervised representation learning method show promising results at the downstream task of predicting team outcomes. Also, examining the embedding, we found interesting information about the dynamics of the entrainment relations. For example, teams with more influential members have more process conflict."
\end{enumerate}

\paragraph{Investigating the Relationship between Multi-Party Linguistic Entrainment, Team Characteristics and the Perception of Team Social Outcomes \citep{yu_investigating_2019}}
\begin{enumerate}
    \item ``Multi-party linguistic entrainment refers to the phenomenon that speakers tend to speak more similarly during conversation."
    \item ``We first developed new measures of multi-party entrainment on features describing linguistic style, and then examined the relationship between entrainment and team characteristics in terms of gender composition, team size, and diversity."
    \item ``Next, we predicted the perception of team social outcomes using multi-party linguistic entrainment and team characteristics with a hierarchical regression model."
    \item ``We found that teams with greater gender diversity had higher minimum convergence than teams with less gender diversity."
    \item ``Entrainment contributed significantly to predicting perceived team social outcomes both alone and controlling for team characteristics."
\end{enumerate}


\subsubsection{Justine Cassell}

\paragraph{We Click, We Align, We Learn: Impact of Influence and Convergence Processes on Student Learning and Rapport Building \citep{sinha_we_2015}}
\begin{enumerate}
    \item ``\textbf{Behavioral convergence} has been identified as one (largely subconscious) contributor to successful conversations, while \textbf{rapport} is one of the central constructs that explains development of personal relationships between these speakers over time. Social factors such as these have been shown to play a potent role in learning."
    \item ``Therefore, in this work, we investigate the relationship in dyadic peer tutoring conversations of convergence, building up of interpersonal rapport over time, and student learning, while positing a novel mechanism that links these constructs."
    \item ``We develop an approach for hierarchical computational modeling of convergence by accounting for time-based dependencies that arise in longitudinal interaction streams, and can thus a) quantify the effect of one partner's behavior on the other and differentiate between driver and recipient (Influence), b) extrapolate the outcome of directional influence to determine adaptation in partners' behaviors (Convergence)."
    \item ``Our results illustrate that influence, convergence and rapport in the peer tutoring dialog are correlated with learning gains and provide concrete evidence for rapport being a causal mechanism that leads to convergence of speech rate in the interaction."
    \item ``We discuss the implications of our work for the development of peer tutoring agents that can improve learning gains through convergence to and from the human learner's behavior."
\end{enumerate}

\paragraph{Exploring Socio-Cognitive Effects of Conversational Strategy Congruence in Peer Tutoring \citep{sinha_exploring_2015}}
\begin{enumerate}
    \item ``Conversational interaction is a dynamic process in which information is conveyed and relationships are negotiated via the use and timing of specific conversational strategies."
    \item ``In this work we \textbf{examine similarity in use and timing of the relationship-oriented communicative strategies self-disclosure, reference to shared experience and praise, during a reciprocal peer tutoring interaction}."
    \item ``We \textbf{computationally model two kinds of similarity} that quantify whether and how students are similar or different in their use of the strategies over time, and differentiate the effects by gender, relationship status and session."
    \item ``In order to assess their impact, we leverage learning and self-reported rapport as outcome variables."
    \item ``Our results show significant effects in cumulative use as well as in the pattern of timings of conversational strategy usage by partners in a dyad, along with \textbf{interesting relationships to socio-cognitive processes.}"
\end{enumerate}

\paragraph{Automatic Recognition of Conversational Strategies in the Service of a Socially-Aware Dialog System \citep{zhao_automatic_2016}}
\begin{enumerate}
    \item ``In this work, we focus on automatically recognizing social conversational strategies that in human conversation contribute to building, maintaining or sometimes destroying a budding relationship. These conversational strategies include self-disclosure, reference to shared experience, praise and violation of social norms."
    \item ``By including rich contextual features drawn from verbal, visual and vocal modalities of the speaker and interlocutor in the current and previous turn, we can successfully recognize these dialog phenomena with an accuracy of over 80\% and kappa ranging from 60-80\%."
    \item ``Our findings have been successfully integrated into an end-to-end socially aware dialog system, with implications for virtual agents that can use rapport between user and system to improve task-oriented assistance."
\end{enumerate}

\paragraph{Using Temporal Association Rule Mining to Predict Dyadic Rapport in Peer Tutoring \citep{madaio_using_2017}}
\begin{enumerate}
    \item ``Social relationships, such as interpersonal closeness or rapport, can lead to improved student learning, but such dynamic, interpersonal phenomena can be difficult for educational support technologies to detect."
    \item ``In this paper, we describe an approach for rapport detection in peer tutoring, using temporal association rules learned from nonverbal, social, and on-task verbal behaviors."
    \item ``From a corpus of 60 hours of annotated multimodal peer tutoring data, we learn the temporal association between behaviors and the rapport score for each 30-second "thin-slice". We then train a stacked ensemble classification model on those association rules and evaluate our ability to reliably predict rapport using multimodal behavioral data."
    \item ``We find that our approach allows us to predict rapport well above chance, and more accurately than two baseline models. We are able to predict high rapport more accurately for strangers and low rapport more accurately for friends, which we believe holds promise for the integration of rapport detection into collaborative learning supports and intelligent tutoring systems."
\end{enumerate}

% \paragraph{Towards a Computational Architecture of Dyadic Rapport Management for Virtual Agents \citep{papangelis_towards_2014}}
% \begin{enumerate}
%     \item ``Rapport has been identified as an important factor in human task performance. Motivated by the proliferation of virtual agents that assist humans on various tasks, we propose a computational architecture for virtual agents, building on our own work on a dyadic model of rapport between humans and virtual agents."
%     \item ``We show how such a system can be trained in order to build, maintain and destroy rapport."
% \end{enumerate}

% \paragraph{Towards a Dyadic Computational Model of Rapport Management for Human-Virtual Agent Interaction \citep{zhao_towards_2014}}
% \begin{enumerate}
%     \item ``Rapport has been identified as an important function of human interaction, but to our knowledge no model exists of building and maintaining rapport between humans and conversational agents over the long-term that operates at the level of the dyad."
%     \item ``In this paper we leverage existing literature and a corpus of peer tutoring data to develop a framework able to explain how humans in dyadic interactions build, maintain, and destroy rapport through the use of specific conversational strategies that function to fulfill specific social goals, and that are instantiated in particular verbal and nonverbal behaviors."
%     \item ``We demonstrate its functionality using examples from our experimental data."
% \end{enumerate}

% \paragraph{Towards a Model of Face-to-Face Grounding \citep{nakano_towards_2003}}
% \begin{enumerate}
%     \item ``We investigate the verbal and nonverbal means for grounding, and propose a design for embodied conversational agents that relies on both kinds of signals to establish common ground in human-computer interaction."
%     \item ``We analyzed eye gaze, head nods and attentional focus in the context of a direction-giving task."
%     \item ``The distribution of nonverbal behaviors differed depending on the type of dialogue move being grounded, and the overall pattern reflected a monitoring of lack of negative feedback."
%     \item ``Based on these results, we present an ECA that uses verbal and nonverbal grounding acts to update dialogue state."
% \end{enumerate}

% \paragraph{Socially-Conditioned Task Reasoning for a Virtual Tutoring Agent \citep{zhao_socially-conditioned_2018}}
% \begin{enumerate}
%     \item ``Virtual agents have been shown to be more effective when incorporating social factors such as trust into task action selection. However, there has been less work on how virtual tutoring agents can incorporate social factors into pedagogical action selection."
%     \item ``We propose and evaluate how a socially-conditioned task reasoner for a virtual pedagogical agent can incorporate both task and social factors into task reasoning."
%     \item ``Our work contributes to the autonomous agent community by providing further evidence that incorporating information about dyadic social factors (e.g.\ \textbf{rapport}) can be beneficial for agents' task reasoning in the case of a tutoring agent."
% \end{enumerate}

% \paragraph{``Oh dear stacy!": social interaction, elaboration, and learning with teachable agents \citep{ogan_oh_2012}}
% \begin{enumerate}
%     \item ``We describe results from a think-aloud study where children were instructed to narrate their experience teaching Stacy, an agent who can learn to solve linear equations with the student's help."
%     \item ``We found treating her as a partner, primarily through aligning oneself with Stacy using pronouns like you or we rather than she or it significantly correlates with student learning, as do playful face-threatening comments such as teasing, while elaborate explanations of Stacy's behavior in the third-person and formal tutoring statements reduce learning gains. 
%     \item ``Additionally, we found that the agent's mistakes were a significant predictor for students shifting away from alignment with the agent."
% \end{enumerate}



\subsubsection{Others}

\paragraph{Linguistic and Gestural Coordination: Do Learners Converge in Collaborative Dialogue? \citep{sinclair_linguistic_2021}}
\begin{enumerate}
    \item ``Collaborative dialogue is rich in conscious and subconscious coordination behaviours between participants. This work explores collaborative learner dialogue through theories of alignment, analysing inter-partner movement and language use with respect to our hypotheses: that they interrelate, and that they form predictors of collaboration quality and learning"
    \item ``In keeping with theories of alignment, we find that linguistic alignment and gestural synchrony both correlate significantly with one another in dialogue."
    \item ``We also find strong individual correlations of these metrics with collaboration quality. We find that linguistic and gestural alignment also correlate with learning. Through regression analysis, we find that although interconnected, these measures in combination are significant predictors of collaborative problem solving success."
    \item ``We contribute additional evidence to support the theory that alignment takes place across multiple levels of communication, and provide a methodological approach for analysing inter-speaker dynamics in a multimodal task based setting."
    \item ``Our work has implications for the teaching community, our measures can help identify poorly performing groups, lending itself to informing the design of real time intervention strategies or formative assessment for collaborative learning."
\end{enumerate}
	
\paragraph{Tutorbot Corpus: Evidence of Human-Agent Verbal Alignment in Second Language Learner Dialogues \citep{sinclair_tutorbot_2019}}
\begin{enumerate}
    \item ``We present a novel analysis of H-A and H-H L2 learner dialogues using automated metrics of alignment. Our contributions are twofold: firstly we replicated the reported H-A alignment within an educational context, finding L2 students align to an automated tutor."
    \item ``Secondly, we performed an exploratory comparison of the alignment present in comparable H-A and H-H L2 learner corpora using Bayesian Gaussian Mixture Models (GMMs), finding preliminary evidence that students in H-A L2 dialogues showed greater variability in engagement."
\end{enumerate}

\paragraph{Lexical entrainment and success in student engineering groups \citep{friedberg_lexical_2012}}
\begin{enumerate}
    \item compares to success, uses method by~\citet{nenkova_high_2008}
    \item ``Lexical Entrainment Score: Our group entrainment score is adapted from the pair score from~\citep{nenkova_high_2008}"
\end{enumerate}
 
\paragraph{[Thesis] Linguistic Entrainment in Multi-party Spoken Dialogues \citep{rahimi_linguistic_2019}}
\begin{enumerate}
    \item Advised by Diane Litman
    \item ``I explore the relation between entrainment on acoustic-prosodic and lexical features and show that they correlate.  In addition, I show that a multi-modal model using entrainment features from both of these modalities outperforms the uni-modal model at predicting team outcomes."
    \item ``Moreover, I present enhanced multi-party entrainment measures which utilize dynamics of entrainment in groups for both global and local settings.  As for the global entrainment, I present a weighted convergence based on group dynamics."
\end{enumerate}


\subsection{Other approaches to quantify alignment} \label{subsec: quantifying_alignment_papers}
% Reviewer 1: ``Finally, there is a wealth of methods for computationally computing alignment (again, search for other terms such as entrainment etc.) in dialogue besides the Dubuisson work that this paper builds upon, as well as for showing that the measures predict task success. The paper needs to be situated in this broader literature as well (some names to start with here include Julia Hirschberg, Cristian Danescu-Niculescu-Mizil, and David Reitter)."


\subsubsection{Julia Hirschberg}

\paragraph{Measuring Acoustic-Prosodic Entrainment with Respect to Multiple Levels and Dimensions \citep{levitan_measuring_2011}}
\begin{enumerate}
    \item ``In conversation, speakers become more like each other in various dimensions. This phenomenon, commonly called entrainment, coordination, or alignment, is widely believed to be crucial to the success and naturalness of human interactions."
    \item ``We investigate entrainment in four acoustic and prosodic dimensions: energy, pitch, speaking rate, and voice quality.  We explore whether speakers coordinate with each other in these dimensions over the conversation as a whole as well as on a turn-by-turn basis and in both relative and absolute terms, and whether this coordination improves over the course of the conversation."
    \item Dimensions: ``We distinguish between the similarity of a feature over the entire conversation, the product of a single coordination step at the start of the dialogue, and the degree to which a feature becomes more similar over the course of a conversation, reflecting an ongoing coordination process. We call the first aspect of entrainment proximity and the second convergence, an increase in proximity over time."
    \item ``The Columbia Games Corpus consists of twelve spontaneous dyadic conversations. In each session, a pair of subjects played three computer games requiring cooperation and communications. They were separated by a curtain to ensure that all communication was verbal."
    \item ``We find that all features exhibit proximity and synchrony at the turn level; at the session level, some features display proximity and some converge later in the conversation. Speakers entrain on different features in different ways, suggesting that it is important to be clear about exactly what is being measured when discussing enrainment."
\end{enumerate}

\paragraph{``Talk to me with left, right, and angles": Lexical entrainment in spoken Hebrew dialogue \citep{weise_talk_2021}}
\begin{enumerate}
    \item ``entrainment, affects lexical choice as well, both with regard to specific words, such as referring expressions, and overall style."
    \item ``We offer what we believe to be the first investigation of such lexical entrainment in \textbf{Hebrew}."
    \item ``Using two existing measures, we analyze Hebrew speakers interacting in \textbf{a Map Task}", a popular experimental setup, and find rich evidence of lexical entrainment"
    \item ``We do, however, find that speakers in a position of less power entrain more than those with greater power, which matches theoretical accounts." 
    \item  \textbf{lexical entrainment and aspects of the conversation:} ``there are correlations between lexical entrainment and interesting aspects of the conversation. These include task success for both speaker pairs (Reitter and Moore, 2007; Nenkova et al., 2008) and groups (Gonzales et al., 2010; Friedberg et al., 2012), conversation flow and perceived naturalness (Nenkova et al., 2008), as well as power differences between the speakers  \citep{danescu-niculescu-mizil_mark_2011}."
    \item \textbf{Power!} ``Speakers in subordinate roles are predicted to entrain more than those in power (Giles et al., 1991). This has been confirmed for lexical entrainment in English \citep{danescu-niculescu-mizil_mark_2011} and we find the same here. Followers, having less power due to their dependency on information from the leaders, entrain more than leaders with regard to their overall productions. Conversely, for directional terms alone, Silber-Varod et al. (2020) found that followers had greater influence on the terminology, that is, leaders adopted followers’ terms more often than vice versa."
\end{enumerate}

\paragraph{Individual differences in acoustic-prosodic entrainment in spoken dialogue \citep{weise_individual_2019}}
\begin{enumerate}
    \item ``We analyze individual differences in two forms of local, acoustic-prosodic entrainment in two large corpora between English and Chinese native speakers conversing in English"
    \item ``We find considerable variation in both degree and valence of entrainment behavior across speakers with some consistent trends, such as synchronous behavior being mostly positive in direction and somewhat more prevalent than convergence. However, we do not find entrainment to vary significantly based on gender, native language, or their combination."
\end{enumerate}

\paragraph{Acoustic-Prosodic and Lexical Entrainment in Deceptive Dialogue \citep{levitan_acoustic-prosodic_2018}}
\begin{enumerate}
    \item ``We analyze entrainment in acoustic-prosodic and lexical dimensions in a deceptive speech corpus of dialogues between native speakers of Mandarin Chinese and Standard American English, both speaking in English."
    \item ``Further, we identify differences in entrainment behavior between deceptive and truthful speech. These differences suggest that entrainment behavior can be a useful indicator of truthful and deceptive speech, with potential applications for automatic deception detection.
    we studied entrainment in four lexical features: 100 most frequent words, 25 most frequent words, hedge words/phrases, and cue phrases. 
    Entrainment in the use of the most frequent words in a dialogue or corpus has been studied by~\citet{nenkova_high_2008} and shown to be predictive of dialogue naturalness and correlated with task success. 
    \textbf{Hedge words and phrases} are used by speakers to express distance or lack of commitment to what they are saying (e.g. I think, sort of), and are a novel domain for entrainment analysis. 
    Cue phrases are linguistic expressions that function as explicit indicators of discourse structure, and have also not been previously studied in the context of entrainment. We used lists of hedge words and affirmative cue words that are available online 1."
\end{enumerate}

\paragraph{Implementing Acoustic-Prosodic Entrainment in a Conversational Avatar \citep{levitan_implementing_2016}}
\begin{enumerate}
    \item ``there has been little on entrainment in speech and even less on how Spoken Dialogue Systems which entrain to their users’ speech can be created."
    \item ``We present an architecture and algorithm for implementing acoustic-prosodic entrainment in SDS and show that speech produced under this algorithm conforms to the feature targets, satisfying the properties of entrainment behavior observed in human-human conversations."
    \item ``We present results of an extrinsic evaluation of this method, comparing whether subjects are more likely to ask advice from a conversational avatar that entrains vs. one that does not, in English, Spanish and Slovak SDS."
\end{enumerate}
	
	
\paragraph{Entrainment and Turn-Taking in Human-Human Dialogue \citep{levitan_entrainment_2015}}
\begin{enumerate}
    \item ``We investigate the relationship between entrainment and turn-taking."
    \item ``We show that speakers entrain on turn-taking behaviors such as the distribution of turn types and degree of latency between turns, and that entrainment at turn exchanges is related to some extent to the type of turn exchange."
    \item ``The experiments in this study were conducted on the \textbf{Columbia Games Corpus}~\citep{gravano_turn-taking_2009}, a corpus of twelve spontaneous, task-oriented dyadic conversations elicited from native speakers of Standard American English."
    \item ``During the collection of the corpus, each pair of participants played a set of computer games that required them to verbally cooperate to achieve a mutual goal.  Neither subject could see the other’s laptop screen"
    \item ``In the Cards games, one speaker (the information giver described the cards she saw on her screen, and her partner (the follower) attempted to match them to the cards on his own screen. 
    In the Objects games, one speaker (the giver described the location of an object on her screen, and her partner (the follower) attempted to place the corresponding object in exactly the same location on his own screen. 
    For both games, the participants received points based on how exact a match was; they later were paid for each point. Each of the twelve sessions consists of two Cards games and one Objects game."
\end{enumerate}

\paragraph{Pragmatic aspects of temporal accommodation in turn-taking \citep{benus_pragmatic_2011}}
\begin{enumerate}
    \item ``We study the timing of turn-initial single word grounding responses and conversational fillers." 
    \item ``Qualitative and quantitative analyses."
    \item ``Interlocutors accommodate the timing of these turn-initial responses to each other."
    \item ``Accommodation facilitates the creation of common ground and asymmetrical dominance relationship."
    ``This study investigates the relationship between the variability in the temporal alignment of turn initiations and the pragmatics of interpersonal communication."
    \item ``we examine the role of timing in establishing common ground, and test the hypothesis that the degree of accommodation to temporal and metrical characteristics of an interlocutor's speech is one aspect of turn-taking behavior that signals asymmetrical dominance relationships between interlocutors. 
    \item ``Our results show that dominance relationships linked to floor-control, as well as mutual common ground, are pragmatically constructed in part through the accommodation patterns in timing of turn-initial single word utterances."
\end{enumerate}


\paragraph{Acoustic-Prosodic Entrainment and Social Behavior \citep{levitan_acoustic-prosodic_2012}}
\begin{enumerate}
    \item `` We measure entrainment on eight acoustic features extracted from the speech of subjects playing a cooperative computer game and associate the degree of entrainment with a number of manually-labeled social variables acquired using Amazon Mechanical Turk, as well as objective measures of dialogue success."
    \item ``we asked Amazon Mechanical Turk annotators to label the 168 Objects games in our corpus for an array of social behaviors perceived for each of the speakers, which we term here `social variables.': Is the speaker trying to be liked? Is the speaker trying to dominate the conversation? Is the speaker giving encouragement to his/her partner? Is the conversation awkward?"
    \item `We find that male-female pairs entrain on all features, while male-male pairs entrain only on particular acoustic fea- tures (intensity mean, intensity maximum and syllables per second). We further determine that entrainment is more important to the perception of female-male social behavior than it is for same-gender pairs, and it is more important to the smoothness and flow of male-male dialogue than it is for female-female or mixed-gender pairs. 
    [W]e find that entrainment is more pronounced when intensity or speaking rate is especially high or low."
\end{enumerate}

\paragraph{High Frequency Word Entrainment in Spoken Dialogue \citep{nenkova_high_2008}}
\begin{enumerate}
    \item ``we examine novel types of entrainment in two corpora—Switchboard and the Columbia Games corpus."
    We examine entrainment in use of high-frequency words (the most common words in the corpus), and its association with dialogue naturalness and flow, as well as with task success."
    \item ``Our results show that such entrainment is predictive of the perceived naturalness of dialogues and is significantly correlated with task success; in overall interaction flow, higher degrees of entrainment are associated with more overlaps and fewer interruptions."
\end{enumerate}

\paragraph{Developing an Integrated Model of Speech Entrainment \citep{levitan_developing_2020}}
\begin{enumerate}
    \item Research proposal by Levitan herself
    \item ``Entrainment, the phenomenon of conversational partners’ speech becoming more similar to each other, is generally accepted to be an important aspect of human-human and human-machine communication."
    \item ``However, there is a gap between accepted psycholinguistic models of entrainment and the body of empirical findings, which includes a large number of unexplained negative results."
    \item ``Existing research does not provide insights specific enough to guide the implementation of entraining spoken dialogue systems or the interpretation of entrainment as a measure of quality."
    \item ``A more integrated model of entrainment is proposed, which looks for consistent explanations of entrainment behavior on specific features and how they interact with speaker, session, and utterance characteristics."
\end{enumerate}

\paragraph{[Thesis] Acoustic-Prosodic Entrainment in Human-Human and Human-Computer Dialogue \citep{levitan_acoustic-prosodic_2014}}
\begin{enumerate}
    \item did her thesis~\citep{levitan_acoustic-prosodic_2014} at Columbia University 2009-2014, working with Prof. Julia Hirschberg in the Spoken Language Processing Group. Then joined the Computer Science Department at Brooklyn College CUNY as an assistant professor.
    \item Thesis proposal:~\citep{levitan_entrainment_2013}
\end{enumerate}

\subsubsection{Cristian Danescu-Niculescu-Mizil}

\paragraph{Mark my words! linguistic style accommodation in social media \citep{danescu-niculescu-mizil_mark_2011}}
\begin{enumerate}
    \item ``The psycholinguistic theory of communication accommodation accounts for the general observation that participants in conversations tend to converge to one another's communicative behavior: they coordinate in a variety of dimensions including choice of words, syntax, utterance length, pitch and gestures."
    \item ``In its almost forty years of existence, this theory has been empirically supported exclusively through small-scale or controlled laboratory studies."
    \item ``Here we address this phenomenon in the context of Twitter conversations. Undoubtedly, this setting is unlike any other in which accommodation was observed and, thus, challenging to the theory. Its novelty comes not only from its size, but also from the non real-time nature of conversations, from the 140 character length restriction, from the wide variety of social relation types, and from a design that was initially not geared towards conversation at all. Given such constraints, it is not clear a priori whether accommodation is robust enough to occur given the constraints of this new environment."
    \item ``To investigate this, we develop a probabilistic framework that can model accommodation and measure its effects. We apply it to a large Twitter conversational dataset specifically developed for this task."
    \item ``This is the first time the hypothesis of linguistic style accommodation has been examined (and verified) in a large scale, real world setting. Furthermore, when investigating concepts such as stylistic influence and symmetry of accommodation, we discover a complexity of the phenomenon which was never observed before."
    \item ``We also explore the potential relation between stylistic influence and network features commonly associated with social status."
\end{enumerate}

\paragraph{Chameleons in imagined conversations: A new approach to understanding coordination of linguistic style in dialogs \citep{danescu-niculescu-mizil_chameleons_2011}}
\begin{enumerate}
    \item ``Conversational participants tend to immediately and unconsciously adapt to each other's language styles: a speaker will even adjust the number of articles and other function words in their next utterance in response to the number in their partner's immediately preceding utterance."
    \item ``This striking level of coordination is thought to have arisen as a way to achieve social goals, such as gaining approval or emphasizing difference in status. But has the adaptation mechanism become so deeply embedded in the language-generation process as to become a reflex?"
    \item ``We argue that fictional dialogs offer a way to study this question, since authors create the conversations but don't receive the social benefits (rather, the imagined characters do)."
    \item ``Indeed, we find significant coordination across many families of function words in \textbf{our large movie-script corpus}. We also report suggestive preliminary findings on the effects of gender and other features; e.g., surprisingly, for articles, on average, characters adapt more to females than to males."
\end{enumerate}

\paragraph{[Thesis] A Computational Approach To Linguistic Coordination \citep{danescu-niculescu-mizil_computational_2012}}



\subsubsection{David Reitter}

\paragraph{An Evaluation and Comparison of Linguistic Alignment Measures \citep{xu_evaluation_2015}}
\begin{enumerate}
    \item ``Linguistic alignment has emerged as an important property of conversational language and a driver of mutual understanding in dialogue. While various computational measures of linguistic alignment in corpus and experimental data have been devised, a systematic evaluation of them is missing."
    \item ``In this study, we first evaluate the sensitivity and distributional properties of three measures, indiscriminate local linguistic alignment ({LLA}), Spearman’s correlation coefficient ({SCC}), and repetition decay ({RepDecay})."
    \item ``Then we apply them in a study of interactive alignment and individual differences to see how well they conform to the Interactive Alignment Model ({IAM}), and how well they can reveal the individual differences in alignment propensity."
    \item ``Our results suggest that {LLA} has the overall best performance."
\end{enumerate}

\paragraph{Alignment and task success in spoken dialogue \citep{reitter_alignment_2014}}
\begin{enumerate}
    \item ``New methods to quantify structural priming across all syntactic choices in corpora of speech, dialogue or text."
    \item ``We test of two predictions from Interactive Alignment Theory~\citep{pickering_towards_2004}"
    \item ``We find priming within and between speakers; stronger in task-oriented dialogue."
    \item ``Long-term adaptation is correlated with success in task-oriented dialogue, confirming the Interactive Alignment Model."
    \item ``Lexical and syntactic material together can predict success in task-oriented dialogue."
    \item (H1: syntatic alignment more in task-oriented) ``We hypothesize that there is a tendency for dialogue partners to repeat syntactic structure within brief time windows, and that they do more so in task-oriented dialogue than in spontaneous conversation."
    \item (H2: higher syntatic alignment, higher success) ``The IAM predicts that task-oriented dialogues that exhibit more syntactic adaptation between the interaction partners will ultimately yield more task success."
\end{enumerate}

\paragraph{Predicting Success in Dialogue \citep{reitter_predicting_2007}}
\begin{enumerate}
    \item ``Task-solving in dialogue depends on the linguistic alignment of the interlocutors, which \citet{pickering_towards_2004} have suggested to be based on mechanistic repetition effects."
    \item ``we seek confirmation of this hypothesis by looking at repetition in corpora, and whether repetition is correlated with task success. 
    \item ``We show that the relevant repetition tendency is based on slow adaptation rather than short-term priming and demonstrate that lexical and syntactic repetition is a reliable predictor of task success given the first five minutes of a task oriented dialogue.
\end{enumerate}

\paragraph{Priming of Syntactic Rules in Task-Oriented Dialogue and Spontaneous Conversation \citep{reitter_priming_2006}}
\begin{enumerate}
    \item ``The present paper extends these results by investigating priming effects involving arbitrary syntactic rules in spoken dialogue corpora."
    \item ``We demonstrate the existence of within- and between-speaker priming in both spontaneous conversation (the Switchboard corpus) and task-oriented dialogue (the Map Task corpus)."
    \item ``We also find that between-speaker priming is stronger in the Map Task corpus. This supports the hypothesis that in task-oriented dialog, low-level priming is linked to higher-level alignment of situation models." \dots ``Unlike Switchboard, Map Task contains \emph{task-oriented dialogue}: interlocutors work together to achieve a task as quickly and efficiently as possible."
    \item ``we examined two spoken-language corpora with respect to \textbf{structural repetition}: both contain transcriptions of spoken dilogue and phrase-structure-based syntactic tree annotation." - syntactic repetition
    \item ``Syntactic priming as an instance of general priming or pre-activation is an almost universal effect. We know, however, that some control is exerted by the conditions of the dialogue and possibly by speakers tailoring their utterances to match the needs of their audience. Still, we would expect to find syntactic priming in the task-oriented dialogue of Map Task."
    \item ``Both corpora of spoken dialogue we investigated showed an effect of distance between prime and target in syntactic repetition, thus providing evidence for a structural priming effect for arbitrary syntactic rules"
\end{enumerate}

\paragraph{Computational Modelling of Structural Priming in Dialogue \citep{reitter_computational_2006}}
\begin{enumerate}
    \item ``Syntactic priming effects, modelled as increase in repetition probability shortly after a use of a syntactic rule, have the potential to improve language processing components." 
    \item ``We model priming of syntactic rules in annotated corpora of spoken dialogue, extending previous work that was confined to selected constructions. "
    \item ``We find that speakers are more receptive to priming from their interlocutor in task-oriented dialogue than in spontaneous conversation. Low-frequency rules are more likely to show priming."
\end{enumerate}
    
\paragraph{A Computational Cognitive Model of Syntactic Priming \citep{reitter_computational_2011}}
\begin{enumerate}
    \item ``The psycholinguistic literature has identified two syntactic adaptation effects in language production: rapidly decaying short-term priming and long-lasting adaptation."
    \item ``To explain both effects, we present an {ACT}-R model of syntactic priming based on a wide-coverage, lexicalized syntactic theory that explains priming as facilitation of lexical access."
    \item ``Our model simulates incremental language production and in a series of modeling studies, we show that it accounts for 
    (a) the inverse frequency interaction; 
    (b) the absence of a decay in long-term priming; and 
    (c) the cumulativity of long-term adaptation.
    \item ``The model also explains the lexical boost effect and the fact that it only applies to short-term priming."
    \item ``We also present corpus data that verify a prediction of the model, that is, that the lexical boost affects all lexical material, rather than just heads."
\end{enumerate}

\paragraph{Not that much power: Linguistic alignment is influenced more by low-level linguistic features rather than social power \citep{xu_not_2018}}
\begin{enumerate}
    \item ``A common finding has been that interlocutors of higher power tend to receive more alignment than those of lower power. However, these studies overlook some low-level linguistic features that can also affect alignment, which casts doubts on these findings.`
    \item ``This work characterizes the effect of power on alignment with logistic regression models in two datasets, finding that the effect vanishes or is reversed after controlling for low-level features such as utterance length. Thus, linguistic alignment is explained better by low-level features than by social power."
    \item ``We argue that a wider range of factors, especially cognitive factors, need to be taken into account for future studies on observational data when social factors of language use are in question."
    \item Power?  ``The Communication Accommodation Theory (Giles, 2008) states that the social power of speakers influence the extent to which conversation partners accommodate (or align, coordinate) their communicating styles towards them. \dots  Typically, people of lower power converge their linguistic styles to those of higher power; for example, interviewees towards interviewers (Willemyns et al., 1997), or students towards teachers (Jones et al., 1999)"
\end{enumerate}

\paragraph{How Emotional Support and Informational Support Relate to Linguistic Alignment \citep{wang_how_2017}}
\begin{enumerate}
    \item ``Do the two lower-level alignment measures (lexical and syntactic) relate to these two types of social support in the same way or, are they different?"
    \item ``Our hypothesis was that they are similar, due to their correlation relationship. However, we found that, based on an analysis of a 10-year online forum for cancer survivors, the lower-level alignment measures have distinct relationships to the two higher-level support functions."
    \item ``In this paper, we describe this finding and its implications regarding potential refinement of the Interactive Alignment Model"
\end{enumerate}

\paragraph{Linguistic Adaptation in Conversation Threads: Analyzing Alignment in Online Health Communities \citep{wang_linguistic_2014}}
\begin{enumerate}
    \item ``Linguistic alignment at lexical and syntactic levels, as well as decay of alignment was observed in forum threads, although the decay was slower than commonly found in psycholinguistic studies. Previous studies of alignment have focused on two-party conversations. We study multi-party conversation in online health communities, which have shown benefits for their members from forum conversations."
    \item ``This paper quantifies linguistic alignment in the oldest and the largest cancer online forum."
    \item ``The different pattern of adaptation to the initial post on a thread suggests that specific roles in the online forum (e.g., seeking support from the community) can potentially be revealed through alignment theory and its extensions."
\end{enumerate}

\paragraph{Pragmatic Alignment on Social Support Type in Health Forum Conversations \citep{wang_pragmatic_2015}}
\begin{enumerate}
    \item ``While adaptation can occur at lexical, syntactic and pragmatic levels, relationships between alignments at multiple levels are neither theoretically nor empirically well understood."
    \item ``In this study, we find that community members show pragmatic alignment on social support type, distinguishing emotional and informational support, both of which provide benefits to members."
    \item ``We also find that lexical alignment is correlated with emotional support."
    \item ``This finding can contribute to our understanding of the linguistic signature of different types of support as well as the theory of Interactive Alignment in dialogue."
\end{enumerate}

\paragraph{Alignment in Web-based Dialogue: Who Aligns, and How Automatic Is It? Studies in Big-Data Computational Psycholinguistics \citep{reitter_alignment_2016}}
\begin{enumerate}
    \item ``survey studies on linguistic alignment in order to connect the inferences we make from large datasets to the psycholinguistics of dialogue."
    \item ``This work is motivated by a high-level question: How does our mind select and combine words in a way that reliably communicates our intentions to a dialogue partner? The search for a computational answer to this question has been revitalized in recent years by the advent of large datasets."
    \item ``Large data give us a window into an individual’s mind and a cooperative process between minds. It allows us to look at how dialogue partners gradually converge in their choices of words and sentence structure, thereby creating a shared language."
\end{enumerate}

\paragraph{[Thesis] Context Effects in Language Production: Models of Syntactic Priming in Dialogue Corpora \citep{reitter_context_2008}}
\begin{enumerate}
    \item ``This thesis addresses the cognitive basis of syntactic adaptation, which biases speakers to repeat their own syntactic constructions and those of their conversational partners. 
    I address two types of syntactic adaptation: short-term priming and long-term adaptation"
\end{enumerate}




\subsubsection{Others}

\paragraph{Measuring Adaptation Between Dialogs \citep{stenchikova_measuring_2007}}
\begin{enumerate}
    \item ``The paper proposes two new approaches for measuring adaptation between dialogs. These approaches permit measurement of adaptation both to conversational partner (partner adaptation) and to the local dialog context (recency adaptation), and can be used with different types of feature."
    \item ``We used these measures to study adaptation in the Maptask corpus of spoken dialogs."
    \item ``We show that for syntactic features, recency adaptation is stronger than partner adaptation; however, we find no significant differences for lexical adaptation using these measures."
\end{enumerate}

\paragraph{A unifying framework for modeling acoustic/prosodic entrainment: definition and evaluation on two large corpora \citep{galvez_unifying_2020}}
\begin{enumerate}
    \item cites \citep{levitan_entrainment_2015,levitan_measuring_2011,nenkova_high_2008}
\end{enumerate}

\paragraph{Measuring prosodic alignment in cooperative task-based conversations \citep{truong_measuring_2012}}
\begin{enumerate}
    \item ``we investigate prosodic alignment in task-based conversations. We use the {HCRC} Map Task Corpus and investigate how familiarity affects prosodic alignment and how task success is related to prosodic alignment."
    \item ``A variety of existing alignment measures is used and applied to our data. In particular, a windowed cross-correlation procedure, that has been used previously in visual behavior research, is applied to prosodic features"
    \item ``Alignment tendencies are strongest for intensity, and familiarity seems to play a role in convergence. Finally, \textbf{weak evidence was found for a correlation between prosodic alignment measures and task success}"
\end{enumerate}

\paragraph{Lexical Entrainment and Intra-Speaker Variability in Cooperative Dialogues \citep{menshikova_lexical_2021}}
\begin{enumerate}
    \item cites \citep{weise_talk_2021,weise_individual_2019,levitan_measuring_2011} \dots
    \item ``we measured lexical entrainment in a series of dialogues, where each one of 20 “core” speakers talked to five different interlocutors: a sibling, a close friend, an unfamiliar person of the same gender and similar age, an unfamiliar person of the other gender and similar age, and an unfamiliar person of the same gender, greater age and higher job position."
    \item `` Our data have shown that a person speaks very similarly to his/her sibling; dialogues with a friend or a same- gender stranger of similar age show fewer similarities; the least `common language' is observed in dialogues with a stranger of the opposite gender and with a stranger of greater age and higher job position."
    \item ``Speech entrainment is manifested at all levels of linguistic analysis: syntactic [10], lexical [11], and phonetic [2]. This paper deals with lexical entrainment. But, along with lexemes, we are also analysing word forms—which makes this research related to syntax and pragmatics as well."
    \item ``To determine the extent to which task success is related to the degree of entrainment in high-frequency word usage, we examined 48 dialogues"
    \item ``We computed the correlation coefficient between the game score (normalized by the highest achieved score for the game type) and two different ways of quantifying the degree of entrainment between the speakers (S1 and S2) in several word classes. In addition to overall high-frequency words, we looked at two subclasses of words often used in dialogue:
    25MF-G The 25 most frequent words in the game.
    25MF-C The 25 most frequent words over the entire corpus: the, a, okay, and, of, I, on, right, is, it, that, have, yeah, like, in, left, it’s, uh, so, top, um, bottom, with, you, to.
    ACW Affirmative cue words: alright, gotcha, huh, mm-hm, okay, right, uh-huh, yeah, yep, yes, yup. 
    There are 5831 instances in the corpus (7.9\% of all words).
    FP Filled pauses: uh, um, mm. The corpus contains 1845 instances of filled pauses (2.5\% of all tokens)."
\end{enumerate}


\paragraph{A Robust Framework for Estimating Linguistic Alignment in Twitter Conversations \citep{doyle_robust_2016}}
\begin{enumerate}
    \item cites / follows up on \citep{danescu-niculescu-mizil_mark_2011}
    \item \dots
\end{enumerate}


\paragraph{Multi-Level Linguistic Alignment in a Virtual Collaborative Problem-Solving Task \citep{duran_multi-level_2021}}
\begin{enumerate}
    \item ``Co-creating meaning in conversation is challenging. Success is often determined by people's abilities to coordinate their language in strategic ways to signal problems and to align mental representations."
    \item ``We explore one set of grounding mechanisms, known as interactive linguistic alignment, that makes use of the ways people re-use, i.e., `align to,' the lexical, semantic, and syntactic forms of others’ utterances."
    \item ``In particular, the focus is on the temporal development of multi-level linguistic alignment and examine how its expression is related to communicative outcomes within a unique collaborative problem-solving paradigm." 
    \item ``The primary task, situated within an educational video game, requires creative thinking between three people where the paths for possible solutions are highly variable."
    \item ``We find that over time interactions are marked by decreasing lexical and syntactic alignment, with a trade-off of increasing semantic alignment."
    \item ``However, a greater semantic alignment does not necessarily translate into better team performance." 
    \item ``Overall, these findings provide greater clarity on the role of grounding mechanisms in complex and dynamic collaborative problem-solving tasks."
\end{enumerate}

\paragraph{Language Style Matching as a Predictor of Social Dynamics in Small Groups \citep{gonzales_language_2010}}
\begin{enumerate}
    \item ``Synchronized verbal behavior can reveal important information about social dynamics."
    \item ``This study introduces the linguistic style matching (LSM) algorithm for calculating verbal mimicry based on an automated textual analysis of function words."
    \item ``The LSM algorithm was applied to language generated during a small group discussion in which 70 groups comprised of 324 individuals engaged in an information search task either face-to-face or via text-based computer-mediated communication."
    \item ``As a metric, LSM predicted the cohesiveness of groups in both communication environments, and it predicted task performance in face-to-face groups."
    \item ``Other language features were also related to the groups' cohesiveness and performance, including word count, pronoun patterns, and verb tense."
    \item ``The results reveal that this type of automated measure of verbal mimicry can be an objective, efficient, and unobtrusive tool for predicting underlying social dynamics."
    \item ``In total, the study demonstrates the effectiveness of using language to predict change in social psychological factors of interest."
\end{enumerate}

\paragraph{Linguistic Style Matching in Social Interaction \citep{niederhoffer_linguistic_2002}}
\begin{enumerate}
    \item ``Three experiments were conducted to determine the psychometric properties of language in dyadic interactions."
    \item ``Using text-analysis, it was possible to assess the degree to which people coordinate their word use in natural conversations."
    \item ``In Experiments 1 (n = 130) and 2 (n = 32), college students interacted in dyadic conversations in laboratory-based private Internet chat rooms."
    \item ``Experiment 3 analyzed the official transcripts of the Watergate tapes involving the dyadic interactions between President Richard Nixon and his aids H. R. Haldeman, John Erlichman, \& John Dean."
    \item ``The results of the three studies offer substantial evidence that individuals in dyadic interactions exhibit linguistic style matching (LSM) on both the conversation level as well as on a turn-by-turn level."
    \item ``Furthermore, LSM is unrelated to ratings of the quality of the interaction by both participants and judges.
    \item ``We propose that a coordination-engagement hypothesis is a better description of linguistic behaviors than the coordination-rapport hypothesis that has been proposed in the nonverbal literature."
\end{enumerate}

\paragraph{Do (and Say) as I Say: Linguistic Adaptation in Human–Computer Dialogs \citep{koulouri_and_2016}}
\begin{enumerate}
    \item ``This article provides an account of lexical alignment in human–computer dialogs, based on empirical data collected in a simulated human–computer interaction scenario."
    \item ``The results indicate that alignment is present, resulting in the gradual reduction and stabilization of the vocabulary-in-use, and that it is also reciprocal."
    \item ``Further, the results suggest that when system and user errors occur, the development of alignment is temporarily disrupted and users tend to introduce novel words to the dialog."
    \item ``lower alignment is associated with less successful interaction, as measured by user perceptions."
\end{enumerate}

\paragraph{Linguistic alignment is affected more by lexical surprisal rather than social power \citep{xu_linguistic_2019}}
\begin{enumerate}
    \item no abstract
    \item ``2.2  Characterize alignment with GLM: We formulate alignment as the impact of usingcertain linguistic markers in the preceding utterance (prime) on their chance to appear again in the following utterance (target)." 
    \item ``The linguistic markers examined here are 14 LIWC categories~\citep{pennebaker_linguistic_2001} as shown in Table 1." - LIWC: Linguistic inquiry and word count - tool
    \item ``We use generalized linear models (GLMs), in which the occurrence of linguistic markers (binary) in target as the response variable; the predictor is their occurrence (frequency count) in prime."
    \item ``Thus alignment is characterized by the coefficient of the predictor. Larger (positive) indicates stronger influence from prime on target, i.e., stronger alignment."
\end{enumerate}

\paragraph{ALIGN: Analyzing linguistic interactions with generalizable techNiques—A Python library \citep{duran_align_2019}}
\begin{enumerate}
    \item ``One barrier to more systematic investigation of these effects lies in the diversity in the methods employed to analyze {LA}, which makes it difficult to integrate and compare results of individual studies."
    \item ``To overcome this issue, we have developed {ALIGN} (Analyzing Linguistic Interactions with Generalizable {techNiques}), an open-source Python package to measure {LA} in conversation."
\end{enumerate}
	
\paragraph{[Thesis] Coordination: Theoretical, Methodological, and Experimental Perspectives \citep{paxton_coordination_2015}}
\begin{enumerate}
    \item coordination terminology
    \item ``Not only are there more than a dozen terms used to describe the phenomenon, but there is little to no consensus about their relation to one another. : An inexhaustive list includes accommodation, adaptation, alignment, contagion, congruency, coordination, coupling, entrainment, imitation, mimicry, social tuning, synchrony, and synergy."
\end{enumerate}


\paragraph{Modeling Linguistic and Personality Adaptation for Natural Language Generation \citep{hu_modeling_2018}}
\begin{enumerate}
    \item ``We propose an adaptation measure for adaptive natural language generation for dialogs that integrates the predictions of both personality theories and adaptation theories, that can be applied as a dialog unfolds, on a turn by turn basis." 
    \item ``We show that our measure meets criteria for validity, and that adaptation varies according to corpora and task, speaker, and the set of features used to model it."
    \item ``We also produce fine-grained models according to the dialog segmentation or the speaker, and demonstrate the decaying trend of adaptation. For this purpose, previous measures of dialog adaptation~\citep{stenchikova_measuring_2007,danescu-niculescu-mizil_mark_2011} have two limitations:
    (1) their calculation require the complete dialog, and 
    (2) they focus on single features and do not provide a model to control the interaction of multiple parameters in a single output, while our method measures adaptation with respect to any set of features."
\end{enumerate}

\paragraph{[Thesis] Quantification of Mutual Understanding in Task-Based Human-Human Interactions \citep{reverdy_quantification_2021}}
\begin{enumerate}
    \item base method: \citep{vogel_measuring_2012,vogel_attribution_2013}
    \item Reverdy's papers: \citep{reverdy_measuring_2017,reverdy_linguistic_2017}
    \item cites \citep{dubuisson-duplessis_automatic_2017}
    \item ``compares repetition patterns to different communicative assessment methods, namely task-success scores, presence of high levels of negative/positive cognitive states, and third-party moderator evaluation. Five corpora with a total of 192 dialogues (about 32 hours) are analysed in terms of other-shared and self-shared repetitions, at different levels of linguistic representations and utterance lengths."
    \item ``The main contribution of this thesis is the establishment of the extent to which repetitions– categorised as happening outside chance variation – may function as a proxy measure of mutual understanding. Results suggest a higher proportion of other than self -repetitions happening above chance in task-based interactions."
\end{enumerate}

\paragraph{Measuring Synchrony in Task-Based Dialogues \citep{reverdy_measuring_2017}}
\begin{enumerate}
    \item ``In many contexts from casual everyday conversations to formal discussions, people tend to repeat their interlocutors, and themselves. This phenomenon not only yields random repetitions one might expect from a natural Zipfian distribution of linguistic forms, but also projects underlying discourse mechanisms and rhythms that researchers have suggested establishes conversational involvement and may support communicative progress towards mutual understanding."
    \item ``In this paper, advances in an automated method for assessing interlocutor synchrony in \textbf{task-based} Human-to-Human interactions are reported."
    \item ``The method focuses on dialogue structure, rather than temporal distance, \textbf{measuring repetition between speakers and their interlocutors last n-turns (n = 1, however far back in the conversation that might have been) rather than utterances during a prior window fixed by duration.}"
    \item ``The significance of distinct linguistic levels of repetition are assessed by observing contrasts between actual and randomized dialogues, in order to provide a quantifying measure of communicative success."
    \item ``Definite patterns of repetitions where identified, notably in contrasting the role of participants (as information giver or follower)."
    \item ``The extent to which those interacted sometime surprisingly with gender, eye-contact and familiarity is the principal contribution of this work."
\end{enumerate}

\paragraph{Linguistic repetitions, task-based experience and a proxy measure of mutual understanding \citep{reverdy_linguistic_2017}}
\begin{enumerate}
    \item ``Diverse conversational mechanisms are involved in developing a common ground, and \textbf{repetition phenomena appear to be strongly connected to these processes}. 
    \item ``This article describes the use of an automatic method to detect, within dialogue transcripts, linguistic cues of engagement and synchrony, by observing repetitions at different linguistic levels."
    \item ``We focus on the relationship between repetition patterns and task-based success in interaction with task-based experience and partner familiarity."
    \item ``We conduct our analysis on the data of the HCRC Map Task corpus."
    \item ``Results suggests that, among other patterns, significant amounts of repetitions play a role for unfamiliar participants, with greater success, in particular, at first attempts."
\end{enumerate}

\paragraph{Attribution of Mutual Understanding \citep{vogel_attribution_2013}}
\begin{enumerate}
    \item ``This article explores advances in a method of analysis of conversational interaction, as recorded through text transcripts, for evidence of grounding in order to quantify certainty of mutual understanding."
    \item ``a method is described for analyzing interaction in dialogue with respect to interlocutor alignment: \dots For each transcript processed, the algorithm for data extraction designates a location of memory called a `register' for each speaker. The register, which is initially empty, eventually contains the contents of the most recent contribution of the corresponding speaker. A generalization of the method would afford each speaker a vector of registers in order to evaluate repetitions arbitrarily far back in a conversation."
\end{enumerate}
	
\paragraph{Measuring Synchrony in Dialog Transcripts \citep{vogel_measuring_2012}}
\begin{enumerate}
    \item A finite register method of processing dialog transcripts is used to measure interlocutor synchrony. Successive contributions by participants are measured for word n-gram repetitions and temporal overlaps."
    \item ``The Zipfian distribution of words in language use leads to a natural expectation that random re-orderings of dialog contributions will unavoidably exhibit repetition – one might reasonably expect that the frequency of repetition in actual dialog is in fact best explained as a random effect."
    \item ``Repetition in actual dialog exceeds the frequency one might expect from a random process. Perhaps surprisingly from the perspective of using repetition as an index of synchrony, self-repetition significantly exceeds allo-repetition."
\end{enumerate}

\paragraph{I Wanna Talk Like You: Speaker Adaptation to Dialogue Style     in L2 Practice Conversation \citep{sinclair_i_2019}}
\begin{enumerate}
    \item ``We present a novel method to analyse speaker alignment in second language practice dialogue. Our method represents utterances as Dialogue Acts and applies Epistemic Network Analysis to their use."
    \item ``ENA makes convergence between speakers visible, and enables us to confirm hypotheses that both initial similarity and final convergence increase with student ability; and that Dialogue Act use changes with ability, and over the course of an interaction."
    \item ``Our results can inform personalised automatic tutoring tools as well as formative assessment and feedback."
\end{enumerate}

\paragraph{Alignment in a Multimodal Interlingual Computer-Mediated Map Task Corpus \citep{reverdy_alignment_2018}}
\begin{enumerate}
    \item ``This work presents an assessment of interlocutor alignment using a semi-automated method in the context of multimodal interlingual (English-Portuguese) computer-mediated interactions."
    \item ``We study the adaptation phenomenon (also known as convergence behaviour and alignment behaviour) by looking at verbal repetition at different levels of linguistic representation."
    \item ``First, we compare repetitions patterns in task-oriented dialogues of human-to-human communication ({HCRC} Edinburgh Map Task corpus) and interlingual computer-mediated human-to-human communication ({ILMT}-s2s corpus), for eye-contact and no eye-contact scenarios. Secondly, we study the relation between the cognitive state of the subject, and the alignment process in interlingual computer-mediated communication settings."
    \item ``Results show that above chance repetitions, signalling verbal alignment, are present in both direct human-to-human communication and interlingual computer-mediated interactions, and that interlingual computer-mediated setting yields significantly more self-repetitions than direct human-to-human interactions."
    \item ``Also, in interlingual computer-mediated communication, a lack of alignment cues for long sequences correlated with a high amount of negative cognitive states in the eye-contact setting, implying a potential lack of mutual understanding."
\end{enumerate}

\paragraph{Linguistic Repetition in Three-Party Conversations \citep{reverdy_linguistic_2020}}
\begin{enumerate}
    \item ``We report on three-party game-based interactions where two players participate in a quiz supervised by a facilitator."
    \item ``We use a semi-automatic method to detect alignment between players by observing linguistic repetitions in the dialogue transcripts and investigate the relation of the alignment to the type of the facilitator’s feedback."
    \item ``Results suggest that the repetitions detected with this method have a function in the interaction, as it is reflected in the verbal and non-verbal behaviours of an interaction facilitator: facilitators provided more encouragement than expected where alignment lacked evidence and less than expected where alignment was ample."
    \item ``The study presented here exploits the MULTISIMO corpus [18], a multimodal corpus consisting of 23 sessions of collaborative group interactions, where two players work together to provide answers to a quiz and are guided by a facilitator, who monitors their progress and provides feedback or hints when needed." \dots ``two annotation layers were introduced: the first annotation layer includes the values of positive, neutral and negative feedback"
    \item ``We counted the repetition of tokens of a contribution and the immediately preceding contributions~\citep{vogel_measuring_2012,vogel_attribution_2013} count self-repetition (SelfShared) and other-repetition (OtherShared). We note that among OtherShared, the repetitions counted are those of the other player and of the facilitator.
\end{enumerate}

\paragraph{Persistent Lexical Entrainment in HRI \citep{brandstetter_persistent_2017}}
\begin{enumerate}
    \item ``does lexical entrainment with a robot interlocutor persist after an interaction?"
    \item ``what role is played by personality traits in lexical entrainment to robots, and how does this compare with the role of personality in entrainment to other humans?"
    \item ``Our experiment shows that first, robots can indeed prompt lexical entrainment that persists after an interaction is over." This finding is interesting since it demonstrates that speakers can be linguistically influenced by a robot, in a way that is not merely motivated by a desire to be understood. Second, we find similarities between lexical entrainment to the robot peer and lexical entrainment to a human peer, although the effects are stronger when the peer is human. Third, we find that whether the peer is a robot or a human, similar personality traits contribute to lexical entrainment. In both peer conditions, participants who score higher on ``Openness to experience" are more likely to adopt less conventional terminology."
\end{enumerate}

\paragraph{Exploring the Effects of a Social Robot's Speech Entrainment and Backstory on Young Children's Emotion, Rapport, Relationship, and Learning \citep{kory-westlund_exploring_2019}}
\begin{enumerate}
    \item ``In positive human-human relationships, people frequently mirror or mimic each other’s behavior. This mimicry, also called entrainment, is associated with rapport and smoother social interaction. Because rapport in learning scenarios has been shown to lead to improved learning outcomes, we examined whether enabling a social robotic learning companion to perform rapport-building behaviors could improve children’s learning and engagement during a storytelling activity."
    \item ``3.8. Entrainment: In the Entrainment condition, the speaking rate and pitch of the robot's voice were automatically adjusted to be more similar to the child. In addition, the robot’s volume and exuberance were manually adapted by the teleoperator."
\end{enumerate} 

\paragraph{Lexical Entrainment in Human Robot Interaction \citep{iio_lexical_2015}}
\begin{enumerate}
    \item \dots
\end{enumerate}


\paragraph{Looking for Structure in Lexical and Acoustic-Prosodic Entrainment Behaviors \citep{weise_looking_2018}}
\begin{enumerate}
    \item ``Motivated by cognitive theories regarding linguistic entrainment, we analyze speakers' overall entrainment behaviors and search for an underlying structure. We consider various measures of both acoustic-prosodic and lexical entrainment, measuring the latter with a novel application of two previously introduced methods in addition to a standard high-frequency word measure."
    \item ``We present a negative result of our search, finding no meaningful correlations, clusters, or principal components in various entrainment measures, and discuss practical and theoretical implications."
\end{enumerate}


% \paragraph{Lexical entrainment without conceptual pacts? Revisiting the matching task \citep{bangerter_lexical_2020}}

==> sections/revised/results.tex <==
\section[Results and Discussion]{Results and Discussion\footnote{The code that reproduces all the results and figures given in this paper are available from the Zenodo Repository, DOI:~\href{https://sandbox.zenodo.org/record/742549}{10.5072/zenodo.742549}}} \label{sec:results}

\subsection{RQ1: How do the interlocutors use task-specific referents? Does this link to task success?} \label{subsec:results_rq1}

\subsubsection*{H1.1: Task-specific referents become routine early for more successful teams.} \label{subsec:results_h1_1}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/h1_1_time_absolute_plot.pdf}
    \caption{The team's establishment times for H1.1. The teams are sorted by decreasing task performance (i.e.\ increasing \measure{error}). The boxplots, with the same colour have the same \measure{error} (sorted by increasing duration for the ties). The thick, bold boxplots with whiskers with maximum 1.5 IQR show the distributions of the establishments that occurred in the common duration (i.e.\ as marked by the dashed green line), while the thin boxplots show the distributions through the total duration of interaction. The learning outcome of each team is indicated with a plus (`+') for $\measure{learn} > 0$, or a minus (`-') otherwise. Solid lines indicate the end of the interaction, by submitting a correct solution (in green) or timing out (in red). The thin blue lines indicate submission of a solution, with the number showing the error quantifying how far the submitted solution is from an optimal solution in terms of its cost (e.g.\ $\measure{error} = 0\%$ means the team has found an optimal solution). The red and blue dots indicate the utterance times of the interlocutors, to give an idea of when the interlocutors are speaking versus when are their establishment times.} \label{fig:h1_1_time_absolute_plot}
\end{figure}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/h1_1_time_plot.pdf}
    \caption{The teams' establishment times as normalised by the duration for each team separately, i.e.\ 100\% indicates the end of that team's interaction. Sorting is as in Fig.~\ref{fig:h1_1_time_absolute_plot}.} \label{fig:h1_1_plot}
\end{figure}

\paragraph{For task performance.}
Fig.~\ref{fig:h1_1_time_absolute_plot} shows for each team the distribution of the establishment times of the routines. The median establishment times for all of the routines is strongly positively correlated with the task performance measure \measure{error} (Spearman's $\rho =0.69$, $p < .05$), that is, better-performing teams establish routines earlier\footnote{The magnitude of Spearman's correlation coefficient ($\rho$) can be interpreted by using the thresholds e.g.\ from~\citet{evans_straightforward_1996}, i.e.\ $0.00-0.19$ ``very weak", $0.20-0.39$ ``weak", $0.40-0.59$ ``moderate", $0.60-0.79$ ``strong", and $0.80-1.00$ ``very strong" \label{foot:spearman_groups}.}. We see from the figure that the results are influenced by the variation in the duration of the activity: the interaction ends for the well-performing teams when they find a correct solution, whereas the badly-performing teams continue their interaction until the experimenters intervene and stop the activity. Inspecting the distribution of the routines that are established in the common duration, i.e.\ first $\approx 11$ mins, we see that there is a moderate correlation coefficient between the establishment times and \measure{error} ($\rho =0.52$, $p = .15$), neglecting Team 18, which established no routines at all during this period and spoke very little in this common duration. Once we normalise the establishment times by the duration for each team separately, we see that the normalised median establishment times has a positive, medium Spearman's correlation coefficient ($\rho =0.38$, $p = .28$), indicating a general trend that establishments occur earlier for the better-performing teams. Fig.~\ref{fig:h1_1_plot} shows the normalised establishment times.

While it is expected that better-performing teams have established routines, from the figures we observe even badly-performing teams still successfully established routines. All teams, regardless of performance, have aligned to some degree. Focusing on Fig.~\ref{fig:h1_1_plot}, the establishment tends to occur around the middle of the dialogue: establishment times have mean of the medians~$= 63.0\%$ (combined $SD = 22.2\%$). While we hypothesised that establishment will happen early in the dialogue, this is the case for an ideal dialogue; people will `share' expressions earlier. However, we observe that there is an \emph{exploratory} period (roughly the period before Q1), where the interlocutors take the time to understand the task, followed by a \emph{collaborative} period that corresponds to the establishment period (roughly the period between Q1 and Q3). We expect that if the interlocutors had to complete the task again, the establishment/collaborative period would be closer to the start of the dialogue.

We observe that five teams (7, 8, 10, 18, and 47) that could not find a correct solution started collaborating later in their dialogue, in terms of when they establish most of their routines (median establishment time~$> 60\%$). Though the measures of task performance would only reflect that these teams performed badly with a final overall score of performance, our alignment measures reflect details of the performance. Interlocutors are gently reminded a few minutes before the end of the task the remaining time, but were not rushed to find a solution: which could have changed the way they aligned by forcing an establishment period. Thus, we observe through our alignment measures that badly performing teams were simply slower to collaborate and establish routines. 

Two teams have established routines later in their dialogue: Team 17 that found a correct solution, and Team 18 that could not (their median establishment times are around 70\%). Yet, 17 has a focused establishment period (with a smaller IQR $= 18\%$ vs.\ $30\%$ of the time, respectively, see Fig.~\ref{fig:h1_1_plot}). We interpret that Team 17 was able to turn it around and find a correct solution, while Team 18 did not; ending up as the worst performing team. 17 has positive learning gain (\measure{learn} = 25\%), while it is negative for Team 18 (\measure{learn} = -56\%, the highest decrease among the transcribed teams, see Fig.~\ref{fig:transcribed_scatter}). While bad performance could be reflected through a collaborative period starting later in their dialogue (such as Team 18; with later establishment, and not finding a solution in time), Team 17 shows that there are exceptions to this. Team 18 also possibly got confused, reflected in the high and negative \measure{learn}.

The collaborative and exploratory periods can also be observed by examining the error progression of teams' submitted solutions during the task, as shown in Fig.~\ref{fig:h1_1_plot}. During the exploratory period, Nine out of ten teams had their highest error. For teams that performed well, their collaborative period had their lowest error before finding an optimal solution (thus ending the task), and for other teams; their closest solution to the optimal solution. There are 8 such teams that exhibit this behaviour. The teams that did not achieve a correct solution, never regressed to their largest error from the exploratory period. Looking at the number of attempts, for the well-performing teams, their collaborative period was productively used, with their next solution reaching an optimal cost (Teams 17 and 28), or one more attempt before their optimal cost (Team 20). Several teams that did not perform well have a greater number of attempts submitted after their collaborative period (Teams 9, 7, 8, 10, 47). Their submission pattern of attempts indicate a ``trial-and-error" strategy on how to solve the task, for example, Teams 8 and 9 increasing their submissions after their collaborative period, or Teams 7, 10 and 47 submitting throughout.

\paragraph{For learning outcomes.}
The distribution of the median establishment times are not statistically significantly different for teams with positive learning outcomes (Teams 7, 9, 10, 11, 17) vs.\ others (Teams 8, 18, 20, 28, 47) by Kruskal-Wallis H test ($H = 0.88$, $p = .35$ for times in absolute values, and $H = 0.10$, $p = .75$ for normalised times).

\paragraph{Synopsis.}
Overall, the results support H1.1 for task performance, while they are inconclusive for learning outcomes. Surprisingly, we see that all teams, regardless of task success, are (lexically) aligned to some degree. Thus, inspecting the distributions of the establishment times together with their proposed solutions gave further insight into the collaboration processes, specifically revealing a ``collaborative period" that most of the teams came up with their best solutions. This captures some patterns of alignment that might have otherwise been overlooked.

\subsubsection*{H1.2: Hesitation phenomena are more likely to occur in the vicinity of priming and establishment of task-specific referents for more successful teams.} \label{subsec:results_h1_2}

We consider hesitation phenomena as cued by the presence of a filler, and thus investigate how are the fillers distributed as compared to the priming and establishment of the routines. The results for Mann-Whitney U test and effect size as estimated by Cliff's Delta ($\delta$) are given in Table~\ref{tab:filler_priming_establishment}. $\delta$ ranges from $-1$ to $1$, where $0$ would indicate that the group distributions overlap completely; whereas values of $-1$ and $1$ indicate a complete absence of overlap with the groups. For example, $-1$ indicates that all fillers occur before priming times, and $1$ indicates that all fillers occur after priming.


We observe that filler and \textbf{priming times} differ significantly for most of the teams (for eight out of ten teams by Mann-Whitney U test $p < .05$). We see positive $\delta$ values, except for one team. Most teams thus have fillers that occur after priming times. We see that the magnitude of $\delta$ for most teams is large except for Team~7 (excluding Teams 20 and 8 that are not statistically significant)\footnote{The magnitude of Cliff's Delta ($\delta$) can be interpreted by using the thresholds from~\citet{romano_appropriate_2006}, i.e.\ $|\delta|<0.147$ ``negligible", $|\delta|<0.33$ ``small", $|\delta|<0.474$ ``medium", and otherwise ``large".}. We interpret that most fillers do occur visibly after priming times (with little overlap from the large effect sizes). We observe that filler and \textbf{establishment times} differ significantly for most of the teams (for seven out of ten teams by Mann-Whitney U test $p < .05$). We see $\delta$ ranging from $-0.67$ for Team 7, to $0.33$ for Team 11 (though most are negative). However, we see that the magnitude of $\delta$ for most teams is small, with the exception of two teams. This means that the distributions of fillers differ with a small effect size compared to the distributions of establishment times, especially considering that the token number values do not overlap; i.e.\ we do not expect an effect size of $0$. We thus interpret most fillers do occur around (from positive and negative $\delta$ values) establishment times (with larger overlap from small effect sizes).

\begin{table}[tbp]
    \centering
    \caption{The results for the Mann-Whitney U test that compares the distribution of filler times with  establishment and priming times for H1.2. The effect size is estimated by Cliff's Delta ($\delta$). Teams are sorted by decreasing task performance i.e.\ increasing \measure{error}. The horizontal line separates well-performing teams (that found a correct solution) from badly-performing teams. $U$ is the U statistic, and $p$ is the `two-sided' p-value of a Mann-Whitney U test (without continuity correction as there can be no ties, via our unique token number assignment).}
    \label{tab:filler_priming_establishment}
    \footnotesize
    \begin{tabular}{r|rr|rrr|rrr|rrr}
        {} & \multicolumn{2}{c}{count} & \multicolumn{3}{c}{median (\%)} & \multicolumn{3}{c}{priming} & \multicolumn{3}{c}{establishment} \\
        Team & filler & routine &     filler & priming & establishment &       $U$ &        $p$ &      $\delta$ &             $U$ &        $p$ &      $\delta$ \\
        \midrule
        28   &     38 &            58 &       11.6 &     3.5 &          15.2 &  1600.5 &  $< .05$ &   0.45 &         828.5 &  $< .05$ &  -0.25 \\
        17   &     27 &            41 &       14.0 &     6.2 &          17.1 &   823.0 &  $< .05$ &   0.49 &         431.0 &    $.12$ &  -0.22 \\
        20   &     59 &            51 &       20.7 &    18.1 &          22.8 &  1746.5 &    $.15$ &   0.16 &        1139.5 &  $< .05$ &  -0.24 \\ \hline
        11   &     35 &            70 &       34.5 &     3.5 &          24.4 &  2229.0 &  $< .05$ &   0.82 &        1624.0 &  $< .05$ &   0.33 \\
        9    &     81 &           131 &       46.3 &    11.4 &          37.4 &  8805.5 &  $< .05$ &   0.66 &        6561.5 &  $< .05$ &   0.24 \\
        47   &     56 &            74 &       19.5 &     6.7 &          21.9 &  3189.0 &  $< .05$ &   0.54 &        1627.0 &  $< .05$ &  -0.21 \\
        10   &     20 &            65 &       20.1 &     8.7 &          20.4 &   982.0 &  $< .05$ &   0.51 &         660.0 &    $.92$ &   0.02 \\
        8    &     26 &            62 &       19.8 &    15.7 &          36.0 &   883.0 &    $.48$ &   0.10 &         461.0 &  $< .05$ &  -0.43 \\
        7    &     27 &            59 &       24.9 &    25.9 &          37.8 &   562.0 &  $< .05$ &  -0.29 &         259.0 &  $< .05$ &  -0.67 \\
        18   &     52 &            57 &       10.8 &     4.3 &          11.8 &  2136.0 &  $< .05$ &   0.44 &        1326.0 &    $.34$ &  -0.11 \\
                
    \end{tabular}
\end{table}

These results indicate that in the process of routine formation, in between the priming and the establishment of the expression, there seems to be a period in which the interlocutors exhibit hesitation phenomena. This placement of fillers is of interest due to the potentially unfamiliar vocabulary of the task-specific referents that the interlocutors had to utilise in the situated environment. The results demonstrate a lack of hesitation phenomena at the start of the formation of a routine; i.e.\ they occur visibly after the priming of expressions that contain task-specific referents. The large effect size shows that this is predominantly the case for most teams. In addition to this, fillers were found to occur around establishment times. We suggest that a part of establishment is often a clarification request, as shown by the following example. Red indicates the routine expression, while blue indicates the filler.

\begin{idea}
\noindent\textbf{\textit{A}:} \textcolor{red}{\textit{Mount Zurich to Mount Bern}}.
\newline \textbf{\textit{\dots \dots}} 
\newline \textbf{\textit{B}:} \textcolor{blue}{uh} isn't already \textcolor{red}{\textit{Mount Zurich to Mount Bern}} isn't it connected?
\newline \textbf{\textit{\dots \dots}} 
\newline \textbf{\textit{A}:} So if we erase Mount \textcolor{red}{\textit{Zurich}} or Mount Ber- to Mount Bern or Mount \textcolor{red}{\textit{Zurich}} to Mount Gallen?
\newline \textbf{\textit{B}:} Wait \textcolor{blue}{uh} \textcolor{red}{\textit{Zurich}} to Mount \dots ?
\label{quote:clar_req}
\end{idea}

Speakers are able to prime these expressions without exhibiting this hesitation phenomena, but this does not guarantee that the primed expression was fully understood by the listener, as shown by the results of the Mann-Whitney U test. Following the idea of IF and IG pairs in the dialogue, the IG (speaker) tends to be in the abstract view, and can see the minimally represented names of gold mines. They need only concentrate on the gold mines that have the lowest cost to connect. Perhaps the reason why the IG does not exhibit (by our measures) this uncertainty is because they can see the task-specific referents available to them written down on the map. Expressions that contain task-specific referents could successfully become part of the IG's expression lexicon when given these new referents. The IG may also feel at ease to read out these expressions. The IF (listener) must follow the instructions with actions, and since they can not see the cost of adding and removing edges, they must search for the specific gold mine names given by the IG. This could create an uncertainty in the IG, and bring about a need to clarify.

\paragraph{For task performance.}
The distribution of the Cliff's Delta between filler times and both priming or establishment times has a very weak correlation coefficient with \measure{error} (Spearman's $\rho =-0.18$, $p = .62$ for priming, $\rho =0.06$, $p = .88$ for establishment). Therefore, we can not conclude that there is a significant relationship between how early are the priming or establishment times, and how well a team performs.

\paragraph{For learning outcomes.}
The distribution of the Cliff's Delta that quantifies how different are filler times from priming or establishment times are not statistically significantly different for teams with positive learning outcomes (Teams 7, 9, 10, 11, 17) vs.\ others (Teams 8, 18, 20, 28, 47) by Kruskal-Wallis H tests ($H = 1.32$, $p = .25$ for both). Therefore, we can not conclude that a significant difference exists, between how early fillers occur compared to priming (or establishments) between these two learning groups.

\paragraph{Synopsis.}
Regarding H1.2, we can not conclude that the usage of fillers occur in the vicinity of 
priming or establishments times for more successful teams (for neither better-performing teams, nor higher-learning teams). Overall, we see that for most of the teams, the fillers tend to occur visibly after priming times, and around establishment times. We still believe that this gives us a fascinating insight into the way the interlocutors use task-specific expressions in a situated environment.

% By inspecting how are the fillers distributed in comparison to establishment times, we see that  \dots.
% Further investigation of comparing the filler distribution with priming times indicate \dots
% when task-specific referents become routine, they are more likely to be surrounded by hesitation phenomena, particularly around establishment times and not around priming times.

\subsection{RQ2: How do the interlocutors follow up the use of task-specific referents with actions? Does this link to task success?}\label{subsec:results_rq2}

\subsubsection*{H2.1: Instructions are more likely to be followed by a corresponding action early in the dialogue for more successful teams.}

To investigate H2.1, we automatically infer (mis)matches\footnote{As described in Algorithm~\ref{algo:match_instructions_actions}. We process this combined dialogue and actions corpus via a script (\notebook{tools/6\_recognise\_instructions\_detect\_follow-up\_actions.ipynb} in the tools) to generate an annotated corpus (\folder{processed\_data/annotated\_corpus}, available with the tools). The annotated corpus contains the inferred instructions, their pending lists used for matching, matches, mismatches, and nonmatches if there were no instructions to be (mis)matched.}, where a verbal instructions' follow-up action is labelled as a (mis)match following the methodology described in Sec.~\ref{subsec:studying_RQ1}. Then, we inspect the distribution of the (mis)matches of the teams, and see how this is related to task success.

\paragraph{For task performance.}
The median match times has a moderate positive correlation coefficient with the task performance measure \measure{error} (Spearman's $\rho = 0.59$, $p = .08$), that is, better-performing teams have matches earlier. This follows the results in H1.1, regarding establishment times. For the matches in the common duration (i.e.\ first $\approx 11$ mins), there is a moderate correlation coefficient ($\rho = 0.45$, $p = .23$, ignoring Team 18 that has no matches in this common period). Fig.~\ref{fig:h2_1_time_absolute_plot} shows the the distribution of the (mis)match times for each team. When the times are normalised by the duration for each team separately, we observe a positive, moderate Spearman's correlation coefficient ($\rho = 0.54$, $p = .11$), that indicates a general trend that matches happen earlier for the better-performing teams.

Fig.~\ref{fig:h2_1_plot} shows for each team, the distribution of the match and mismatch times, normalised by the duration of each team itself. While it is natural to think that instructions will be followed by a match for more successful teams in a structured and organised manner, we observe that teams that performed badly and teams that did not learn also have a certain period of matches. Therefore, all teams, independent of their task success, have their IG's instructions matched to the IF's actions to some extent. Match times have mean of the medians~$= 62.6\%$ (combined $SD = 21.9\%$), and mismatches have mean of medians~$= 67.6\%$ (combined $SD = 26.0\%$).

By inspecting the outputs of the automatically inferred instructions in Table~\ref{tab:algo_results}, occasionally, we see that the traditional roles of IF and IG are not maintained, even for the brief fixed time of views (i.e.\ within a turn). The IF, having just been switched from IG, may have their own ideas about the next best edit action, as seen in Utt.\ no.\ $199$ (prior to  Utt.\ no.\ $198$, the views were swapped, with B being in the abstract view, meaning B was just previously the IG). Thus the interlocutors can also conduct a negotiation where they collaboratively decide which action to take. It is therefore not always the case that the IG is in the abstract view deciding and instructing what the IF in the visual view should do; and this is supported by the frequent swapping of views.

\begin{table}[tbp]
    \centering
    \scriptsize
    \caption{An example from the output of recognising instructions and detecting follow-up actions (by Algorithms~\ref{algo:recognise_instructions} and~\ref{algo:match_instructions_actions}), from Team 10. \textit{View} denotes which view the interlocutor is in (refer to Sec.~\ref{subsec:activity}). \textit{Annotations} denotes the automatically inferred instructions and follow-up actions in the activity.
    For example, \textit{Instruct\textsubscript{A}} indicates that interlocutor A has given an instruction to add two nodes (inferred from referents), which can be partially recognised \textit{(Gallen,?)}. As shown, the algorithm builds up (or ``caches") instructions until an edit action is performed (`\naannotation' in Utt.\ no.). Note, since B is in the visual view his/her inferred instruction is deliberately not matched.}
    \label{tab:algo_results}
    \begin{tabular}{c|c|c|c|l|l}
    % \begin{tabular}{c|c|c|c|p{0.25\textwidth}|p{0.35\textwidth}}
          & Utt. no. & View & Verb & Utterance & Annotations\\
        \cline{1-6}
        \multirow{2}*{A} & \multirow{2}*{198} & \multirow{2}*{Abstract} & \multirow{2}*{says} & Maybe we start from, & Instruct\textsubscript{A}(Add(Zermatt,?)) \\
        &&&& Mount Zermatt ? &  \\ 
        \cline{5-6}
        \multirow{2}*{B} & \multirow{2}*{199} & \multirow{2}*{Visual} & \multirow{2}*{says} & No lets do Mount Davos to, & {Instruct\textsubscript{A}(Add(Zermatt,?), Instruct\textsubscript{B}(Add(Davos,?))
        % \textit{As prev.}
        } \\
        &&&& where do you wanna go? &  \\ 
        \cline{5-6}
        \multirow{2}*{A} & \multirow{2}*{200} & \multirow{2}*{Abstract} & \multirow{2}*{says} & \multirow{2}*{\dots to Mount, St Gallen.} & {Instruct\textsubscript{A}(Add(Zermatt,?), Instruct\textsubscript{B}(Add(Davos,?)}, \\
        % {\textit{As prev.} $+$}, \\
        &&&&& \textcolor{blue}{Instruct\textsubscript{A}(Add(Gallen,?))} \\ 
        \cline{5-6}
        \multirow{1}*{B} & \multirow{1}*{201} & \multirow{1}*{Visual} & \multirow{1}*{says} & \multirow{1}*{Okay.} & {\textit{As previous}} \\

        \cline{5-6}
        \multirow{1}*{B} & \multirow{1}*{\naannotation} & \multirow{1}*{Visual} & \multirow{1}*{adds} & \multirow{1}*{Gallen-Davos} 
        % &  \textcolor{red}{Match\textsubscript{B}}(\textcolor{blue}{Instruct\textsubscript{A}(Add(Gallen, ?))\textcolor{red}{)}} \\
        &  Instruct\textsubscript{A}(Add(Zermatt,?), \textcolor{magenta}{Match\textsubscript{B}}\textcolor{blue}{(Instruct\textsubscript{A}(Add(Gallen,?)))}\\
        \cline{1-6}
    \end{tabular}
\end{table}


\begin{figure}[tbp]
    \centering %  Box and whiskers plots of the
    \includegraphics[width=\linewidth]{figs/h2_1_time_absolute_plot.pdf}
    \caption{The team's match and mismatch times in blue (`$+$') and red (`$\times$') respectively, to study H2.1. The teams are sorted by decreasing learning outcomes (i.e.\ decreasing \measure{learn}). See Fig.~\ref{fig:h1_1_time_absolute_plot} for a description of the green, red and blue lines.} \label{fig:h2_1_time_absolute_plot}
\end{figure}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/h2_1_time_plot.pdf}
    \caption{The teams’ match and mismatch times in green and red respectively, as normalised by the duration for each team separately. Sorting is as in Fig.~\ref{fig:h2_1_time_absolute_plot}.} \label{fig:h2_1_plot}
\end{figure}


\paragraph{For learning outcomes.}
By inspecting the median of the match times with \measure{learn}, we observe that they are not statistically significantly different for teams with positive learning outcomes (Teams 7, 9, 10, 11, 17) vs.\ others (Teams 8, 18, 20, 28, 47) by Kruskal-Wallis H tests ($H = 0.54$, $p = .47$ for times in absolute values, and $H = 0.10$, $p = .75$ for normalised times).

Though not statistically significant by these measures, from the Algorithm~\ref{algo:match_instructions_actions}'s results, we see that all teams have more inferred matches than mismatches (see Table~\ref{tab:oh_match_mismatch} for reference). Teams 18 and 20 that learnt the least, have the highest match-to-mismatch ratio ($3.6$ and $4.0$ matches of instructions-to-actions for every $1$ mismatch respectively.), as well as Team 7 ($3.3$). Teams 8 and 47, which are also amongst the teams that had a negative learning gain (but close to zero, substantially higher than 18 and 20), have lower match-to-mismatch ratio of $2.7$ and $1.3$ respectively. 
% Inspecting Fig.~\ref{fig:transcribed_scatter}, we observe that they are farther away from teams 18 and 20 in terms of \measure{learn}. 
We observe that Teams 10, 11 and 17, who had the highest learning gain, comparatively have a lower ratio of matches-to-mismatches of $2.4$, $1.8$ and $2.3$ respectively. We interpret that it is important for learning that interlocutors have a good ratio of matches-to-mismatches, and not just be in total (blind) agreement with the other. This is consistent with previous research, as stated in Sec.~\ref{subsec:structure}. By just inspecting performance, superficially, Team 20 performed well. However, they did not learn (in fact, ``unlearnt", as shown with a negative learning outcome). Observing their progression of costs for submitted solutions (from $191 \%$, to $109 \%$, to finding an optimal solution) informs us that they ``got lucky" in finding a solution, however did not learn, as is further evidenced by only a few, and sparse mismatched instructions-to-actions. Indeed, before finding an optimal solution, their previous error ($109 \%$) was substantially higher than any other team that performed badly.

From the results, we interpret that positive learning teams seem to have conflict(s) that they resolved collaboratively while building and submitting solutions (and receiving feedback from the robot), whereas the others either had less or unresolved conflicts. By inspecting how the (mis)matches are distributed, and how they are they positioned in relation to the costs of the submitted solutions, we observe nuances of conflicts and their resolutions. For instance, consider a high-learning Team 11. The team began with a high cost ($191\%$, i.e.\ they basically connected everything to each other, with many redundant connections). One interpretation is that they initially misunderstood the goal of the task of connecting the graph minimally\footnote{And are not only exploring the graph to see the costs and available connections, as is evidenced by their following submissions that had again a very high cost ($127\%$), only later decreasing further through several submissions.}. Then, they had many mismatches (``a mismatch period"), which is followed by many matches ending with (at Q3 of matches) their best solution, getting very close ($5\%$, i.e.\ they did not notice that they could replace a particular connection with a better/lower-cost one). Although the team could not find a correct solution, they learnt a lot from this interaction flow. In comparison, Team 20 also started with that high cost of $191\%$. Yet, they could not resolve the conflict, as their (mis)matches did not result in them getting closer to an optimal solution, but rather still keeping to high cost solutions, and repeating these high cost submissions (109\%, i.e. more than double the cost they could make with many redundant connections). Although they found a correct solution next, since they did not have the conflict resolution period that could be cued by (mis)matches, they did not end up learning.

\paragraph{Synopsis.}
We see that all teams have (mis)matches, irrespective of their task success; therefore, it is not necessary to follow-up with an action in order to succeed. In terms of task performance, we observe a general trend that supports the H2.1, i.e.\ better performing teams tend to follow up the instructions with actions (as matches) early overall (the absolute times), as well as in their dialogues (normalised times). For learning, although the general trend is not statistically confirmed, we gained insight into the nuances of the dynamics of interaction: by inspecting the normalised (mis)match time plots alongside with the submission costs. There seems to be conflicts that may be collaboratively resolved and resulted in learning, or may not be resolved and have adverse effects on the learning outcomes.

\subsubsection*{H2.2: When instructions are followed by a corresponding or a different action, the action is more likely to be in the vicinity of information management phenomena for more successful teams.}
% \subsubsection*{H2.2: When instructions are followed by a corresponding or a different action, the action is more likely to be in the vicinity of information management phenomena for more successful teams.}

To investigate H2.2, we consider the distribution of the information management marker `oh' through time\footnote{We note that the `oh' marker occurs 333 times in the transcripts (average per transcript $= 33.3$, $SD = 20.3$). See Table~\ref{tab:oh_match_mismatch} for the number of utterances that contain one or more `oh's for each team.}, in relation to the distribution of matches and mismatches. In particular, we check if the distributions of `oh' times and (mis)matches are significantly different by Mann-Whitney U test, and estimate the effect size by computing Cliff's Delta ($\delta$). The results of the tests for each team are given in Table~\ref{tab:oh_match_mismatch}. Here, $\delta = -1$ would mean that all `oh's occur earlier than (mis)match times, and $1$; that all `oh's occur later\footnote{As H1.2, $\delta$ ranges from  $-1$ to $1$, where $0$ would mean that the group distributions overlap completely; whereas values of $-1$ and $1$ indicate a absence of overlap between the groups. 
% However, due to the difference in calculation of H1.2 and H2.2 (please see Section~\ref{sec:methodology}), the small effect size in H2.1 is less negligible than in H1.1
}. For all teams except one, the value of $\delta$ is negative, indicating that the distribution of `oh' tends to occur earlier than (mis)match times. We observe that `oh' and (mis)match times do not significantly differ for half of the teams (Mann-Whitney U test $p < .05$). We see $\delta$ ranging from $-0.54$ for Team 8, to $0.09$ for Team 11: this indicates that `oh' occurs differently compared to the (mis)match times within the teams. We see that for the teams that had significantly different distributions, the effect size ranges from negligible ($|\delta|<0.147$) to medium ($|\delta|<0.474$), with the exception of Team 8, that has large effect size ($\delta = -0.54$).      

\begin{table}[tbp]
    \centering
    \caption{The results for Mann-Whitney U tests that compare the distribution of information marker (i.e.\ `oh') times, with (mis)match times for H2.2. The effect size estimated by Cliff's Delta ($\delta$). Teams are sorted by decreasing task performance, i.e.\ increasing \measure{error}. $U$ is the U statistic, and $p$ is the `two-sided' p-value of a Mann-Whitney U test (without continuity correction).}
    \label{tab:oh_match_mismatch}
    % \footnotesize
    \small
    \begin{tabular}{r|rrrr|rrr|rrr}
        {} & \multicolumn{4}{c|}{count (number of utterances)} & \multicolumn{3}{c|}{median (\%)} & \multicolumn{3}{c}{(mis)match} \\
        Team &  oh & match & mismatch & match/mism. &         oh & match & mismatch &      $U$ &        $p$ &      $\delta$ \\
        \midrule
        % 10   &  18 &    36 &       15 &       2.4 &       47.6 &  67.3 &     65.3 &          264.0 &  $< .05$ &  -0.42 \\
        % 11   &  15 &    34 &       18 &       1.8 &       57.3 &  59.5 &     38.5 &          427.0 &    $.58$ &   0.09 \\
        % 17   &  20 &    23 &       10 &       2.3 &       61.1 &  61.1 &     69.4 &          318.0 &    $.83$ &  -0.04\\
        % 9    &  29 &    28 &        9 &       3.1 &       42.9 &  59.9 &     70.2 &          429.0 &    $.16$ &  -0.20 \\
        % 7    &  51 &    43 &       13 &       3.3 &       49.7 &  65.5 &     79.7 &          841.0 &  $< .05$ &  -0.41 \\
        % \hline
        % 28   &  24 &    19 &       13 &       1.5 &       61.7 &  62.7 &     73.6 &          344.0 &    $.51$ &  -0.10 \\
        % 8    &  55 &    30 &       11 &       2.7 &       36.3 &  65.3 &     86.3 &          522.0 &  $< .05$ &  -0.54 \\
        % 47   &  29 &    28 &       21 &       1.3 &       53.4 &  56.8 &     75.7 &          488.0 &  $< .05$ &  -0.31 \\
        % 20   &  65 &    24 &        6 &       4.0 &       35.0 &  58.0 &     42.3 &          715.0 &  $< .05$ &  -0.27 \\
        % 18   &  12 &    25 &        7 &       3.6 &       69.6 &  69.5 &     75.0 &          157.0 &    $.36$ &  -0.18\\
        % \hline
        28   &  24 &    19 &       13 &       1.5 &       61.7 &  62.7 &     73.6 &          344.0 &    $.51$ &  -0.10 \\
        17   &  20 &    23 &       10 &       2.3 &       61.1 &  61.1 &     69.4 &          318.0 &    $.83$ &  -0.04\\
        20   &  65 &    24 &        6 &       4.0 &       35.0 &  58.0 &     42.3 &          715.0 &  $< .05$ &  -0.27 \\
        \hline
        11   &  15 &    34 &       18 &       1.8 &       57.3 &  59.5 &     38.5 &          427.0 &    $.58$ &   0.09 \\
        9    &  29 &    28 &        9 &       3.1 &       42.9 &  59.9 &     70.2 &          429.0 &    $.16$ &  -0.20 \\
        47   &  29 &    28 &       21 &       1.3 &       53.4 &  56.8 &     75.7 &          488.0 &  $< .05$ &  -0.31 \\
        10   &  18 &    36 &       15 &       2.4 &       47.6 &  67.3 &     65.3 &          264.0 &  $< .05$ &  -0.42 \\
        8    &  55 &    30 &       11 &       2.7 &       36.3 &  65.3 &     86.3 &          522.0 &  $< .05$ &  -0.54 \\
        7    &  51 &    43 &       13 &       3.3 &       49.7 &  65.5 &     79.7 &          841.0 &  $< .05$ &  -0.41 \\
        18   &  12 &    25 &        7 &       3.6 &       69.6 &  69.5 &     75.0 &          157.0 &    $.36$ &  -0.18
        % \\ \\ \\
        % 10   &  18 &    36 &       12 &       3\phantom{.000} &       47.6 &  67.3 &     67.0 &          242.0 &  $< .05$ &  -0.44 \\
        % 11   &  15 &    32 &       19 &       1.684 &       57.3 &  60.3 &     39.6 &          394.0 &    $.86$ &   0.03 \\
        % 17   &  20 &    21 &       10 &       2.1\phantom{00} &       61.1 &  54.3 &     74.7 &          291.0 &    $.71$ &  -0.06 \\
        % 9    &  29 &    27 &       10 &       2.7\phantom{00} &       42.9 &  60.1 &     69.0 &          429.0 &    $.16$ &  -0.20 \\
        % 7    &  51 &    43 &        8 &       5.375 &       49.7 &  65.5 &     85.0 &          759.0 &  $< .05$ &  -0.42 \\
        % 28   &  24 &    15 &       14 &       1.071 &       61.7 &  62.7 &     74.4 &          296.0 &    $.35$ &  -0.15 \\
        % 8    &  55 &    27 &       11 &       2.454 &       36.3 &  64.3 &     82.7 &          495.0 &  $< .05$ &  -0.53 \\
        % 47   &  29 &    27 &       20 &       1.35\phantom{0} &       53.4 &  59.1 &     66.6 &          479.0 &  $< .05$ &  -0.30 \\
        % 20   &  65 &    23 &        4 &       5.75\phantom{0} &       35.0 &  57.3 &     42.2 &          641.0 &  $< .05$ &  -0.27 \\
        % 18   &  12 &    24 &        6 &       4\phantom{.000} &       69.6 &  70.0 &     73.1 &          149.0 &    $.39$ &  -0.17 \\ 
        % \\ \\
        % \multicolumn{11}{l}{in increasing error order} \\
        % \\
        % 28   &  24 &    15 &       14 &       1.071429 &       61.7 &  62.7 &     74.4 &          296.0 &    $.35$ &  -0.15 \\
        % 17   &  20 &    21 &       10 &       2.1 &       61.1 &  54.3 &     74.7 &          291.0 &    $.71$ &  -0.06 \\
        % 20   &  65 &    23 &        4 &       5.75 &       35.0 &  57.3 &     42.2 &          641.0 &  $< .05$ &  -0.27 \\
        % 11   &  15 &    32 &       19 &       1.68 &       57.3 &  60.3 &     39.6 &          394.0 &    $.86$ &   0.03 \\
        % 9    &  29 &    27 &       10 &       2.7 &       42.9 &  60.1 &     69.0 &          429.0 &    $.16$ &  -0.20 \\
        % 47   &  29 &    27 &       20 &       1.35 &       53.4 &  59.1 &     66.6 &          479.0 &  $< .05$ &  -0.30 \\
        % 10   &  18 &    36 &       12 &       3. &       47.6 &  67.3 &     67.0 &          242.0 &  $< .05$ &  -0.44 \\
        % 8    &  55 &    27 &       11 &       2.45 &       36.3 &  64.3 &     82.7 &          495.0 &  $< .05$ &  -0.53 \\
        % 7    &  51 &    43 &        8 &       5.375 &       49.7 &  65.5 &     85.0 &          759.0 &  $< .05$ &  -0.42 \\
        % 18   &  12 &    24 &        6 &       4. &       69.6 &  70.0 &     73.1 &          149.0 &    $.39$ &  -0.17 \\
    \end{tabular}
\end{table}

\paragraph{For task performance.}
Since the $\delta$ values are varying from being around 0 to negative values (see Table~\ref{tab:oh_match_mismatch}), for all teams except one, oh's occur earlier than (mis)match times. Following this, the $\delta$ values between `oh' times and (mis)match times has a medium negative correlation coefficient with \measure{error} (Spearman's $\rho =-0.53$, $p = .12$). This means that the better the performance, the more the overlap between (mis)match times and `oh's. There is a general trend that for well-performing teams the `oh's occur more in the vicinity of (mis)match times with larger overlap between the two groups, and the badly-performing teams have comparably less overlap. Thus the results support H2.2. 
% , then for badly-performing teams they tend to occur earlier than the (mis)matches (with less and less overlap). 
% However, keeping in mind the negligible to medium $\delta$ values, 
% For most teams, `oh' does occur consistently before the (mis)matched instructions-to-actions (indicated by the negative $\delta$ values, except for one team), 
% just generally with more overlap for better-performing teams, and generally less overlap for worse-performing teams.
% just generally closer for better-performing teams, and generally farther away for worse-performing teams.


\begin{table}[tbp]
    \centering
    \footnotesize
    \caption{% Example utterances 
    Excerpts that contain information management marker `oh' from Team 20, who performed well but did not learn. 
    % We sample utterances from 2 teams at the start and end of the dialogue. 
    % We choose team 17, who had high task success (i.e.\ performed and learnt well), versus team 20, who performed well but did not learn. 
    Annotations could have the pending instructions, and (mis)matched or nonmatched actions.
     Note, \textcolor{blue}{Nonmatch\textsubscript{Interlocutor}} frequently occurs when the interlocutor follows their own intentions, as seen after Utterance 10, \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)), where A connects two nodes (for brevity, nodes given in Utterance column, unless partial (mis)match).
    }
    \label{tab:algo_results_oh_20}
    % \begin{tabular}{c|c|c|l|l}
    \begin{tabular}{P{.02\textwidth}|R{.04\textwidth}|P{0.06\textwidth}|p{.35\textwidth}|p{.4\textwidth}}
        Int. & Utt. & Verb & Utterance & Annotations \\ \hline
        \dots  & \dots  & \dots & \dots & \dots \\
        B & 10 & says & I'm just gonna \dots & \nautterance \\
        A & \nautterance & adds & Luzern-Zermatt & \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)) \\
        A & 11 & says & Uh \dots & \nautterance \\
        A & 12 & says & Uh \dots & \nautterance \\
        B & 13 & says & \textcolor{red}{Oh} there. & \nautterance \\
        A & 14 & says & \textcolor{red}{Oh} two three. & \nautterance \\
        B & 15 & says & \textcolor{red}{Oh} that's what you've been doing this all time. & \nautterance \\
        \dots  & \dots  & \dots & \dots & \dots \\
        % A & \nautterance & adds & Interlaken-Neuchatel &
        % \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)) \\
        % A & 39 & says & \textcolor{red}{Oh} we, \textcolor{red}{oh} wait \textcolor{red}{oh} wait. & \naannotation \\
        % B & 40 & says & Let me see this. & \naannotation \\ 
        % A & \nautterance & adds & Basel-Neuchatel & \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)) \\
        % B & 41 & says & We've got \dots & \naannotation \\ 
        % A & 42 & says & \textcolor{red}{Oh} it's your turn. & \naannotation \\
        % B & 43 & says & \dots um that was quick. & \naannotation  \\      
        % \dots  & \dots  & \dots & \dots & \dots \\
        B & 56 & says & \textcolor{red}{Oh} I think we have to connect all of them. & Instruct\textsubscript{A}(Add(Gallen,?)) \\  
        B & \nautterance & adds & Luzern-Interlaken & % Do\textsubscript{B}(Add),  
        \textcolor{magenta}{Mismatch\textsubscript{B}}(Instruct\textsubscript{A}(Add(Gallen,?))) \\
        % &&&& \textcolor{magenta}{Mismatch\textsubscript{B}}(Instruct\textsubscript{A}(Add(Gallen,?))\textcolor{magenta}{)}\\
        B & \nautterance & adds & Luzern-Zurich & \textcolor{blue}{Nonmatch\textsubscript{B}}(Do\textsubscript{B}(Add)) \\
        A & 57 & says & \textcolor{red}{Oh}. & \naannotation \\
        B & 58 & says & Okay I did some & \multirow[t]{2}{*}{\naannotation}  \\ 
        A & 59 && okay for me.  & \\
        A & \nautterance & adds & Luzern-Davos & \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)) \\
        A & 60 & says & \textcolor{red}{Oh} no. & \naannotation \\
        B & 61 & says & I think we are doing terrible. & \naannotation \\
        \dots & \dots & \dots & \dots & \dots \\
        A & 450 & says & \textcolor{red}{Oh}. & \naannotation  \\ 
        B & 451 & \multirow[t]{2}{*}{says} & 3. & \multirow[t]{2}{*}{\naannotation}  \\ 
        B & 452 && What?  &\\ 
        A & 453 & says & Let me \dots & \naannotation  \\ 
        A & \nautterance & removes & Luzern-Zermatt & \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Remove)) \\
        A & 454 & \multirow[t]{2}{*}{says} & There you go. & \multirow[t]{2}{*}{\naannotation} \\
        A & 455 && What no. & \\
        B & 456 & \multirow[t]{2}{*}{says} & You are erasing my mistake. & \multirow[t]{2}{*}{\naannotation} \\ 
        B & 457 && How dare you. & \\
        \multirow[t]{6}{*}{A} & 458 & \multirow[t]{6}{*}{says} & I know. & \multirow[t]{6}{*}{\naannotation} \\
        & 459 && Wait, what? &\\
        & 460 && Can I get pencil again? &\\
        & 461 && \textcolor{red}{Oh oh}. &\\
        & 462 && \textcolor{red}{Oh}. &\\
        & 463 && Okay. &\\
        B & 464 & says & We messed up again didn't we? & \naannotation \\
        \dots  & \dots  & \dots & \dots & \dots \\ 
        % \bottomrule
        \hline
    \end{tabular}
\end{table}


\begin{table}[tbp]
    \centering
    \footnotesize
    \caption{
    Excerpts that contain information management marker `oh' from Team 17, who had high task success (i.e.\ performed and learnt well). Utt.\ stands for the utterance number, which is not applicable for the edit actions. See the caption of Table~\ref{tab:algo_results_oh_20} for further details.
    % Example utterances that contain information management marker ``oh'' . We sample utterances from 2 teams at the start and end of the dialogue. We choose team 17, who had high task success, versus team 20, who performed well but did not learn. Note, Nonmatch\textsubscript{Int.} frequently occurs when the interlocutor follows their own intentions, as seen in the first utterance given for Team 20, \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}), where A connects two nodes (for brevity, nodes given in Utterance column, unless partial match/mismatch).
    }
    \label{tab:algo_results_oh_17}
    % \begin{tabular}{c|c|c|c|l|l}
    \begin{tabular}{P{.02\textwidth}|R{.04\textwidth}|P{0.06\textwidth}|p{.35\textwidth}|p{.4\textwidth}}
        Int. & Utt. & Verb & Utterance  & Annotations \\ \hline
        \dots & \dots & \dots & \dots & \dots \\
        I & 4 & says & So you only build from something & \naannotation \\
        &&& that is already connected. &\\
        B & 5 & says & \textcolor{red}{Oh}. & \naannotation \\
        A & 6 & says & \textcolor{red}{Oh} okay. & \naannotation \\ 
        B & \nautterance & adds & Zermatt-Davos & \textcolor{blue}{Nonmatch\textsubscript{B}}(Do\textsubscript{B}(Add)) \\
        B & \nautterance & adds & Gallen-Davos & \textcolor{blue}{Nonmatch\textsubscript{B}}(Do\textsubscript{B}(Add)) \\
        A & \nautterance & adds & Zurich-Davos & \textcolor{blue}{Nonmatch\textsubscript{A}}(Do\textsubscript{A}(Add)) \\
        \dots & \dots & \dots & \dots & \dots \\
        B & \nautterance & adds & Basel-Bern & \textcolor{magenta}{Match\textsubscript{B}(}Instruct\textsubscript{A}(Add(Basel,?))) \\
        A & 61 & says & Yeah, and then go to Mount Zurich. & Instruct\textsubscript{A}(Add(Zurich,?)) \\ 
        % \dots & \dots & \dots & \dots & \dots \\
        B & \nautterance & adds & Basel-Zurich & \textcolor{magenta}{Match\textsubscript{B}}(Instruct\textsubscript{A}(Add(Zurich,?))) \\
        \multirow[t]{3}{*}{A} & 62 & \multirow[t]{3}{*}{says} & Yeah. & \naannotation \\ 
         & 63 && \textcolor{red}{Oh} no that costs more. & \\   
         & 64 && uh \dots & \\ 
        B & 65 & says & We should erase it. & \naannotation \\
        \dots & \dots & \dots & \dots & \dots \\ 
        A & 266 & says & Then do Mount Bern to Mount Zermatt. & Instruct\textsubscript{A}(Add(Bern,Zermatt)) \\
        A & 267 & says & Maybe that's better. & \naannotation \\
        B & 268 & says & You can't do that. & \naannotation \\
        A & 269 & says & \textcolor{red}{Oh}. & \naannotation \\
        A & 270 & says & Then do \dots & \naannotation \\
        B & 271 & says & Mount Bern to Mount Interlaken? & Instruct\textsubscript{B}(Add(Bern,Interlaken)) \\
        A & 272 & says & Yeah. & \naannotation \\
        A & 273 & says & I think that's 4 though. & \naannotation \\
        B & \nautterance & adds & Interlaken-Bern & \textcolor{magenta}{Mismatch\textsubscript{B}}(Instruct\textsubscript{A}(Add(Bern,Zermatt))) \\
        A & 274 & says & So don't do that. & \naannotation \\
        B & 275 & says & Is that 4? & \naannotation \\
        A & 276 & says & \textcolor{red}{Oh} yeah it's, it is 4. & \naannotation \\
        \dots & \dots & \dots & \dots & \dots \\
        % \bottomrule
        \hline
    \end{tabular}
\end{table}


\paragraph{For learning outcomes.}
The distribution of the Cliff's Delta, that quantifies how different `oh' times are from (mis)match times, is not statistically significantly different for teams with positive learning outcomes (Teams 7, 9, 10, 11, 17) vs.\ others (Teams 8, 18, 20, 28, 47) by Kruskal-Wallis H test ($H = 0.27$, $p = .60$). 

We see from Table~\ref{tab:oh_match_mismatch} there is a delicate balance between performance and learning. Team 20 for example, performed well but learnt nothing, and differ with statistical significance in their distribution of `oh' versus (mis)match times compared to other better performing teams. For comparison, we thus choose Team 17, who had high task success (i.e.\ performed and learnt well), vs.\ Team 20, who performed well but did not learn, and then we sample utterances from these two teams at the start and end of their dialogue. See Table~\ref{tab:algo_results_oh_20} and Table~\ref{tab:algo_results_oh_17} for excerpts from Teams 20 and 17, respectively. For both teams, we see the first occurrences of `oh' in the tables (corresponding to the exploratory period, from H1.1) and a period of nonmatched instructions for both teams, as they individually figure out the constraints of the task and navigate the situated environment. Keeping in mind the stylistic differences amongst interlocutors (for example, in Team 20 we clearly see that interlocutor A tends to use `oh' frequently), we still see interesting differences between the teams in terms of their usage of `oh's and their instructions-to-actions.

In Team 20 (Utt.\ no.\ $56-61$), we see both interlocutors using `oh' traditionally as an information management marker (e.g.\ ``Oh I think we have to connect all of them"); but from the mismatch/nonmatch of instructions-to-actions, we see that this information state of the interlocutor is not transferred to the collective information state of both interlocutors. Essentially, the interlocutors are working in isolation, individually gaining (perceived) information about the situated environment (measured by use of `oh'), and then following up with their own intentions in isolation (e.g.\ mismatch and nonmatch between utt.\ no.\ 56 and 57). To contrast, we clearly see that Team 17 (Utt.\ no.\ $61-65$) has this transition of information from the interlocutor to the listener with their use of `oh', signalling information in a shared focus of attention (with A saying ``Oh no that costs more" and B responding ``We should erase it"). We see similar patterns of behaviour towards the end of the dialogue (by this point, interlocutors have had opportunity to build a collaboration with each other). 

The intuition behind H2.2 seems reasonable here; Team 20 for example, had 65 occurrences of the information marker `oh', but they significantly differ from the 30 times the instructions given by the IG was (mis)matched by the IF. Interestingly, we observe in the last period for Team 20 a lack of inferred instructions. Inferred instructions are a precursor to an action being (mis)matched or nonmatched. Indeed, there is also a lack of nonmatched actions, which typically occur when the interlocutor takes the liberty to follow their own intentions. Here, they do not even verbalise their own intentions, visible from the lack of inferred instructions. This indicates a strong tendency of working in isolation despite the design of the task.

\paragraph{Synopsis.}
Overall, regardless of a team's task success, we see that `oh' does occur earlier than (mis)matched instructions-to-actions, as evidenced by the negative effect sizes of Cliff's Delta. Specifically for performance, there is a general trend that for well-performing teams the `oh's occur more in the vicinity of (mis)match times with larger overlap between the two groups, and the badly-performing teams have comparably less overlap. This result supports H2.2. While we cannot conclude on the results for learning, using our automatically annotated instructions-to-actions and occurrences of `oh', we still gain some insight into the way the teams collaborate\footnote{Future work could expand more on the inferred instructions and nonmatches and their implications of collaboration, rather than only focusing on (mis)matched actions.}.
